Recurring Contingent Service Payment

Fair exchange protocols let two mutually distrustful parties exchange digital data in a way that neither party can cheat. They have various applications such as the exchange of digital items, or the exchange of digital coins and digital services between a buyer/client and seller/server. In this work, we formally define and propose a generic blockchain-based construction called "Recurring Contingent Service Payment" (RC-S-P). It (i) lets a fair exchange of digital coins and verifiable service reoccur securely between clients and a server while ensuring that the server is paid if and only if it delivers a valid service, and (ii) ensures the parties' privacy is preserved. RC-S-P supports arbitrary verifiable services, such as "Proofs of Retrievability" (PoR) or verifiable computation and imposes low on-chain overheads. Our formal treatment and construction, for the first time, consider the setting where either client or server is malicious. We also present a concrete efficient instantiation of RC- S-P when the verifiable service is PoR. We implemented the concrete instantiation and analysed its cost. When it deals with a 4-GB outsourced file, a verifier can check a proof in only 90 milliseconds, and a dispute between a prover and verifier is resolved in 0.1 milliseconds. At CCS 2017, two blockchain-based protocols were proposed to support the fair exchange of digital coins and a certain verifiable service; namely, PoR. In this work, we show that these protocols (i) are susceptible to a free-riding attack which enables a client to receive the service without paying the server, and (ii) are not suitable for cases where parties' privacy matters, e.g., when the server's proof status or buyer's file size must remain private from the public. RC- S-P simultaneously mitigates the above attack and preserves the parties' privacy.

==> Conclusion_2.tex <==
% !TEX root =main.tex

\section{Conclusion}


Fair exchange is an interesting problem. It captures the scenario in which two mutually distrusted parties want to swap digital items such that   either each party gets the other's item, or neither party does.  Solutions to the problem are often certain cryptographic protocols. They have numerous real-world applications; especially, nowadays where the use of  the Internet for conducting business is swiftly increasing. Many years ago, it was shown that fairness is unachievable without the aid of a trusted third party. However, the advent of  blockchain offered a possibility to eliminate the trusted third party’s involvement. Therefore,  various blockchain-based fair exchange protocols were proposed. In this work, we showed that the blockchain-based fair exchange protocols are not suitable for the exchange of digital coins and digital verifiable services. If they are used directly, in this setting, then serious issues would arise, i.e., real-time information leakage and waste of seller's resources. We formally defined and proposed a generic construction called ``recurring contingent service payment'' (RC-S-P) that addresses the issues. RC-S-P lets a fair exchange of digital coins and verifiable service's proof, while ensuring that the buyer cannot waste the seller's resources, and the parties' privacy is preserved. RC-S-P uses smart contracts; however, most of the computation is performed off-chain which makes the smart contracts-side computation  very low. RC-S-P is the first fair service payment scheme that offers a combination of  the above appealing features.  We also presented concrete instantiation of the RC-S-P, when the verifiable service is the ``proofs of retrievability'' (PoR). The instantiation is called ``recurring contingent PoR payment'' (RC-PoR-P). We  implemented the RC-PoR-P and analysed its costs. Our cost evaluation indicated that the RC-PoR-P is  efficient. RC-PoR-P is the first PoR scheme that offers all the above features at once.

%\clearpage

==> Definition.tex <==
% !TEX root =main.tex

\section{Definitions}\label{Definition}

%In this section, first we present a generic formal definition of a verifiable service (VS) scheme. Second, we provide a formal definition of an enhanced VS scheme that  allows: (a) either party to be malicious and (b) a trusted third party arbiter, to identify a corrupt party. We call the  scheme that offers the above features \emph{verifiable service with identifiable abort (VSID}).   Third, we present a formal definition of an upgraded VSID scheme that  addresses   the issues we identified in Section \ref{sec::previous-work-limitations}, i.e., wasting server's resources and real-time leakage of service input and proof's status.  We call the latter scheme \emph{recurring contingent service payment (RC-S-P)}. 



In this section, we present a formal definition of a scheme called \emph{recurring contingent service payment} (RC-S-P) that addresses the issues we identified in Section \ref{sec::previous-work-limitations}, i.e., wasting server's resources and real-time leakage of service input and proof's status.    Before we present the formal definition of RC-S-P, we outline what a verifiable service (VS) is. At a high level, a verifiable service scheme is a two-party protocol in which a client chooses a function, $F$, and provides (an encoding of) $F$, its input $u$, and a query $\bm{q}$ to a server.  The server is expected to evaluate $F$ on $u$ and $\bm{q}$ (and some public parameters) and respond with the output. Then, the client verifies that the output is indeed the output of the function computed on the provided input. In verifiable services, either the computation (on the input) or both the computation and storage of the input are delegated to the server. We present a full formal definition of a verifiable service in Appendix \ref{}. Now, we present the definition of RC-S-P (which also captures VS's definition).


%\input{VS-definition.tex}
%
%\input{VSID-definition.tex}

\input{RC-S-P-Definition}











==> Merkle-tree.tex <==
% !TEX root =main.tex


\section{Merkle Tree}\label{sec::merkle-tree}


In the setting where  a Merkle tree is used to remotely check a file, the file  is  split into blocks and the tree is built on top of the file blocks. Usually, for the sake of simplicity, it is assumed the number of blocks, $m$, is a power of $2$. The height of the tree, constructed on $m$ blocks, is $\log_{\st 2}(m)$. The 
Merkle tree scheme includes three algorithms $(\mathtt{MT.genTree}, \mathtt{MT.prove}, \mathtt{MT.verify})$ as follows: 

%There are  roles invovled, the prover $\mathcal{P}$ and the verifier $\mathcal{V}$. 



\begin{itemize}
\item[$\bullet$] The algorithm that constructs a Merkle tree, $\mathtt{MT.genTree}$, is run by $\mathcal{V}$. It takes file blocks, $u:=u_{\st 1},...,u_{\st m}$, as input. Then, it groups the blocks  in pairs. Next,   a collision-resistant hash function, $\mathtt{H}(.)$, is used to hash each pair. After that, the hash values are grouped in pairs and each pair is further hashed, and this process is repeated until only a single hash value, called ``root'', remains. This yields a  tree with the leaves corresponding to the blocks of the input file and the root corresponding to the last remaining hash value.  $\mathcal{V}$ locally stores the root, and sends the file and tree to $\mathcal{P}$.

\item[$\bullet$] The proving algorithm, $\mathtt{MT.prove}$, is run by $\mathcal{P}$. It takes a block index, $i$, and a tree as inputs. It outputs  
a vector proof, of  $\log_{\st 2}(m)$ elements. The proof asserts the membership of $i$-th block in the tree, and consists of  all the sibling nodes on a path from the $i$-th block to the root of the Merkle tree (including $i$-th block). The proof is given to $\mathcal{V}$.

\item[$\bullet$] The verification algorithm, $\mathtt{MT.verify}$, is run by $\mathcal{V}$. It takes as input $i$-th block, a proof and tree's root. It checks if the $i$-th block corresponds to the root. If the verification passes, it outputs $1$; otherwise, it outputs $0$.

\end{itemize}

The Merkle tree-based scheme has two properties: \emph{correctness} and \emph{security}. Informally, the correctness requires that if both parties run the algorithms correctly, then a proof  is always accepted by  $\mathcal{V}$. The security requires that a computationally bounded malicious $\mathcal{P}$ cannot convince  $\mathcal{V}$ into accepting an incorrect proof, e.g., proof for non-member block. The security  relies on the assumption that it is computationally infeasible to find the hash function's collision. 

==> PRF.tex <==
% !TEX root =main.tex





\section{Pseudorandom Function}\label{subsec:PRF}

Informally, a pseudorandom function ($\mathtt{PRF}$) is a deterministic function that takes as input a key and some argument and outputs a value  indistinguishable from that of a truly random function with the same domain and range.  Pseudorandom functions have many applications in cryptography as they provide an efficient and deterministic way to turn  input into a value that looks random. Below, we restate the formal definition of $\mathtt{PRF}$, taken from \cite{DBLP:books/crc/KatzLindell2007}. 

\begin{definition} Let $W:\{0,1\}^{\st\psi}\times \{0,1\}^{\st \eta}\rightarrow \{0,1\}^{\st  \iota}$ be an efficient  keyed function. It is said $W$ is a pseudorandom function if for all probabilistic polynomial-time distinguishers $B$, there is a negligible function, $\mu(.)$, such that:

\begin{equation*}
\bigg | \Pr[B^{\st W_{\hat{k}}(.)}(1^{\st \psi})=1]- \Pr[B^{\st \omega(.)}(1^{\st \psi})=1] \bigg |\leq \mu(\psi)
\end{equation*}
where  the key, $\hat{k}\stackrel{\st\$}\leftarrow\{0,1\}^{\st\psi}$, is chosen uniformly at random and $\omega$ is chosen uniformly at random from the set of functions mapping $\eta$-bit strings to $\iota$-bit strings.
\end{definition}

==> PoRID-Proof.tex <==
% !TEX root =main.tex


%\subsection{Proof of PoRID}\label{sec::Proof-of-PoRID}


In this section, we prove the security of the PoRID. \\

%\begin{reptheorem}{thm:PoRID}
%The PoRID protocol satisfies the $\epsilon$-soundness, inputs well-formedness, and detectable abort properties, w.r.t. Definitions \ref{deff::PoRID-Soundness}, \ref{deff::VSID-Inputs-Well-formedess}, and \ref{def::VSID-Identifiable-Abort}, if the PoR is $\epsilon$-sound and the  blockchain   is secure.
%\end{reptheorem}

\textsc{Theorem~\ref{thm:PoRID}.}
\emph{The PoRID protocol presented in Subsection~\ref{subsec:PoRID} satisfies the $\epsilon$-soundness, inputs well-formedness, and detectable abort properties, (cf. Definitions \ref{extractable}, \ref{deff::VSID-Inputs-Well-formedess}, and \ref{def::VSID-Identifiable-Abort}), if the underlying PoR is $\epsilon$-sound and the underlying signature scheme is secure.}

\begin{proof}[Proof sketch]
The $\epsilon$-soundness of the PoRID  stems from the security of the PoR scheme, i.e., $\epsilon$-soundness. Specifically,
in the PoRID the (honest) client makes black-box calls to the algorithms of the PoR, to ensure the soundness. In the PoRID no additional message is provided to the adversary/server.  It receives the same messages as it receives in the PoR. The latter scheme's soundness ensures that an extractor can recover the entire file interacting with a corrupt server which passes  $\epsilon$ fraction of challenges. On the other hand, the inputs well-formedness holds for the following reasons. The metadata generation algorithm, i.e., the Merkle tree algorithm that builds a tree and computes a root, is deterministic and involves only public  parameters. Thus, given the tree's leaves (i.e., file blocks), its parameters, and the root, anyone can reconstruct it, check if it yields the same root, and verify the tree's parameters. Also, a query contains a single random key, $\hat{k}$, whose correctness can be checked deterministically, i.e., by checking $\hat{k}\neq \bot$ and  $\hat{k}\in \{0,1\}^{\st\psi}$. The detectable abort property holds as long as the soundness and inputs well-formedness hold and the blockchain is secure. The reason is that algorithm $\mathtt{PoRID.identify}(.)$, which ensures detectable abort, is a wrapper function that makes black-box calls to algorithms $\mathtt{PoRID.checkQuery}(.)$ and $\mathtt{PoR.verify}(.)$, where the former  ensures input, i.e., query, well-formedness, and the latter  ensures soundness.  


The (blockchain's) signature security ensures if  a proof (or a transaction in general) is signed correctly, then it cannot be repudiated by the signer later, this  guarantees the signer is held accountable for a rejected proof it provided. Moreover, a malicious party cannot frame an honest party for proving  an ill-formed or no proof. In particular, to do that, it has to either (a)  forge the honest party's signature, so it can send an ill-formed proof on its behalf, or (b) fork the blockchain so the chain comprising the accepting proof is discarded. In the former case,  the adversary's probability of success  is negligible as long as the  signature is secure. The adversary has the same success probability  in the  latter case; because it has to generate a long enough chain that excludes the accepting proof which has a negligible success probability, under the assumption that the hash power of the adversary is lower than those of honest miners and  due to the blockchain's \emph{liveness} property an honestly generated transaction will eventually appear on an honest miner's chain \cite{GarayKL15}.
%
%The blockchain's signature security ensures if a proof is not signed correctly, then it will not be registered in the smart contract  and the signer is held accountable for not providing a proof; on the other hand, if a proof is signed correctly, then it cannot be repudiated by the signer later, this  guarantees the signer is held accountable for a rejected proof it provides. Moreover, a malicious party cannot frame an honest party. In particular, to do that, it has to either (a)  forge the honest party's signature, to send an ill-formed message on its behalf, or (b) fork the blockchain so the chain comprising the accepting proof is discarded. In the former case,  the adversary's probability of success  is negligible as long as the blockchain's signature is secure.
%
\end{proof}



==> PoRID-protocol.tex <==
% !TEX root =main.tex


\subsection{PoRID Protocol}\label{subsec:PoRID}

In this section, we present ``PoR with identifiable abort'' (PoRID) that is a concrete instantiation of $\text{VSID}_{\st\text{light}}$. It is built upon the PoR protocol, presented in the previous section and is in the same security model as $\text{VSID}_{\st\text{light}}$ is, i.e., either $\mathcal C$ or $\mathcal S$ can be malicious. In PoRID similar to $\text{VSID}_{\st\text{light}}$, $\mathcal C$ and $\mathcal S$ use a bulletin board to exchange signed messages.  In the protocol, at setup $\mathcal C$ encodes its file and generates public parameters and  metadata.  It posts the public parameters and metadata to the bulletin board and   sends the encoded file to $\mathcal S$ which runs a few lightweight checks to ensure the correctness of the public parameters and metadata. It agrees to serve if it is convinced of their correctness. Later, when $\mathcal C$ wants to ensure the availability of its outsourced file, it  generates and posts a query  to the board.   $\mathcal S$  checks the correctness of the query, by performing a couple of highly efficient verifications. 

The server-side prove and client-side verify algorithms are similar to those in PoR with a difference that $\mathcal S$ posts the PoR proofs (i.e., the output of prove algorithm) to the board. In  case of any dispute, $\mathcal C$ or $\mathcal S$ invokes the arbiter which, given the signed posted messages, checks the proofs  to identify a corrupt party. In particular,  it first checks the validity of the query (regardless of the party which invokes it). However, if  is invoked by  $\mathcal C$, it also checks  only one of the PoR proofs that the client claims it is invalid. Thus, it is much more efficient than $\text{VSID}_{\st\text{light}}$ as it does not need any zero-knowledge proofs (mainly due to the use of Merkle tree) and requires the  arbiter to check only one of the proofs (due  to the idea of proof of misbehaviour). PoRID protocol is presented below.






\begin{enumerate}
   
\item\textbf{Client-side Setup}. $\mathtt{PoRID.setup}(1^{\lambda}, u)$ 
\begin{enumerate}
\item Calls  $\mathtt{PoR.setup}(1^{\lambda}, u)\rightarrow (u^{\st *},pp)$, that results in public parameters $pp:=(\sigma, \phi, m, \zeta)$ and encoded file: $u^{\st *}=u^{\st '}_{\st 0}||0,...,u^{\st '}_{\st m}||m$. Recall that  $\zeta:=(\psi,\eta, \iota)$ is the $\mathtt{PRF}$'s description.

\item Posts $pp$ to the bulletin board and sends $u^{\st *}$ to $\mathcal{S}$. 
\end{enumerate}



%\TZ{The key generation algorithm is missing. Is this on purpose, and if so, why we deviate from the VSID syntax?}--> Aydin: yes it's on purpose-- because (a) all public parameters are  generated in the setup, and (b) no verification keys are needed anymore. Also, it can be seen as a ''subclass'' of the VSID definition, so it may not be deviation from VSID syntax. 

\item\textbf{Server-side Setup}. $\mathtt{PoRID.serve}(u^{\st *},pp)$
%\begin{enumerate}

Verifies the correctness of public parameters:
\begin{enumerate}
\item rebuilds  the Merkle tree on $u^{\st *}$ and checks the resulting root equals $\sigma$.
\item checks $|u^{*}|=m$ and  $\phi\leq m$.
\end{enumerate}
 If the proofs are accepted, then  it outputs $a = 1$ and proceeds to the next step; otherwise, it outputs $a = 0$ and halts.
 
 




\item\textbf{Client-side Query Generation}. $\mathtt{PoRID.genQuery}(1^{\lambda},  pp)$ 
\begin{enumerate}
\item Calls $\mathtt{PoR.genQuery}(1^{\lambda}, pp)\rightarrow \hat{k}$, to generate a key, $\hat{k}$. %whose element have been sorted 
\item Posts $\hat{k}$ to the board. 
\end{enumerate}




\item\textbf{Server-side Query Verification}. $\mathtt{PoRID.checkQuery}(\hat{k}, pp)$
\begin{enumerate}
\item  Checks if  $\hat{k}$ is not empty, i.e., $\hat{k}\neq \bot$, and is in the key's universe, i.e., $\hat{k}\in \{0,1\}^{\st\psi}$.%If it is empty, then it outputs $I=\mathcal C$
\item  If the checks pass, then it outputs $b=1$; otherwise, it outputs $b=0$.


\end{enumerate}




\item\textbf{Server-side Service Proof Generation}. $\mathtt{PoRID.prove}(u^{\st *},\hat{k},pp)$.
\begin{enumerate}
\item Calls $\mathtt{PoR.prove}(u^{\st *},\hat{k},pp)\rightarrow  {\bm{\pi}}$, to generate proof vector, $ {\bm{\pi}}$. 
\item Posts $ {\bm{\pi}}$ to the board. 
\end{enumerate}



\item\textbf{Client-side Proof Verification}\label{PoRID::Client-side-Proof-Verification}. $\mathtt{PoRID.verify}( {\bm{\pi}},\hat{k} ,pp)$
%\begin{enumerate}

 Calls $\mathtt{PoR.verify}( {\bm{\pi}},\hat{k} ,pp)\rightarrow  {\bm{d}}$, to verify the proof. If $ {\bm{d}}[0] = 1$,  it accepts the proof; otherwise, it rejects it.




\item\textbf{Arbiter-side Identification}\label{PoRID::Arbiter-side-Identification}. $\mathtt{PoRID.identify}( {\bm{\pi}}, q,pp)$ 

This algorithm can be invoked by $\mathcal{C}$ or $\mathcal{S}$, in the case of a dispute. Let  $q:=(\hat{k},g)$. If it is invoked by $\mathcal{C}$, then $g$ refers to a rejected proof's  index; however, if it is invoked by $\mathcal{S}$, then $g$ is null, i.e.,  $g=\bot$. The arbiter performs as follows. 


\begin{enumerate}



\item Ensures  query $\hat{k}$ is well-structured by calling $\mathtt{PoRID.checkQuery}(\hat{k}, pp)$. If it returns $b=0$, then it outputs $I=\mathcal C$ and halts; otherwise, it proceeds to the next step. 




\item Derives the related challenged block's index from $\hat{k}$, by computing $q_{\st g}=\mathtt{PRF}(\hat{k},g)\bmod m+1$.



\item If $g\neq \bot$, then verifies only $g$-th proof, by setting $\hat{\bm{\pi}}={\bm{\pi}}[g], \hat{\bm{q}}=q_{\st g}$ and then calling $\mathtt{PoR.verify}( \hat{\bm{\pi}},\hat{\bm{q}},$ $pp)\rightarrow  {\bm{d}}'$. If $ {\bm{d}}'[0]=0$, then it outputs $I=\mathcal S$. Otherwise, it outputs $I=\bot$.
\end{enumerate}
\end{enumerate}

%\TZ{In the Theorem below we should say that the security properties are satisfied for some $F,M,Q$.}--> Aydin: We have already defined each function in the context of PoR. 

\begin{theorem}\label{thm:PoRID}
The PoRID protocol presented in Subsection~\ref{subsec:PoRID} satisfies the $\epsilon$-soundness, inputs well-formedness, and detectable abort properties, (cf. Definitions \ref{extractable}, \ref{deff::VSID-Inputs-Well-formedess}, and \ref{def::VSID-Identifiable-Abort}), if the underlying PoR is $\epsilon$-sound and the underlying signature scheme is secure.
\end{theorem}

We refer readers to Appendix \ref{sec::Proof-of-PoRID} for the above theorem's proof. 

%\TZ{shouldn't we prove VSID soundness instead? and what about correctness?}--> Aydin: in Section 5, we highlight that PoR definition  is a VS’s special case. In particular, PoR’s ε-soundness captures VS’s soundness. Also, in the below proof we say that in PoRID no additional message is given to the adversary than what is given to it in PoR. Therefore, PoRID soudness is equivalent to PoR soundness. 

%\begin{proof}[Proof sketch]
%The $\epsilon$-soundness of PoRID directly stems from the security of PoR scheme, i.e., $\epsilon$-soundness. Specifically,
%in PoRID the (honest) client makes black-box calls to the algorithms of PoR, to ensure the soundness. In PoRID no additional message is provided to the adversary/server.  It receives the same messages as it receives in PoR. The latter scheme's soundness ensures that an extractor can recover the entire file interacting with a corrupt server that passes  $\epsilon$ fraction of challenges. On the other hand, the inputs well-formedness holds for the following reasons. The metadata generation algorithm, i.e., the Merkle tree algorithm that builds a tree and computes a root, is deterministic and involves only public  parameters. Thus, given the tree's leaves (i.e., file blocks), its parameters, and the root, anyone can reconstruct it, check if it yields the same root, and verify the tree's parameters. Also, a query contains a single random key, $\hat{k}$, whose correctness can be checked deterministically, i.e., by checking $\hat{k}\neq \bot$ and  $\hat{k}\in \{0,1\}^{\st\psi}$. The detectable abort property holds as long as the soundness and inputs well-formedness hold and the signature scheme is secure. The reason is that algorithm $\mathtt{PoRID.identify}(.)$, which ensures detectable abort, is a wrapper function that makes black-box calls to algorithms $\mathtt{PoRID.checkQuery}(.)$ and $\mathtt{PoR.verify}(.)$, where the former  ensures input (i.e., query) well-formedness, and the latter  ensures soundness.  The signature’s security ensures if a proof is not signed correctly, then it can also be rejected by the arbiter and the signer is held accountable for providing an ill-formed message; on the other hand, if a proof is signed correctly, then it cannot be repudiated by the signer later on that guarantees the signer is held accountable for a rejected proof it provides. 
%%\hfill\(\Box\)
%\end{proof}
%





==> RC-PoR-P-Definition.tex <==
% !TEX root =main.tex

\section{Recurring Contingent PoR Payment Definition}\label{sec::RC-PoR-P-Definition}





\begin{definition}[RC-PoR-P Scheme]\label{RC-PoR-P-def}
A recurring contingent service payment scheme RCPoRP  $=(\mathtt{RCPoRP}.\mathtt{keyGen}, $ $\mathtt{RCPoRP}.\mathtt{cInit}, $ $\mathtt{RCPoRP}.\mathtt{sInit},  $ $\mathtt{RCPoRP}.\mathtt{genQuery},\mathtt{RCPoRP}.\mathtt{prove},\mathtt{RCPoRP}.\mathtt{verify},\mathtt{RCPoRP}.\mathtt{resolve},\mathtt{RCPoRP}.\mathtt{pay})$ involves three parties; namely, client, server,  and smart contract, and consists of eight algorithms defined as follows.


\begin{itemize}

\item[$\bullet$] $\mathtt{RCPoRP}.\mathtt{keyGen}(1^{\scriptscriptstyle\lambda})\rightarrow k$.  A probabilistic algorithm run by the client. It takes as input security parameter $1^{\scriptscriptstyle\lambda}$. It outputs $\bm{k}$ that contains a pair of secret and public parameters, $k:=(sk',pk')$. It sends  $pk'$ to the smart contract.

\

\item[$\bullet$] $\mathtt{RCPoRP}.\mathtt{cInit}(1^{\scriptscriptstyle\lambda}, u, k, z, pl,enc)\rightarrow (u^{\scriptscriptstyle *},T, p_{\scriptscriptstyle\mathcal S},  \bm{y}, coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C})$. It is run by the client. It takes as input $1^{\scriptscriptstyle\lambda}$,  the service input $u$, key pair  $k:=(sk', pk')$,   the total number of verifications $z$,   price list $pl$ containing pairs of  actual coin amount for each accepting service proof and the amount for covering each potential dispute resolution's cost, and encoding/decoding functions $enc:=(E,D)$ used to encode/decode the service queries/proofs.  It encodes $u$, that yields  $u^{\scriptscriptstyle *}$. It computes $pp$ that contains a set of input dependent parameters $pp'$ and a  representation of $\sigma=M(u^{\scriptscriptstyle *},{pp'})$. It sets value of $p_{\scriptscriptstyle\mathcal S}$ to the total coins the server should deposit. It picks a private price pair $(o,l)\in pl$. It sets coin secret parameters $cp$ that include $(o,l)$ and parameters of $pl$, e.g. its maximum values. It constructs coin encoding token $T_{\scriptscriptstyle cp}$ containing   $cp$ and   $cp$'s witness, $g_{\scriptscriptstyle cp}$. It   constructs  encoding token $T_{\scriptscriptstyle qp}$ that contains secret  parameters $qp$ including {$pp$} and those (in $sk'$) that will be used to encode the service queries/proofs. Also  $T_{\scriptscriptstyle qp}$ contains     $qp$'s witness,  $g_{\scriptscriptstyle qp}$.   Given a valid value and its witness  anyone can check if they match. It sets a vector of parameters $\bm{y}$ that includes  binary vectors $[\bm{y}_{\scriptscriptstyle \mathcal  C}, \bm{y}_{\scriptscriptstyle \mathcal  S}]$ each of which is set to $0$ and its length is $z$.  It outputs  $u^{\scriptscriptstyle *}$,   $T:=(T_{\scriptscriptstyle cp},T_{\scriptscriptstyle qp})$,  $p_{\scriptscriptstyle\mathcal S}$,    $\bm{y}$,  and the encoded coins amount  $coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C}$ (that contains $o_{\scriptscriptstyle i}$ and $l_{\scriptscriptstyle i}$ coins in an encoded form). The client sends  $u^{\scriptscriptstyle *}$, $z$, $T_{\scriptscriptstyle cp} \setminus  \{g_{\scriptscriptstyle cp}\}$ and $T_{\scriptscriptstyle qp} \setminus  \{g_{\scriptscriptstyle qp}\}$ to the server and  sends $g_{\scriptscriptstyle cp},  g_{\scriptscriptstyle qp},p_{\scriptscriptstyle\mathcal S}$, and $\bm{y}$,  and $coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C}$  coins to the  contract. 





%\item[$\bullet$] $\mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, M,z,pl,enc)\rightarrow (u^{\scriptscriptstyle *},e,T, p_{\scriptscriptstyle\mathcal S},  \bm{y}, coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C},pk^{\scriptscriptstyle *})$. It is run by the client. It takes as input $1^\lambda$,  the service input $u$,  the keys  $\bm{k}:=(k, K')$,  the metadata generator function $M$, the total number of verifications $z$, and  price list $pl:\{(o_{\scriptscriptstyle 1},l_{\scriptscriptstyle 1}),...,(o_{\scriptscriptstyle m},l_{\scriptscriptstyle m})\}$, where  each pair contains actual coin amounts for each accepting service proof $o_{\scriptscriptstyle i}$, and for covering each potential dispute resolution's cost, $l_{\scriptscriptstyle i}$.  The algorithm also takes as input encoding/decoding functions $enc:=(E,D)$ used to encode/decode the service public-key/queries/proofs.  It encodes $u$, that results in $u^{\scriptscriptstyle *}$.  It computes metadata $\sigma=M(u^{\scriptscriptstyle *},k)$ and a  proof $w_{\scriptscriptstyle\sigma}$ asserting the metadata is well-structured. It sets value of $p_{\scriptscriptstyle\mathcal S}$ to the total coins the server should deposit. It picks a private price pair $(o_{\scriptscriptstyle i},l_{\scriptscriptstyle i})\in pl$, e.g. depending on the service type or input size. It sets coin secret parameters $cp$ that include $(o_{\scriptscriptstyle i},l_{\scriptscriptstyle i})$ and parameters of $pl$, e.g. its maximum values. It constructs coin encoding token $T_{\scriptscriptstyle cp}$ containing   $cp$ and   $cp$'s witness, $g_{\scriptscriptstyle cp}$.  It   constructs  encoding token $T_{\scriptscriptstyle qp}$ comprising secret  parameters $qp\in K'$ (used to encode the public key and service queries/proofs)  and     $qp$'s witness,  $g_{\scriptscriptstyle qp}$.   Given a valid value and its witness  anyone can check if they match. It sets a vector of parameters $\bm{y}$ that includes  binary vectors $[\bm{y}_{\scriptscriptstyle \mathcal  C}, \bm{y}_{\scriptscriptstyle \mathcal  S},\bm{y}'_{\scriptscriptstyle \mathcal  C}, \bm{y}'_{\scriptscriptstyle \mathcal  S}]$ each of which is set to $0$ and its length is $z$.  It may add other  parameters, e.g. input size, to $pk$. It encodes  $pk^{\scriptscriptstyle *}=E(pk,T_{\scriptscriptstyle qp})$. It outputs encoded input $u^{\scriptscriptstyle *}$, metadata-proof pair $e:=(\sigma,w_{\scriptscriptstyle\sigma})$, the two sets $T:=(T_{\scriptscriptstyle cp},T_{\scriptscriptstyle qp})$, the total coins amount the server should deposit $p_{\scriptscriptstyle\mathcal S}$, the  binary vectors $\bm{y}$,   the encoded coins amount  $coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C}$ (that contains $o_{\scriptscriptstyle i}$ and $l_{\scriptscriptstyle i}$ coins in an encoded form) and the encoded public key $pk^{\scriptscriptstyle *}$. The client sends  $u^{\scriptscriptstyle *}$, $z$,  $e$, $T_{\scriptscriptstyle cp} \setminus  \{g_{\scriptscriptstyle cp}\}$ and $T_{\scriptscriptstyle qp} \setminus  \{g_{\scriptscriptstyle qp}\}$ to the server and  sends $g_{\scriptscriptstyle cp},  g_{\scriptscriptstyle qp},p_{\scriptscriptstyle\mathcal S}$, $\bm{y}$,   $coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C}$  coins, and $pk^{\scriptscriptstyle *}$ to the smart contract. 



%-------------Commented out on 26-11-20
%\item[$\bullet$] $\mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, M,z,cp)\rightarrow (u^{\scriptscriptstyle *},e,t,coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C}, \bm{y}_{\scriptscriptstyle \mathcal  C},\bm{y}_{\scriptscriptstyle \mathcal  S})$. It is run by the client. It takes as input $1^\lambda$,  the service input $u$,  the keys  $\bm{k}:=(k, K')$,  the metadata generator function $M$, the total number of verifications $z$, and coin secret parameters $cp$ that include a subset of  $K'$ and the actual amount of coins for each accepting service proof $o$ and  for covering each potential dispute resolution's cost $l$.  It encodes $u$, that results in $u^{\scriptscriptstyle *}$.  It computes metadata $\sigma=M(u^{\scriptscriptstyle *},k)$ and a  proof $w_{\scriptscriptstyle\sigma}$ asserting the metadata is well-structured.  It constructs coin encoding token $T_{\scriptscriptstyle cp}$ that contains   $cp$, total coins the server should deposit $p_{\scriptscriptstyle\mathcal S}$, and   $cp$'s witness, $g_{\scriptscriptstyle cp}$.  It also constructs query/proof encoding token $T_{\scriptscriptstyle qp}$ that contains  secret  parameters $qp\in K'$ (used to encode the service queries/proofs)  and     $qp$'s witness,  $g_{\scriptscriptstyle qp}$.   Given a valid value and its witness  anyone can check if they match. It constructs two binary vectors $\bm{y}_{\scriptscriptstyle \mathcal  C}$ and $\bm{y}_{\scriptscriptstyle \mathcal  S}$ that are set to $0$ and their length is $z$.  It outputs encoded input $u^{\scriptscriptstyle *}$, metadata-proof pair $e:=(\sigma,w_{\scriptscriptstyle\sigma})$, the two sets $T:=(T_{\scriptscriptstyle cp},T_{\scriptscriptstyle qp})$, the two binary vectors $\bm{y}_{\scriptscriptstyle \mathcal  C}, \bm{y}_{\scriptscriptstyle \mathcal  S}$, and  the encoded coins amount  $coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C}$ (i.e. contains $o$ and $l$ coins in an encoded form). The client sends  $u^{\scriptscriptstyle *}$, $z$, $pk$, $e$, $T_{\scriptscriptstyle cp} \setminus  \{g_{\scriptscriptstyle cp},p_{\scriptscriptstyle\mathcal S}\}$ and $T_{\scriptscriptstyle qp} \setminus  \{g_{\scriptscriptstyle qp}\}$ to the server and  sends $\{g_{\scriptscriptstyle cp},  g_{\scriptscriptstyle qp},p_{\scriptscriptstyle\mathcal S}\}$, $\bm{y}_{\scriptscriptstyle \mathcal  C}$, $\bm{y}_{\scriptscriptstyle \mathcal  S}$  and $coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C}$ coins to the smart contract. 
%--------------------------

%\item[$\bullet$] $\mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, M,z,o,l,E_{\scriptscriptstyle 1})\rightarrow (u^{\scriptscriptstyle *},e,t,coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C})$. It is run by the client. It takes as input $1^\lambda$,  the service input: $u$,  the key pair: $(k, k')$,  metadata generator function: $M$, total number of verifications: $z$,  the amount of coins for each accepting service proof: $o$,  coins amount  to cover each potential dispute resolution's cost: $l$ and  encoding function $E_{\scriptscriptstyle 1}$ to encode the coins actual amount.  It encodes $u$, that results $u^{\scriptscriptstyle *}$.  It computes a metadata, $\sigma=M(u^{\scriptscriptstyle *},k)$, and a publicly verifiable zero-knowledge proof $w_{\scriptscriptstyle\sigma}$ asserting the metadata is well-structured.  It constructs coins' token $t_{\scriptscriptstyle cp}$ that contains  coin's secret  parameters $cp$ and   sealed    parameters $sld_{\scriptscriptstyle cp}$. Given $cp$ and $sld_{\scriptscriptstyle cp}$ anyone can check if $sld_{\scriptscriptstyle cp}$ corresponds to $cp$. It constructs  encoding token $t_{\scriptscriptstyle pq}$ that contains  secret  parameters $qp\in k'$ (used to encode the service queries/proofs) and  sealed   parameters $sld_{\scriptscriptstyle qp}$, where  given $qp$ and $sld_{\scriptscriptstyle qp}$ anyone can check if $sld_{\scriptscriptstyle qp}$ corresponds to $qp$.  It outputs encoded input $u^{\scriptscriptstyle *}$, metadata-proof pair $e:(\sigma,w_{\scriptscriptstyle\sigma})$, the two sets $t:\{t_{\scriptscriptstyle cp},t_{\scriptscriptstyle qp}\}$ and  the encoded coins amount  $coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C}=E_{\scriptscriptstyle 1}(z,cp)$. The server is  given $u^{\scriptscriptstyle *}$,  $e$, and $t \setminus  \{sld_{\scriptscriptstyle cp},sld_{\scriptscriptstyle qp}\}$ and  the smart contract  is given $sld_{\scriptscriptstyle cp}$,  $sld_{\scriptscriptstyle qp}$ and $coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C}$ coins by the client. 


%\item[$\bullet$] $\mathtt{VS.setup}(1^{\lambda}, u,k, M)\rightarrow \sigma$. A probabilistic algorithm run by the client. It takes as input security parameter,  the service input: $u$,  the key pair: $k$ and metadata generator deterministic function: $M$, publicly known. It runs $M(u,k)$ and outputs  metadata: $\sigma$. Right after that, the server might be given $u$,  $\sigma$ and $pk$. 

\


\item[$\bullet$] $\mathtt{RCPoRP}.\mathtt{sInit}(u^{\scriptscriptstyle *},z, T, p_{\scriptscriptstyle\mathcal S},\bm{y},enc)\rightarrow (coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S},a)$. It is  run by the server. It takes as input the  service encoded input $u^{\scriptscriptstyle *}$, the total number of verifications $z$, and $T:=(T_{\scriptscriptstyle cp},T_{\scriptscriptstyle qp})$ (where $\{g_{\scriptscriptstyle cp},  g_{\scriptscriptstyle qp}\}$ are read from the smart contract). Also, it reads $p_{\scriptscriptstyle\mathcal S}$, and $\bm{y}$ from the smart contract and takes as input the encoding/decoding functions $enc:=(E,D)$. It verifies the validity of $T$'s elements. It checks elements of $\bm{y}$ and ensures element of $\bm{y}_{\scriptscriptstyle \mathcal  C}, \bm{y}_{\scriptscriptstyle \mathcal  S}\in \bm{y}$ have been set to $0$. If all checks are successful, then it encodes the amount of its coins  $coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal S}$ and sets $a=1$. Otherwise, it sets $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S}=\bot$ and $a=0$. It outputs $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S}$ and $a$. The smart contract is given $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S}$ coins and $a$.  



%\item[$\bullet$] $\mathtt{RCSP}.\mathtt{sInit}(u^{\scriptscriptstyle *},e, pk^{\scriptscriptstyle *},z, T, p_{\scriptscriptstyle\mathcal S},\bm{y},enc)\rightarrow (coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S},a)$. It is  run by the server. It takes as input the  service encoded input $u^{\scriptscriptstyle *}$, metadata-proof pair $e:=(\sigma,w_{\scriptscriptstyle\sigma})$,  encoded public key $pk^{\scriptscriptstyle *}$ (read from the contract), the total number of verifications $z$, and $T:=(T_{\scriptscriptstyle cp},T_{\scriptscriptstyle qp})$ (where $\{g_{\scriptscriptstyle cp},  g_{\scriptscriptstyle qp}\}$ are read from the smart contract). Also, it reads $p_{\scriptscriptstyle\mathcal S}$, and the parameters in $\bm{y}$ from the smart contract and takes as input the encoding/decoding functions $enc:=(E,D)$. It decodes the public key, $pk=D(pk^{\scriptscriptstyle*}, T_{\scriptscriptstyle qp})$. Then, it verifies the validity of the elements in $e$ and  $T$, with the help of $pk$. Also, it checks elements of $\bm{y}$ and ensures element of $\bm{y}_{\scriptscriptstyle \mathcal  C}, \bm{y}_{\scriptscriptstyle \mathcal  S},\bm{y}'_{\scriptscriptstyle \mathcal  C}, \bm{y}'_{\scriptscriptstyle \mathcal  S}\in \bm{y}$ have been set to $0$. If all checks are successful, then it encodes the amount of its coins  $coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal S}$ and sets $a=1$. Otherwise, it sets $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S}=\bot$ and $a=0$. It outputs $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S}$ and $a$. The smart contract is given $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S}$ coins and $a$.  

\


\item[$\bullet$] $\mathtt{RCPoRP}.\mathtt{genQuery}(1^\lambda, T_{\scriptscriptstyle qp})\rightarrow q_{\scriptscriptstyle j}$. A probabilistic algorithm run by the client. It takes as input  $1^\lambda$ and  encoding token $T_{\scriptscriptstyle qp}$.  It computes a query $q_{\scriptscriptstyle j}$. It outputs and sends $q_{\scriptscriptstyle j}$ to the contract. 



%\item[$\bullet$] $\mathtt{RCSP}.\mathtt{genQuery}(1^\lambda, \text{aux},k,Q, T_{\scriptscriptstyle qp}, enc)\rightarrow c^{\scriptscriptstyle *}_{\scriptscriptstyle j}$. A probabilistic algorithm run by the client. It takes as input  $1^\lambda$,  auxiliary information $\text{aux}$,  the key pair $k$,   query generator deterministic function $Q$, encoding token $T_{\scriptscriptstyle qp}$ and $enc:=(E,D)$.  It computes a pair $c_{\scriptscriptstyle j}$ containing a query vector $\bm{q}_{\scriptscriptstyle j}=Q( \text{aux},k)$,  and proof $\bm{w}_{\scriptscriptstyle q_{_{\scaleto{j}{\size}}}}$ proving the query is well-structured. It outputs the encoding of the pair, $c^{\scriptscriptstyle *}_{\scriptscriptstyle j}=E(c_{\scriptscriptstyle j},T_{\scriptscriptstyle qp})$. The output is sent to the smart contract. 

%\scaleto{c}{1pt}

%a set of (random) challenges $c$ or empty set if the proving/verification  algorithms do not require any challenges. %The challenges set is published to a bulletin board.
\


\item[$\bullet$] $\mathtt{RCPoRP}.\mathtt{prove}(u^{\scriptscriptstyle *},   q_{\scriptscriptstyle j},T_{\scriptscriptstyle qp},enc)\rightarrow (b_{\scriptscriptstyle j},m_{\scriptscriptstyle \mathcal{S},j},\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j})$. It is run by the server. It  takes as input the encoded service input $u^{\scriptscriptstyle *}$,     query $q_{\scriptscriptstyle j}$,    the encoding token $T_{\scriptscriptstyle qp}$, and $enc:=(E,D)$.   It checks the validity of  query $q_{\scriptscriptstyle j}$.  If it is rejected, then it sets $b_{\scriptscriptstyle j}=0$ and constructs a complaint $m_{\scriptscriptstyle \mathcal{S},j}$. Otherwise,  it   sets $b_{\scriptscriptstyle j}=1$ and $m_{\scriptscriptstyle \mathcal{S},j}=\bot$. It outputs $b_{\scriptscriptstyle j},m_{\scriptscriptstyle \mathcal{S},j}$,   and  encoded proof $\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j}=E(\pi_{\scriptscriptstyle j},T_{\scriptscriptstyle qp})$, where  $\pi_{\scriptscriptstyle j}$ contains $h_{\scriptscriptstyle j}=F(u^{\scriptscriptstyle *},q_{\scriptscriptstyle j},{pp'})$. Note,   $\pi_{\scriptscriptstyle j}$ may contain dummy values if $b_{\scriptscriptstyle j}=0$. The smart contract is given $\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j}$.



%\item[$\bullet$] $\mathtt{RCSP}.\mathtt{prove}(u^{\scriptscriptstyle *},  \sigma,  c^{\scriptscriptstyle *}_{\scriptscriptstyle j},pk^{\scriptscriptstyle *}, T_{\scriptscriptstyle qp},enc)\rightarrow (b_{\scriptscriptstyle j},m_{\scriptscriptstyle \mathcal{S},j},\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j})$. It is run by the server. It  takes as input the encoded service input $u^{\scriptscriptstyle *}$, metadata $\sigma$,   encoded query pair $c^{\scriptscriptstyle *}_{\scriptscriptstyle j}$, encoded public key $pk^{\scriptscriptstyle *}$,    the encoding token $T_{\scriptscriptstyle qp}$, and $enc:=(E,D)$.  It decodes the public key, $pk=D(pk^{\scriptscriptstyle *}, T_{\scriptscriptstyle qp})$. It checks the validity of decoded query, $c_{\scriptscriptstyle j}=D(c^{\scriptscriptstyle *}_{\scriptscriptstyle j},T_{\scriptscriptstyle qp})$.  If it is rejected, then it sets $b_{\scriptscriptstyle j}=0$ and constructs a complaint $m_{\scriptscriptstyle \mathcal{S},j}$. Otherwise,  it   sets $b_{\scriptscriptstyle j}=1$ and $m_{\scriptscriptstyle \mathcal{S},j}=\bot$. It outputs $b_{\scriptscriptstyle j},m_{\scriptscriptstyle \mathcal{S},j}$,   and  encoded proof $\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j}=E(\pi_{\scriptscriptstyle j},T_{\scriptscriptstyle qp})$, where  $\pi_{\scriptscriptstyle j}$ contains $h_{\scriptscriptstyle j}=F(u^{\scriptscriptstyle *},\bm{q}_{\scriptscriptstyle j})$ and a proof $\delta_{\scriptscriptstyle j}$  asserting the evaluation is performed correctly ($\pi_{\scriptscriptstyle j}$ may contain dummy values if $b_{\scriptscriptstyle j}=0$). The smart contract is given $\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j}$.


%with the help of decoded public key $pk=D(pk^{\scriptscriptstyle *}, T_{\scriptscriptstyle qp})$

\

\item[$\bullet$] $\mathtt{RCPoRP}.\mathtt{verify}(\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j}, {q}_{\scriptscriptstyle j},T_{\scriptscriptstyle qp},enc)\rightarrow (d_{\scriptscriptstyle j},m_{\scriptscriptstyle \mathcal{C},j})$. A deterministic algorithm run by the client. It takes as input the encoded proof $\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j}$,  query  ${q}_{\scriptscriptstyle j}$,   the encoding token $T_{\scriptscriptstyle qp}$ and $enc:=(E,D)$. If the decoded proof $\pi_{\scriptscriptstyle j}=D(\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j},T_{\scriptscriptstyle qp})$ is rejected,  it outputs $d_{\scriptscriptstyle j}=0$ and a complaint $m_{\scriptscriptstyle \mathcal{C},j}$. Otherwise, it outputs  $d_{\scriptscriptstyle j}=1$ and $m_{\scriptscriptstyle \mathcal{C},j}=\bot$.




%, where $k=pk$  in the case where $\mathtt{VS.verify}()$ is publicly verifiable, or $k:(sk,pk)$ when it is privately verifiable

\


\item[$\bullet$] $\mathtt{RCPoRP}.\mathtt{resolve}(m_{\scriptscriptstyle \mathcal{C}},m_{\scriptscriptstyle \mathcal{S}},z, {\bm{\pi}}^{\scriptscriptstyle *}, {\bm{q}}, T_{\scriptscriptstyle qp},enc)\rightarrow \bm{y}$. It is run by the contract. It takes as input the client's complaints $m_{\scriptscriptstyle \mathcal{C}}$, the server's complaints $m_{\scriptscriptstyle \mathcal{S}}$, the total number of verifications $z$, all encoded proofs $ {\bm{\pi}}^{\scriptscriptstyle *}$, all queries  $ {\bm{q}}$,   encoding token $T_{\scriptscriptstyle qp}$, and $enc:=(E,D)$. It verifies the token,  queries, and proofs.  It reads the  binary vectors $[\bm{y}_{\scriptscriptstyle \mathcal  C}, \bm{y}_{\scriptscriptstyle \mathcal  S}]$ from its internal state. It  updates $\bm{y}_{\scriptscriptstyle \mathcal E}$ by setting an element of it to one, i.e., $y_{\scriptscriptstyle \mathcal E,j}=1$, if party $\mathcal{E}\in\{\mathcal{C},\mathcal{S}\}$ has misbehaved in the $j$-th verification (i.e., provided invalid query or service proof).  




%\item[$\bullet$] $\mathtt{RCSP}.\mathtt{resolve}(m_{\scriptscriptstyle \mathcal{C}},m_{\scriptscriptstyle \mathcal{S}},z, {\bm{\pi}}^{\scriptscriptstyle *}, {\bm{c}}^{\scriptscriptstyle *},pk^{\scriptscriptstyle*}, T_{\scriptscriptstyle qp},enc)\rightarrow \bm{y}$. It is run by the arbiter. It takes as input the client's complaints $m_{\scriptscriptstyle \mathcal{C}}$, the server's complaints $m_{\scriptscriptstyle \mathcal{S}}$, the total number of verifications $z$, all encoded proofs $ {\bm{\pi}}^{\scriptscriptstyle *}$, all encoded query pairs $ {\bm{c}}^{\scriptscriptstyle *}$, encoded public key $pk^{\scriptscriptstyle *}$, encoding token $T_{\scriptscriptstyle qp}$, and $enc:=(E,D)$. It decodes the public key. It verifies the token, decoded queries, and proofs.  It reads the  binary vectors $[\bm{y}_{\scriptscriptstyle \mathcal  C}, \bm{y}_{\scriptscriptstyle \mathcal  S},\bm{y}'_{\scriptscriptstyle \mathcal  C}, \bm{y}'_{\scriptscriptstyle \mathcal  S}]$ from the smart contract. It  updates $\bm{y}_{\scriptscriptstyle \mathcal E}$ by setting an element of it to one, i.e., $y_{\scriptscriptstyle \mathcal E,j}=1$, if party $\mathcal{E}\in\{\mathcal{C},\mathcal{S}\}$ has misbehaved in the $j$-th verification (i.e., provided invalid query or service proof). It also updates $\bm{y}'_{\scriptscriptstyle \mathcal E}$ if party $\mathcal{E}$ has provided a complain that does not allow it to identify a misbehaved party, in $j$-th verification. 


%\item[$\bullet$] $\mathtt{RCSP}.\mathtt{resolve}(m_{\scriptscriptstyle \mathcal{C}},m_{\scriptscriptstyle \mathcal{S}},z, {\bm{\pi}}^{\scriptscriptstyle *}, {\bm{c}}^{\scriptscriptstyle *},pk,E^{\scriptscriptstyle -1}_{\scriptscriptstyle 2},t_{\scriptscriptstyle qp},a)\rightarrow (y_{\scriptscriptstyle \mathcal C},y_{\scriptscriptstyle \mathcal S})$. It is run by the arbiter. It takes client's complaint $m_{\scriptscriptstyle \mathcal{C}}$,   server's complaints   $m_{\scriptscriptstyle \mathcal{S}}$, total number of verifications $z$, all encoded proofs $ {\bm{\pi}}^{\scriptscriptstyle *}$, all encoded queries $ {\bm{c}}^{\scriptscriptstyle *}$, public key $pk$, decoding function $E^{\scriptscriptstyle -1}_{\scriptscriptstyle 2}$, encoding token $t_{\scriptscriptstyle qp}$ and  $a$.  It proceeds only if $a=1$. It verifies the token,   decoded queries, and proofs.  It outputs total number of times the client and server misbehaved, i.e. $y_{\scriptscriptstyle \mathcal C}$ and $y_{\scriptscriptstyle \mathcal S}$ respectively. 

\
	
	
\item[$\bullet$] $\mathtt{RCPoRP}.\mathtt{pay}(\bm{y},T_{\scriptscriptstyle cp},a,p_{\scriptscriptstyle\mathcal S}, coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C},coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S})\rightarrow ({\bm{coin}}_{\scriptscriptstyle\mathcal C},{\bm{coin}}_{\scriptscriptstyle\mathcal S})$. It is run by the smart contract. It takes as input the binary vectors $[\bm{y}_{\scriptscriptstyle \mathcal  C}, \bm{y}_{\scriptscriptstyle \mathcal  S}]\in \bm{y}$ that indicate which party misbehaved,  coins' token $T_{\scriptscriptstyle cp}:=\{cp,g_{\scriptscriptstyle cp}\}$, the output of the checks that server-side initiation algorithm  performed $a$, the total coins the server should deposit $p_{\scriptscriptstyle\mathcal S}$, and the total coins amount the client and server  deposited, i.e. $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C}$ and $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S}$ respectively. If $a=1$ and  $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S}= p_{\scriptscriptstyle\mathcal S}$, then it verifies the validity of $T_{\scriptscriptstyle cp}$. If $T_{\scriptscriptstyle cp}$ is rejected, then it aborts. 
If it is accepted, then it constructs  vector ${\bm{coin}}_{\scriptscriptstyle\mathcal I}$, where $\mathcal{E}\in\{\mathcal{C},\mathcal{S}\}$. It sends ${{coin}}_{\scriptscriptstyle\mathcal{I},j}\in{\bm{coin}}_{\scriptscriptstyle\mathcal I}$ coins to party $\mathcal{I}$ for each $j$-th verification. Otherwise (i.e. $a=0$ or $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S}\neq p_{\scriptscriptstyle\mathcal S}$)  it  sends $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C}$ and $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S}$ coins to $\mathcal C$ and $\mathcal S$ respectively. 	
	
	
	
%\item[$\bullet$] $\mathtt{RCSP}.\mathtt{pay}(\bm{y},T_{\scriptscriptstyle cp},a,p_{\scriptscriptstyle\mathcal S}, coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C},coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S})\rightarrow ({\bm{coin}}_{\scriptscriptstyle\mathcal C},{\bm{coin}}_{\scriptscriptstyle\mathcal S},{\bm{coin}}_{\scriptscriptstyle\mathcal Ar})$. It is run by the smart contract and can be invoked by the client or server. It takes as input the binary vectors $[\bm{y}_{\scriptscriptstyle \mathcal  C}, \bm{y}_{\scriptscriptstyle \mathcal  S},\bm{y}'_{\scriptscriptstyle \mathcal  C}, \bm{y}'_{\scriptscriptstyle \mathcal  S}]\in \bm{y}$ that indicate which party misbehaved, or sent invalid complaint  in each verification,  coins' token $T_{\scriptscriptstyle cp}:=\{cp,g_{\scriptscriptstyle cp}\}$, the output of the checks that server-side initiation algorithm  perfomed $a$, the total coins the server should deposit $p_{\scriptscriptstyle\mathcal S}$, and the total coins amount the client and server  deposited, i.e. $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C}$ and $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S}$ respectively. If $a=1$ and  $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S}= p_{\scriptscriptstyle\mathcal S}$, then it verifies the validity of $T_{\scriptscriptstyle cp}$. If $T_{\scriptscriptstyle cp}$ is rejected, then it aborts. 
%If it is accepted, then it constructs  vector ${\bm{coin}}_{\scriptscriptstyle\mathcal I}$, where $\mathcal{I}\in\{\mathcal{C},\mathcal{S},\mathcal{A}r\}$; It sends ${{coin}}_{\scriptscriptstyle\mathcal{I},j}\in{\bm{coin}}_{\scriptscriptstyle\mathcal I}$ coins to party $\mathcal{I}$ for each $j$-th verification. Otherwise (i.e. $a=0$ or $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S}\neq p_{\scriptscriptstyle\mathcal S}$)  it only sends $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C}$ to $\mathcal C$. 

%sets $coin_{\scriptscriptstyle\mathcal C,0}=coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C}, \bm{coin}_{\scriptscriptstyle\mathcal S}=\bot$, and $\bm{coin}_{\scriptscriptstyle\mathcal Ar}=\bot$.  %It outputs ${\bm{coin}}_{\scriptscriptstyle\mathcal C},{\bm{coin}}_{\scriptscriptstyle\mathcal S}$, and ${\bm{coin}}_{\scriptscriptstyle\mathcal Ar}$

%sends $coin_{\scriptscriptstyle\mathcal C}, coin_{\scriptscriptstyle\mathcal S}$, and $coin_{\scriptscriptstyle\mathcal Ar}$ coins to the client, server, and arbiter respectively. Otherwise, it does nothing. 

\end{itemize}
\end{definition}

Similar to RC-S-P definition, in the above definition, algorithms $\mathtt{RCPoRP}.\mathtt{genQuery}(.),\mathtt{RCPoRP}.\mathtt{prove}(.),\mathtt{RCPoRP}.\mathtt{verify}(.)$ and $\mathtt{RCPoRP}.\mathtt{resolve}(.)$ implicitly  take $a, coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal{S}}, p_{\scriptscriptstyle\mathcal{S}}$ as another inputs and  execute only if $a=1$ and $coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal{S}}=p_{\scriptscriptstyle\mathcal{S}}$; however, for the sake of simplicity we  avoided explicitly stating it  in the definition. 

A recurring contingent service payment (RC-S-P)  scheme satisfies correctness and security. At a high level, correctness requires that by the end of the protocol's execution  (that involves  honest client and server) the client receives all $z$ valid service proofs while the server gets paid  for the proofs, without the involvement of the arbiter. More specifically, it requires that the server accepts an honest client's encoded data and query while the honest client accepts the server's valid service proof (and no one is identified as misbehaving party). Moreover, the honest client gets back all its deposited coins minus the service payment, the honest server gets back all its deposited coins  plus the service payment and the arbiter receives nothing. It is formally stated as below.



\begin{definition}[RC-S-P Correctness] A recurring contingent service payment  scheme  is  correct   if for any functions $F, Q, M, E, D$, any price list $pl$, and any auxiliary information $\text{aux}_{\scriptscriptstyle 1},...,\text{aux}_{\scriptscriptstyle z}$, the key generation algorithm produces keys $\mathtt{RCSP}.\mathtt{keyGen}(1^\lambda, F)\rightarrow \bm{k}$,   such that for any service input $u$, if $\mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, M,z,pl,enc) \rightarrow (u^{\scriptscriptstyle *},e,T, p_{\scriptscriptstyle\mathcal S},  \bm{y}, coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C})$,  $\mathtt{RCSP}.\mathtt{sInit} (u^{\scriptscriptstyle *},e, pk,z, T, p_{\scriptscriptstyle\mathcal S},\bm{y},enc)\rightarrow (coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S},a)$,   $\forall j:\Big($$\mathtt{RCSP}.\mathtt{genQuery}(1^\lambda, \text{aux}_{\scriptscriptstyle j},k,\\Q, T_{\scriptscriptstyle qp}, enc)\rightarrow c^{\scriptscriptstyle *}_{\scriptscriptstyle j}$, $\mathtt{RCSP}.\mathtt{prove}(u^{\scriptscriptstyle *},  \sigma,  c^{\scriptscriptstyle *}_{\scriptscriptstyle j},pk, T_{\scriptscriptstyle qp},enc)\rightarrow (b_{\scriptscriptstyle j},m_{\scriptscriptstyle\mathcal {S},j},\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j})$, $\mathtt{RCSP}.\mathtt{verify}(\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j}, \bm{q}_{\scriptscriptstyle j},k,T_{\scriptscriptstyle qp},enc)\rightarrow (d_{\scriptscriptstyle j}, m_{\scriptscriptstyle\mathcal {C},j})$$\Big),\\ \mathtt{RCSP}.\mathtt{resolve}(m_{\scriptscriptstyle \mathcal{C}},m_{\scriptscriptstyle \mathcal{S}},z, {\bm{\pi}}^{\scriptscriptstyle *}, {\bm{c}}^{\scriptscriptstyle *},pk, T_{\scriptscriptstyle qp},enc)\rightarrow \bm{y}$, $\mathtt{RCSP}.\mathtt{pay}(\bm{y},T_{\scriptscriptstyle cp},a,p_{\scriptscriptstyle\mathcal S}, coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C},coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S})\rightarrow (\bm{coin}_{\scriptscriptstyle\mathcal C},\bm{coin}_{\scriptscriptstyle\mathcal S},\bm{coin}_{\scriptscriptstyle\mathcal Ar})$, then $(a=1)\wedge (\bigwedge\limits^{\scriptscriptstyle z}_{\scriptscriptstyle j=1} b_{\scriptscriptstyle j}= \bigwedge\limits^{\scriptscriptstyle z}_{\scriptscriptstyle j=1} d_{\scriptscriptstyle j}=1)\wedge (\bm{y}_{\scriptscriptstyle \mathcal C}=\bm{y}_{\scriptscriptstyle \mathcal S}=\bm{y}'_{\scriptscriptstyle \mathcal C}=\bm{y}'_{\scriptscriptstyle \mathcal S}=0) \wedge (\sum\limits^{\scriptscriptstyle z}_{\scriptscriptstyle j=1}coin_{\scriptscriptstyle\mathcal C,j}=coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C}-o\cdot z) \wedge  (\sum\limits^{\scriptscriptstyle z}_{\scriptscriptstyle j=1}coin_{\scriptscriptstyle\mathcal S,j}=coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S}+o\cdot z)  \wedge (\sum\limits^{\scriptscriptstyle z}_{\scriptscriptstyle j=1}coin_{\scriptscriptstyle\mathcal Ar,j}=0)$, where $\bm{y}_{\scriptscriptstyle \mathcal C},\bm{y}_{\scriptscriptstyle \mathcal S},\bm{y}'_{\scriptscriptstyle \mathcal C},\bm{y}'_{\scriptscriptstyle \mathcal S}\in \bm{y}$
\end{definition}

%\textcolor{blue}{XXXX Thomas: something is not right in the definition of correctness... we write $\forall j$ but the execution of $\mathtt{RCSP}.\mathtt{genQuery}$ does not depend on $j$. Not sure how to fix it yet.XXXX}

A RC-S-P scheme is said to be secure if it satisfies  three main properties: (a)  security against malicious server, (b) security against malicious client, and (c) privacy.  In the following, we formally define each of them.

 Intuitively, security against a malicious server states that (at the end of the protocol execution) either (i) for each verification the client gets a valid proof and gets back its deposit minus the service payment, or (ii) the client gets its deposit back (for $j$-th verification) and the arbiter receives $l$ coins, or (iii) if it unnecessarily invokes the arbiter, then it has to pay the arbiter. In particular, for each $j$-th verification, the security requires that only with a negligible probability the adversary wins, if it  provides either (a)  correct evaluation of the function on the service input but it either makes the client  withdraw an incorrect amount of coins (i.e. something other than its deposit minus service payment) or makes the arbiter withdraw incorrect amount of coins if it unnecessarily invokes the arbiter, or (b) incorrect evaluation of the function on the service input,  but either persuades the client or the arbiter to accept it (i.e.,  $b_{\scriptscriptstyle j}=1$ or $y_{\scriptscriptstyle\mathcal S,j}=0$) or makes them  withdraw incorrect amount of coins (i.e., $coin_{\scriptscriptstyle\mathcal{C},j}\neq \frac{coin_{\scriptscriptstyle\mathcal C}^{\scriptscriptstyle*}}{z}$ or  $coin_{\scriptscriptstyle\mathcal{A}r,j}\neq l$ coins).  Below, we formalize this intuition. 




%Intuitively, security against a malicious server states that (at the end of the protocol execution) either the client for each verification gets a valid proof or the client gets its coins back (for $j$-th verification) and the arbiter receives $l$ coins. In other words, for each  $j$-th verification, the adversary wins if it provides incorrect evaluation of the function on the service input,  but (with a high probability) either persuades the client or the arbiter to accept it (i.e.  $b_{\scriptscriptstyle j}=1$ or $y_{\scriptscriptstyle\mathcal S}[j]=0$) or makes them to withdraw incorrect amount of coins (i.e. $coin_{\scriptscriptstyle\mathcal{C},j}\neq \frac{coin_{\scriptscriptstyle\mathcal C}^{\scriptscriptstyle*}}{z}$ and  $coin_{\scriptscriptstyle\mathcal{A}r,j}\neq l$ coins).  Below, we formalize this intuition with an experiment, $\textbf{Exp}^{\scriptscriptstyle(1)}_{\scriptscriptstyle\mathcal {A}}[]$: 


%
%\small{
%$$
%    \begin{array}{l}
%    \mathtt{RCSP.keyGen}(1^{\lambda},F)\rightarrow \bm{k}\\
%    \mathcal{A}(1^\lambda,pk, F)\rightarrow (u,\text{state})\\
%    \mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, M,z,cp)\rightarrow (u^{\scriptscriptstyle *},e,t,coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C})\\
%    \mathcal{A}(u^{\scriptscriptstyle *},e, pk,z, t)\rightarrow (coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S},a)\\
%	\mathtt{RCSP}.\mathtt{genQuery}(1^{\lambda}, \text{aux},k,Q,j, en)\rightarrow c^{\scriptscriptstyle *}_{\scriptscriptstyle j}\\
%	
%     \mathcal{A}(\text{state},c^{\scriptscriptstyle *}_{\scriptscriptstyle j},\sigma, u^{\scriptscriptstyle *},j,en,a)\rightarrow 
%     (b_{\scriptscriptstyle j},m_{\scriptscriptstyle \mathcal{A},j},y^{\scriptscriptstyle *}_{\scriptscriptstyle j},\delta^{\scriptscriptstyle *}_{\scriptscriptstyle j})\\ 
%   \mathtt{RCSP}.\mathtt{verify}(\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j}, q,k,j,en)\rightarrow (d_{\scriptscriptstyle j},m_{\scriptscriptstyle \mathcal{C},j})\\
%   \mathtt{RCSP}.\mathtt{resolve}(\bm{m}_{\scriptscriptstyle \mathcal{C}},\bm{m}_{\scriptscriptstyle \mathcal{A}},z, {\bm{\pi}}^{\scriptscriptstyle *}, {\bm{c}}^{\scriptscriptstyle *},pk,en)\rightarrow (y_{\scriptscriptstyle \mathcal C},y_{\scriptscriptstyle \mathcal S})\\
%   \mathtt{RCSP}.\mathtt{pay}(y_{\scriptscriptstyle \mathcal C},y_{\scriptscriptstyle \mathcal S},t_{\scriptscriptstyle cp})\rightarrow ({\bm{coin}}_{\scriptscriptstyle\mathcal C},{\bm{coin}}_{\scriptscriptstyle\mathcal S},{\bm{coin}}_{\scriptscriptstyle\mathcal Ar})\\
%\end{array}$$
%}
%
%
%
%The output of the experiment is $1$, i.e. $\textit{\textbf{Exp}}^{\scriptscriptstyle(1)}_{\scriptscriptstyle\mathcal {A},\text{RC-S-P}}()=1$, if the adversary wins. 
%
%\begin{definition}[RC-S-P Security Against Malicious Server]\label{deff::}  A RC-S-P  is secure against a malicious server  for a function $F$, if for any security parameter $\lambda$, any auxiliary information $aux$, any $Q$ and any probabilistic polynomial time adversary $\mathcal{A}$, there exists a negligible function $\mu(.)$, such that: 
%%\footnotesize{
%
%$$Pr[\textbf{Exp}^{\scriptscriptstyle(1)}_{\scriptscriptstyle\mathcal {A},\text{RC-S-P}}()=1]=Pr\left[
%\begin{array}{l}
%\left((F_{\scriptscriptstyle q}(u^{\scriptscriptstyle *})= y_{\scriptscriptstyle j}\ \wedge coin_{\scriptscriptstyle\mathcal{C},j}\neq  \frac{coin_{\scriptscriptstyle\mathcal C}^{\scriptscriptstyle*}}{z}-o\right)
% \vee\\
%  \left(F_{\scriptscriptstyle q}(u^{\scriptscriptstyle *})\neq y_{\scriptscriptstyle j}\ \wedge (d_{\scriptscriptstyle j}=1	\vee y_{\scriptscriptstyle \mathcal S}[j]=0 \ \vee coin_{\scriptscriptstyle\mathcal{C},j}\neq \frac{coin_{\scriptscriptstyle\mathcal C}^{\scriptscriptstyle*}}{z} \ \wedge coin_{\scriptscriptstyle\mathcal{A}r,j}\neq l)\right)\end{array}\right]\leq \mu(\lambda)$$
%\end{definition}



%_{\scriptscriptstyle q_{_{\scaleto{j}{\size}}}}


\begin{definition}[RC-S-P Security Against Malicious Server]\label{deff::RC-S-P-SecurityAgainstMaliciousServerxx}  A RC-PoR-P  is secure against a malicious server  for a function $F$, if for  any price list $pl$, every $j$ (where $1\leq j\leq z$), and any PPT adversary $\mathcal{A}$, there exists a negligible function $\mu(\cdot)$, such that for any security parameter $\lambda$: 
%\footnotesize{
{\small
$$ \Pr\left[
  \begin{array}{l}
  \Big(F(u^{\scriptscriptstyle *}, \bm{q}_{\scriptscriptstyle j}, {pp})= h_{\scriptscriptstyle j}\ \wedge (coin_{\scriptscriptstyle\mathcal{C},j}\neq  \frac{coin_{\scriptscriptstyle\mathcal C}^{\scriptscriptstyle*}}{z}-o)\Big)\ \vee\\ 

\Big(
F(u^{\scriptscriptstyle *},\bm{q}_{\scriptscriptstyle j}, {pp})\neq h_{\scriptscriptstyle j} \ \wedge (d_{\scriptscriptstyle j}=1	\vee y_{\scriptscriptstyle \mathcal{S},j}=0 \ \vee \\coin_{\scriptscriptstyle\mathcal{C},j}\neq \frac{coin_{\scriptscriptstyle\mathcal C}^{\scriptscriptstyle*}}{z}+l) \Big)\\
%\text{s.t.}\\
%y_{\scriptscriptstyle j}= E^{\scriptscriptstyle -1}_{\scriptscriptstyle 2}(y^{\scriptscriptstyle *}_{\scriptscriptstyle j},t_{\scriptscriptstyle qp})\\
%E^{\scriptscriptstyle -1}_{\scriptscriptstyle 2},t_{\scriptscriptstyle qp}\in en\\
\end{array} \middle |
    \begin{array}{l}
    \mathtt{RCPoRP.keyGen}(1^{\lambda})\rightarrow \bm{k}\\
    \mathcal{A}(1^\lambda,pk)\rightarrow u\\
  
   \mathtt{RCPoRP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, z,pl)\rightarrow (u^{\scriptscriptstyle *},T, p_{\scriptscriptstyle\mathcal S},  \bm{y}, coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C})\\
    
    \mathcal{A}(u^{\scriptscriptstyle *},  pk, z, T, p_{\scriptscriptstyle\mathcal S},\bm{y})\rightarrow (coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S},a)\\
	\mathtt{RCPoRP}.\mathtt{genQuery}(1^\lambda,  T_{\scriptscriptstyle qp})\rightarrow q_{\scriptscriptstyle j}\\
	
     \mathcal{A}( u^{\scriptscriptstyle *}, q_{\scriptscriptstyle j}, a)\rightarrow 
     (b_{\scriptscriptstyle j},m_{\scriptscriptstyle \mathcal{S},j},\bm{\pi}^{\scriptscriptstyle *}_{\scriptscriptstyle j})\\
     
     %(\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j},b_{\scriptscriptstyle j})\\
     
\mathtt{RCPoRP}.\mathtt{verify}(\bm{\pi}^{\scriptscriptstyle *}_{\scriptscriptstyle j}, {q}_{\scriptscriptstyle j},T_{\scriptscriptstyle qp})\rightarrow (d_{\scriptscriptstyle j},m_{\scriptscriptstyle \mathcal{C},j})\\
  \mathtt{resolve}(m_{\scriptscriptstyle \mathcal{C}},m_{\scriptscriptstyle \mathcal{S}}, z, {\bm{\pi}}^{\scriptscriptstyle *}, {\bm{q}},  T_{\scriptscriptstyle qp})\rightarrow \bm{y}\\
   
   \mathtt{RCPoRP}.\mathtt{pay}(\bm{y},T_{\scriptscriptstyle cp},a,p_{\scriptscriptstyle\mathcal S}, coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C},coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S})\rightarrow ({\bm{coin}}_{\scriptscriptstyle\mathcal C},{\bm{coin}}_{\scriptscriptstyle\mathcal S})\\
\end{array}    \right]\leq \mu(\lambda).$$
}
where $h_{\scriptscriptstyle j}= D(h^{\scriptscriptstyle *}_{\scriptscriptstyle j},T_{\scriptscriptstyle qp})$, $
D\in enc$, $\sigma\in e$, $m_{\scriptscriptstyle \mathcal{C},j}\in m_{\scriptscriptstyle \mathcal{C}}, m_{\scriptscriptstyle \mathcal{S},j}\in m_{\scriptscriptstyle \mathcal{S}}$,   $y_{\scriptscriptstyle \mathcal{S},j}\in \bm{y}_{\scriptscriptstyle \mathcal{S}}\in\bm{y}$, and $ {pp}\in T_{\scriptscriptstyle qp}$. 



%\textcolor{blue}{XXXX Thomas: We never define what $m_{\scriptscriptstyle \mathcal{A}}$ is. The $\mathtt{RCSP}.\mathtt{resolve}$ algorithm takes as input $m_{\scriptscriptstyle \mathcal{C}},m_{\scriptscriptstyle \mathcal{S}}$, not $m_{\scriptscriptstyle \mathcal{C}},m_{\scriptscriptstyle \mathcal{A}}$. One extra question is: how is $m_{\scriptscriptstyle \mathcal{S}}$ created in the experiment? --> Aydin--addressed} 


%Also, the probability is taken over uniform  choice of $k,k'\stackrel{\scriptscriptstyle\$}\leftarrow \{0,1\}^{\scriptscriptstyle\lambda}$, where $k,k'\in\bm{k}$, as well as the randomness of $\mathcal{A}$ and the randomness used in witnesses $g_{\scriptscriptstyle cp},g_{\scriptscriptstyle qp}\in t$.
\end{definition}




%\begin{definition}[RC-S-P Correctness] A recurring contingent service payment  scheme  is  correct   if for any function $F$, the key generation algorithm produces keys $\mathtt{RCSP}.\mathtt{keyGen}(1^\lambda,F)\rightarrow (k,k')$,   such that $\forall u \in \mathtt{Domain}(F)$ if $\mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,k,k', M,z,o,l,E_{\scriptscriptstyle 1}) \rightarrow (u^{\scriptscriptstyle *}, e, t, coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C})$, $\mathtt{RCSP}.\mathtt{sInit} (u^{\scriptscriptstyle *}, e, pk, z, t, E_{\scriptscriptstyle 1})\rightarrow (coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S}, a)$, \ \\ $\mathtt{RCSP}.\mathtt{genQuery}(1^{\lambda}, \text{aux}, k, Q, j, E_{\scriptscriptstyle 2}, qp, a)\rightarrow c^{\scriptscriptstyle *}_{\scriptscriptstyle j}$, $\mathtt{RCSP}.\mathtt{prove}(u^{\scriptscriptstyle *},  \sigma, c^{\scriptscriptstyle *}_{\scriptscriptstyle j}, pk, j, E^{\scriptscriptstyle -1}_{\scriptscriptstyle 2},qp,a)\rightarrow (\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j}, b_{\scriptscriptstyle j})$, \\$\mathtt{RCSP}.\mathtt{verify}(\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j}, q,k,j,E^{\scriptscriptstyle -1}_{\scriptscriptstyle 2},qp,a)\rightarrow d_{\scriptscriptstyle j}$, $\mathtt{RCSP}.\mathtt{resolve}(m_{\scriptscriptstyle \mathcal{C}},m_{\scriptscriptstyle \mathcal{S}},z, {\bm{\pi}}^{\scriptscriptstyle *}, {\bm{c}}^{\scriptscriptstyle *},pk,E^{\scriptscriptstyle -1}_{\scriptscriptstyle 2},t_{\scriptscriptstyle qp},a)\rightarrow (y_{\scriptscriptstyle \mathcal C},y_{\scriptscriptstyle \mathcal S})$, \\$\mathtt{RCSP}.\mathtt{pay}(y_{\scriptscriptstyle \mathcal C},y_{\scriptscriptstyle \mathcal S},t_{\scriptscriptstyle cp},a)\rightarrow (coin_{\scriptscriptstyle\mathcal C},coin_{\scriptscriptstyle\mathcal S},coin_{\scriptscriptstyle\mathcal Ar})$, s.t. $a=1\wedge (\bigwedge\limits^{\scriptscriptstyle z}_{\scriptscriptstyle j=1} b_{\scriptscriptstyle j}= \bigwedge\limits^{\scriptscriptstyle z}_{\scriptscriptstyle j=1} d_{\scriptscriptstyle j}=1)\wedge (y_{\scriptscriptstyle \mathcal C}=y_{\scriptscriptstyle \mathcal S}=0) \wedge (coin_{\scriptscriptstyle\mathcal C}=coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C}-oz) \wedge  (coin_{\scriptscriptstyle\mathcal S}=coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S}+oz)   \wedge (coin_{\scriptscriptstyle\mathcal Ar}=0) $
%\end{definition}

 
 
 
 
Informally, security against a malicious client requires that, for each  $j$-th verification, a malicious client with a negligible probability  wins if it provides either (a) valid metadata and query but either makes the server receive incorrect amount of coins (something other than its deposit plus the service payment), or makes the arbiter withdraw incorrect amount of coins if it unnecessarily invokes the arbiter,  or (b) invalid metadata or query but convinces the server to accept either of them (i.e. the invalid metadata or query), or (c) invalid query but persuades the arbiter to accept it, or  makes them withdraw an incorrect amount of coins (i.e. $coin_{\scriptscriptstyle\mathcal{S},j}\neq \frac{coin_{\scriptscriptstyle\mathcal S}^{\scriptscriptstyle*}}{z}+o$ or  $coin_{\scriptscriptstyle\mathcal{A}r,j}\neq l$ coins). Below, we formally state the property. 
 
 %\textcolor{blue}{XXXX Thomas: what does ``them'' refer to? XXXX}--> Aydin: the invalid metadata or query
 
 
 \begin{definition}[RC-S-P Security Against Malicious Client]\label{deff::RC-S-P-Security-Against Malicious-Clientxxx}  A RC-S-P  is secure against a malicious client  for a function $F$, for every $j$ (where $1\leq j\leq z$), any $Q,M,E,D$ and any probabilistic polynomial time adversary $\mathcal{A}$, there exists a negligible function $\mu(\cdot)$, such that for any security parameter $\lambda$: 


{\small
$$ \Pr\left[
  \begin{array}{l}
 \Big((M(u^{\scriptscriptstyle *},k, {pp})= \sigma  \wedge Q(\text{aux},k, {pp})= \bm{q}_{\scriptscriptstyle j})\ \wedge\\
  (coin_{\scriptscriptstyle\mathcal{S},j}\neq  \frac{coin_{\scriptscriptstyle\mathcal S}^{\scriptscriptstyle*}}{z}+o) \Big)\ \vee
  \\
  
  
  \Big(M(u^{\scriptscriptstyle *}, k,  {pp})\neq \sigma \wedge a=1\Big) \ \vee\\ 


  \Big(Q(\text{aux},k,  {pp})\neq \bm{q}_{\scriptscriptstyle j}\ \wedge
  (b_{\scriptscriptstyle j}=1 \ \vee \ y_{\scriptscriptstyle\mathcal{C},j}=0 \ \vee \\ coin_{\scriptscriptstyle\mathcal{S},j}\neq \frac{coin_{\scriptscriptstyle\mathcal S}^{\scriptscriptstyle*}}{z}+o+l)\Big)
 \\
 
\end{array} \middle |
    \begin{array}{l}
   \mathcal{A}(1^{\lambda}, F)\rightarrow (u^{\scriptscriptstyle *},z,\bm{k},e,T, pl, p_{\scriptscriptstyle\mathcal{S}}, coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C},enc, \text{aux},\bm{y}, enc, pk)\\
   
   \mathtt{RCSP}.\mathtt{sInit}(u^{\scriptscriptstyle *}, e, pk, z, T, p_{\scriptscriptstyle\mathcal S},\bm{y},enc)\rightarrow (coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S},a)\\
   
	\mathcal{A}(coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S},a, 1^\lambda, \text{aux},k,Q, T_{\scriptscriptstyle qp}, enc)\rightarrow c^{\scriptscriptstyle *}_{\scriptscriptstyle j}\\

     \mathtt{RCSP}.\mathtt{prove}(u^{\scriptscriptstyle *},  \sigma,  c^{\scriptscriptstyle *}_{\scriptscriptstyle j}, pk, T_{\scriptscriptstyle qp},enc)\rightarrow (b_{\scriptscriptstyle j},m_{\scriptscriptstyle \mathcal{S},j},\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j})\\
     
 \mathcal{A}(\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j}, \bm{q}_{\scriptscriptstyle j},k,T_{\scriptscriptstyle qp},enc)\rightarrow (d_{\scriptscriptstyle j},m_{\scriptscriptstyle \mathcal{S},j})\\
   
   
   \mathtt{RCSP}.\mathtt{resolve}(m_{\scriptscriptstyle \mathcal{C}},m_{\scriptscriptstyle \mathcal{S}},z, {\bm{\pi}}^{\scriptscriptstyle *}, {\bm{c}}^{\scriptscriptstyle *}, pk, T_{\scriptscriptstyle qp},enc)\rightarrow \bm{y}\\
   \mathtt{RCSP}.\mathtt{pay}(\bm{y},T_{\scriptscriptstyle cp},a,p_{\scriptscriptstyle\mathcal S}, coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C},coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S})\rightarrow ({\bm{coin}}_{\scriptscriptstyle\mathcal C},{\bm{coin}}_{\scriptscriptstyle\mathcal S})\\
\end{array}    \right]\leq \mu(\lambda).$$
}
where $\bm{q}_{\scriptscriptstyle j}\in D(c^{\scriptscriptstyle *}_{\scriptscriptstyle j},t_{\scriptscriptstyle qp})$, $
D\in enc$, $\sigma\in e$, $y'_{\scriptscriptstyle \mathcal{C},j}\in \bm{y}'_{\scriptscriptstyle \mathcal{C}}\in\bm{y}$,   $y_{\scriptscriptstyle \mathcal{C},j}\in \bm{y}_{\scriptscriptstyle \mathcal{C}}\in\bm{y}$, and ${pp}\in T_{\scriptscriptstyle qp}$.  
\textcolor{blue}{XXXX Thomas: again here, the coins amount is fixed to $o$. Also I have not understood what is the meaning and use of $\bm{y}'_{\scriptscriptstyle \mathcal{C}},\bm{y}'_{\scriptscriptstyle \mathcal{S}}$ XXXX}
%Moreover,  the probability is taken over the randomness used in witnesses $g_{\scriptscriptstyle cp},g_{\scriptscriptstyle qp}\in t$ as well as  the randomness used in proofs $\bm{w}_{\scriptscriptstyle q_{_{\scaleto{j}{\size}}}}\in c_{\scriptscriptstyle j}$ and $w_{\scriptscriptstyle\sigma}\in e$ and  the randomness of $\mathcal{A}$.
\end{definition}
 










%\small{
%$$ Pr\left[
%  \begin{array}{l}
% \Big((M(u^{\scriptscriptstyle *},k)= \sigma  \wedge Q(\text{aux},k)= q_{\scriptscriptstyle j}) \wedge\\
%  (coin_{\scriptscriptstyle\mathcal{S},j}\neq  \frac{coin_{\scriptscriptstyle\mathcal S}^{\scriptscriptstyle*}}{z}+o)\Big) \vee
%  \\
%  \Big((M(u^{\scriptscriptstyle *},k)\neq \sigma \lor Q(\text{aux},k)\neq q_{\scriptscriptstyle j}) \wedge\\
%  (a=1 \ \vee b_{\scriptscriptstyle j}=1\ \vee y_{\scriptscriptstyle\mathcal{C}}[j]=0 \ \vee \\ coin_{\scriptscriptstyle\mathcal{S},j}\neq \frac{coin_{\scriptscriptstyle\mathcal S}^{\scriptscriptstyle*}}{z}+o \ \vee  coin_{\scriptscriptstyle\mathcal{A}r,j}\neq l) 
%  \Big)
% \\
% 
%\end{array} \middle |
%    \begin{array}{l}
%   \mathcal{A}(1^{\lambda},F)\rightarrow (u^{\scriptscriptstyle *},z,\bm{k},e,t,coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C},en, \text{aux},\bm{y}_{\scriptscriptstyle \mathcal  C},\bm{y}_{\scriptscriptstyle \mathcal  S})\\
%   
%   \mathtt{RCSP}.\mathtt{sInit}(u^{\scriptscriptstyle *},e, pk,z, t,\bm{y}_{\scriptscriptstyle \mathcal  C},\bm{y}_{\scriptscriptstyle \mathcal  S})\rightarrow (coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S},a)\\
%   
%	\mathcal{A}(coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S},a, \text{aux},\bm{k},Q,j, en)\rightarrow c^{\scriptscriptstyle *}_{\scriptscriptstyle j}\\
%
%     \mathtt{RCSP}.\mathtt{prove}(u^{\scriptscriptstyle *},  \sigma,  c^{\scriptscriptstyle *}_{\scriptscriptstyle j},pk, en)\rightarrow (b_{\scriptscriptstyle j},m_{\scriptscriptstyle \mathcal{S},j},\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j})\\
%     
% \mathcal{A}(\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j}, q,k,j,en)\rightarrow (d_{\scriptscriptstyle j},m_{\scriptscriptstyle \mathcal{A},j})\\
%   
%   
%   \mathtt{RCSP}.\mathtt{resolve}(\bm{m}_{\scriptscriptstyle \mathcal{A}},\bm{m}_{\scriptscriptstyle \mathcal{S}},z, {\bm{\pi}}^{\scriptscriptstyle *}, {\bm{c}}^{\scriptscriptstyle *},pk,en)\rightarrow (\bm{y}_{\scriptscriptstyle \mathcal C},\bm{y}_{\scriptscriptstyle \mathcal S})\\
%   \mathtt{RCSP}.\mathtt{pay}(\bm{y}_{\scriptscriptstyle \mathcal C},\bm{y}_{\scriptscriptstyle \mathcal S},t_{\scriptscriptstyle cp},a,coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C},coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S})\rightarrow ({\bm{coin}}_{\scriptscriptstyle\mathcal C},{\bm{coin}}_{\scriptscriptstyle\mathcal S},{\bm{coin}}_{\scriptscriptstyle\mathcal Ar})\\
%\end{array}    \right]\leq \mu(\lambda)$$
%}
%where $q_{\scriptscriptstyle j}\in D(c^{\scriptscriptstyle *}_{\scriptscriptstyle j},t_{\scriptscriptstyle qp})$, $
%D,t_{\scriptscriptstyle qp}\in en$, $\sigma\in e$, and   the probability is taken over the randomness used in witnesses $w_{\scriptscriptstyle cp},w_{\scriptscriptstyle qp}\in t$ as well as  the randomness used in proofs $w_{\scriptscriptstyle q_{_{\scaleto{j}{\size}}}}\in c_{\scriptscriptstyle j}$ and $w_{\scriptscriptstyle\sigma}\in e$ and  the randomness of $\mathcal{A}$.
%\end{definition}
% 
 Note, in the above definition, an honest server either does not deposit (e.g. when $a=0$) or if it deposits (i.e. agrees to serve) ultimately receives its deposit \emph{plus the service payment} (with a high probability). Informally, RC-S-P is privacy preserving if it guarantees the privacy of (a) the service input (e.g. outsourced file) and (b) the service proof's status during the private time bubble. In the following, we formally define privacy.
 

  \begin{definition}[RC-S-P Privacy]\label{deff::RC-S-P-Privacy}  A RC-S-P   preserves privacy, any auxiliary information $\text{aux}$, any number of verifications $z$, any price list $pl$, any $F, Q,M, E$ and $D$, the following hold:
   
\begin{enumerate}

\item For any PPT adversary $\mathcal{A}_{\scriptscriptstyle 1}$ there exists a negligible function $\mu_{\scriptscriptstyle 1}(\cdot)$, such that for any security parameter $\lambda$:
  
{\small
$$\Pr\left[
  \begin{array}{l}
  \mathcal{A}_{\scriptscriptstyle 1}(\bm{c}^{\scriptscriptstyle *},coin^{\scriptscriptstyle *}_{\scriptscriptstyle S},coin^{\scriptscriptstyle *}_{\scriptscriptstyle C}, g_{\scriptscriptstyle cp}, \\ g_{\scriptscriptstyle qp}, \bm{\pi}^{\scriptscriptstyle *}, pl, a)\rightarrow\beta\\
\end{array} \middle |
    \begin{array}{l}
            \mathtt{RCSP.keyGen}(1^{\lambda}, F)\rightarrow \bm{k}\\
        \mathcal{A}_{\scriptscriptstyle 1}(1^\lambda, pk, F)\rightarrow (u_{\scriptscriptstyle 0},u_{\scriptscriptstyle 1})\\


    \beta\stackrel{\scriptscriptstyle\$}\leftarrow\{0,1\}\\

   \mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u_{\scriptscriptstyle\beta},\bm{k}, M,z,pl,enc)\rightarrow (u^{\scriptscriptstyle *}_{\scriptscriptstyle\beta},e,T, p_{\scriptscriptstyle\mathcal S},  \bm{y}, coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C})\\
\mathtt{RCSP}.\mathtt{sInit}(u_{\scriptscriptstyle\beta}^{\scriptscriptstyle *}, e, pk, z, T, p_{\scriptscriptstyle\mathcal S},\bm{y},enc)\rightarrow (coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S},a)\\

\forall j \in [z]:\\

\Big(\mathtt{RCSP}.\mathtt{genQuery}(1^\lambda, \text{aux},k,Q_{\scriptscriptstyle\beta}, T_{\scriptscriptstyle qp}, enc)\rightarrow c^{\scriptscriptstyle *}_{\scriptscriptstyle j}\\
     \mathtt{RCSP}.\mathtt{prove}(u^{\scriptscriptstyle *}_{\scriptscriptstyle\beta},   \sigma,  c^{\scriptscriptstyle *}_{\scriptscriptstyle j}, pk, T_{\scriptscriptstyle qp},enc)\rightarrow (b_{\scriptscriptstyle j},m_{\scriptscriptstyle \mathcal{S},j},\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j})\\  
   \mathtt{RCSP}.\mathtt{verify}(\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j}, \bm{q}_{\scriptscriptstyle j},k,T_{\scriptscriptstyle qp},enc)\rightarrow (d_{\scriptscriptstyle j},m_{\scriptscriptstyle \mathcal{C},j})\Big)\\
\end{array}\right]\leq \frac{1}{2}+\mu_{\scriptscriptstyle 1}(\lambda).$$
}




\item For any PPT adversary $\mathcal{A}_{\scriptscriptstyle 2}$ who plays the above game, there exists a negligible function $\mu_{\scriptscriptstyle 2}(\cdot)$ such that


{\small
$$ Pr\left[\mathcal{A}_{\scriptscriptstyle 2}(\bm{c}^{\scriptscriptstyle *},coin^{\scriptscriptstyle *}_{\scriptscriptstyle \mathcal S},coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C}, g_{\scriptscriptstyle cp},  g_{\scriptscriptstyle qp},\bm{\pi}^{\scriptscriptstyle *}, pl, a)\rightarrow (d_{\scriptscriptstyle j},j)\right]\leq \frac{1}{2}+ \mu_{\scriptscriptstyle 2}(\lambda)$$
}

where $\bm{c}^{\scriptscriptstyle *}=[{c}^{\scriptscriptstyle *}_{\scriptscriptstyle 1},...,{c}^{\scriptscriptstyle *}_{\scriptscriptstyle z}], \bm{\pi}^{\scriptscriptstyle *}=[\pi^{\scriptscriptstyle *}_{\scriptscriptstyle 1},...,\pi^{\scriptscriptstyle *}_{\scriptscriptstyle z}]$, and $ {pp}\in T_{\scriptscriptstyle qp}$.  Also, depending on the choice of $\beta$, algorithm $\mathtt{RCSP}.\mathtt{genQuery}(.)$ outputs an encoded valid query, when the input is $Q_{\scriptscriptstyle 1}$, or outputs an encoded invalid query, when the input is $Q_{\scriptscriptstyle 0}$.
% The probability is taken over uniform  choice of $k,k'\stackrel{\scriptscriptstyle\$}\leftarrow \{0,1\}^{\scriptscriptstyle\lambda}$, where $k,k'\in\bm{k}$, the randomness of $\mathcal{A}_{\scriptscriptstyle 1}$ and $\mathcal{A}_{\scriptscriptstyle 2}$,  the randomness used in witnesses $g_{\scriptscriptstyle cp}, g_{\scriptscriptstyle qp}\in t$,  the randomness used in  $E$.
\end{enumerate}
\end{definition}
 
In the above definition, the experiment is allowed to produce  invalid queries. It is required that  the privacy holds regardless of the queries status, i.e. whether they are valid or invalid, as long as the are encoded and provided.  
 
 
 
%  \begin{definition}[RC-S-P Service Proof Privacy]\label{deff::RC-S-P-ServiceProofPrivacy}  A RC-S-P   preserves the privacy of service proof (status), if for any security parameter $\lambda$, any auxiliary information $\text{aux}$, any $F,Q,M,E,D$ and any probabilistic polynomial time adversary $\mathcal{A}$ that plays the  game in Definition \ref{deff::RC-S-P-Input-Privacy}, there exists a negligible function $\mu(.)$, such that: 
%
%\small{
%$$ Pr\left[\mathcal{A}(\bm{c}^{\scriptscriptstyle *},coin^{\scriptscriptstyle *}_{\scriptscriptstyle \mathcal S},coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C}, g_{\scriptscriptstyle cp},  g_{\scriptscriptstyle qp},\bm{\pi}^{\scriptscriptstyle *},a)\rightarrow (d_{\scriptscriptstyle j},j)\right]\leq \frac{1}{2}+ \mu(\lambda)$$
%}
%where $\bm{c}^{\scriptscriptstyle *}=[{c}^{\scriptscriptstyle *}_{\scriptscriptstyle 1},...,{c}^{\scriptscriptstyle *}_{\scriptscriptstyle z}]$ and $\bm{\pi}^{\scriptscriptstyle *}=[\pi^{\scriptscriptstyle *}_{\scriptscriptstyle 1},...,\pi^{\scriptscriptstyle *}_{\scriptscriptstyle z}]$.  The probability is taken over uniform  choice of $k,k'\stackrel{\scriptscriptstyle\$}\leftarrow \{0,1\}^{\scriptscriptstyle\lambda}$, where $k,k'\in\bm{k}$, the randomness of $\mathcal{A}$,  the randomness used in witnesses $g_{\scriptscriptstyle cp}, g_{\scriptscriptstyle qp}\in t$,  the randomness used in  $E$.
%\end{definition}
 
 
 
 %-----------------------------------
% \begin{definition}[RC-S-P Service Input Privacy]\label{deff::RC-S-P-Input-Privacy}  A RC-S-P   preserves the privacy of service input, if for any security parameter $\lambda$, any auxiliary information $\text{aux}$, any $F, Q,M, E,D$ and any probabilistic polynomial time adversary $\mathcal{A}$, there exists a negligible function $\mu(.)$, such that: 
%
%\small{
%$$ Pr\left[
%  \begin{array}{l}
%  \mathcal{A}(\bm{c}^{\scriptscriptstyle *},coin^{\scriptscriptstyle *}_{\scriptscriptstyle S},coin^{\scriptscriptstyle *}_{\scriptscriptstyle C},g_{\scriptscriptstyle cp},  g_{\scriptscriptstyle qp},\bm{\pi}^{\scriptscriptstyle *},a)\rightarrow\beta\\
%
%
%\end{array} \middle |
%    \begin{array}{l}
%    \mathtt{RCSP.keyGen}(1^{\lambda},F)\rightarrow \bm{k}\\
%    \mathcal{A}(1^\lambda,pk, F)\rightarrow (u_{\scriptscriptstyle 0},u_{\scriptscriptstyle 1})\\
%    \beta\stackrel{\scriptscriptstyle\$}\leftarrow\{0,1\}\\
%   
%   \mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u_{\scriptscriptstyle\beta},\bm{k}, M,z,cp)\rightarrow (u_{\scriptscriptstyle\beta}^{\scriptscriptstyle *},e,t,coin^{\scriptscriptstyle*}_{\scriptscriptstyle\mathcal C}, \bm{y}_{\scriptscriptstyle \mathcal  C},\bm{y}_{\scriptscriptstyle \mathcal  S})\\
%
%\mathtt{RCSP}.\mathtt{sInit}(u_{\scriptscriptstyle\beta}^{\scriptscriptstyle *},e, pk,z, t,\bm{y}_{\scriptscriptstyle \mathcal  C},\bm{y}_{\scriptscriptstyle \mathcal  S})\rightarrow (coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S},a)\\
%
%\mathtt{RCSP}.\mathtt{genQuery}(1^\lambda, \text{aux},k,Q,j, en)\rightarrow c^{\scriptscriptstyle *}_{\scriptscriptstyle j}\\
%	
%     
%     \mathtt{RCSP}.\mathtt{prove}(u^{\scriptscriptstyle *}_{\scriptscriptstyle\beta},  \sigma,  c^{\scriptscriptstyle *}_{\scriptscriptstyle j},pk, en)\rightarrow (b_{\scriptscriptstyle j},m_{\scriptscriptstyle \mathcal{S},j},\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j})\\
%     
%   \mathtt{RCSP}.\mathtt{verify}(\pi^{\scriptscriptstyle *}_{\scriptscriptstyle j}, \bm{q}_{\scriptscriptstyle j},k,en)\rightarrow (d_{\scriptscriptstyle j},m_{\scriptscriptstyle \mathcal{C},j})\\
%\end{array}    \right]\leq \frac{1}{2}+\mu(\lambda)$$
%}
%where $\bm{c}^{\scriptscriptstyle *}=[{c}^{\scriptscriptstyle *}_{\scriptscriptstyle 1},...,{c}^{\scriptscriptstyle *}_{\scriptscriptstyle z}]$ and $\bm{\pi}^{\scriptscriptstyle *}=[\pi^{\scriptscriptstyle *}_{\scriptscriptstyle 1},...,\pi^{\scriptscriptstyle *}_{\scriptscriptstyle z}]$.  The probability is taken over uniform  choice of $k,k'\stackrel{\scriptscriptstyle\$}\leftarrow \{0,1\}^{\scriptscriptstyle\lambda}$, where $k,k'\in\bm{k}$, the randomness of $\mathcal{A}$,  the randomness used in witnesses $g_{\scriptscriptstyle cp},g_{\scriptscriptstyle qp}\in t$,  the randomness used in  $E$.
%
%\end{definition}
% 
% 
% 
%  \begin{definition}[RC-S-P Service Proof Privacy]\label{deff::RC-S-P-ServiceProofPrivacy}  A RC-S-P   preserves the privacy of service proof (status), if for any security parameter $\lambda$, any auxiliary information $\text{aux}$, any $F,Q,M,E,D$ and any probabilistic polynomial time adversary $\mathcal{A}$ that plays the  game in Definition \ref{deff::RC-S-P-Input-Privacy}, there exists a negligible function $\mu(.)$, such that: 
%
%\small{
%$$ Pr\left[\mathcal{A}(\bm{c}^{\scriptscriptstyle *},coin^{\scriptscriptstyle *}_{\scriptscriptstyle \mathcal S},coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C}, g_{\scriptscriptstyle cp},  g_{\scriptscriptstyle qp},\bm{\pi}^{\scriptscriptstyle *},a)\rightarrow (d_{\scriptscriptstyle j},j)\right]\leq \frac{1}{2}+ \mu(\lambda)$$
%}
%where $\bm{c}^{\scriptscriptstyle *}=[{c}^{\scriptscriptstyle *}_{\scriptscriptstyle 1},...,{c}^{\scriptscriptstyle *}_{\scriptscriptstyle z}]$ and $\bm{\pi}^{\scriptscriptstyle *}=[\pi^{\scriptscriptstyle *}_{\scriptscriptstyle 1},...,\pi^{\scriptscriptstyle *}_{\scriptscriptstyle z}]$.  The probability is taken over uniform  choice of $k,k'\stackrel{\scriptscriptstyle\$}\leftarrow \{0,1\}^{\scriptscriptstyle\lambda}$, where $k,k'\in\bm{k}$, the randomness of $\mathcal{A}$,  the randomness used in witnesses $g_{\scriptscriptstyle cp}, g_{\scriptscriptstyle qp}\in t$,  the randomness used in  $E$.
%\end{definition}
 %-------------------------
 
 
 
 \begin{definition}[RC-S-P Security]\label{def::RC-S-P-Security} A RC-S-P scheme is secure if it satisfies security against malicious server, security against malicious client, and preserves privacy, w.r.t. Definitions \ref{deff::RC-S-P-SecurityAgainstMaliciousServer}-\ref{deff::RC-S-P-Privacy}. 
 \end{definition}
 

 
 


==> RC-PoR-P-Gas.tex <==
% !TEX root =main.tex


%\vspace{-5mm}
 
 
 


 %\vspace{-7mm}
 
 \begin{table*}[!htbp]
\begin{footnotesize}

\begin{center}
\caption{ \small RC-PoR-P  on-chain cost of $z$ verifications, breakdown by phases.}\label{table::RC-PoR-P-runTime} 

\renewcommand{\arraystretch}{1}
%\scalebox{0.94}{
%\begin{subtable}{.64\linewidth}%xxxx
%\begin{minipage}{.88\linewidth}
%\caption{\small Computation Cost}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
   \hline
\cellcolor[gray]{0.9} &
 \multicolumn{2}{c|}{\cellcolor[gray]{0.9}\scriptsize \underline{  \  \ \ \ \  \ \ \ \  \ \ Cost \  \ \ \ \  \ \ \ \  \ \ }}\\
 %\cline{3-5}
\cellcolor[gray]{0.9} \multirow{-2}{*} {\scriptsize Phase}&\cellcolor[gray]{0.9}\scriptsize In ether&\cellcolor[gray]{0.9}\scriptsize In US dollar\\
\hline

\multirow{3}{*}{\rotatebox[origin=c]{0}{\scriptsize }} \cellcolor[gray]{0.9}\scriptsize Client-side Ini.&\scriptsize$123\cdot 10^{-5}$&\scriptsize$3.42$ \\
     \cline{1-3}  
     
 \cellcolor[gray]{0.9}\scriptsize Server-side Ini.&\scriptsize$9\cdot 10^{-5}$ &\scriptsize$0.22$\\
     \cline{1-3} 
       \cellcolor[gray]{0.9}\scriptsize Client-side Query Gen.&\scriptsize$6\cdot 10^{-5}\cdot z$&\scriptsize$0.17\cdot z$ \\
   %  \cline{1-3} 
  %\cellcolor[gray]{0.9}\scriptsize Client-side Proof Ver.&\scriptsize$ 0.09\cdot z$&\scriptsize$0.11\cdot z$ \\
  \cline{1-3} 
    \cellcolor[gray]{0.9}\scriptsize Arbiter-side Dispute Res.&\scriptsize$ 1\cdot 10^{-4}$&\scriptsize$ 0.27$\\
 \cline{1-3}
    \cellcolor[gray]{0.9}\scriptsize Coin Transfer.&\scriptsize$6\cdot 10^{-5}$&\scriptsize$ 0.17$\\

 \hline
\end{tabular}
%\end{minipage}%******
%\end{subtable}%xxxx
%}
\end{center}
\end{footnotesize}
\end{table*}



% \noindent\textbf{\textit{Computation Complexity}}. For a client to generate $z$ puzzles, it performs $z$ symmetric key-based encryption,  $z$ modular exponentiations  and $z$ modular additions. Also, to commit to values, it invokes a commitment scheme $z$ times; if a hash-based commitment is used then it would involve $z$ invocations of a hash function, and if Pedersen commitment is used then it would involve $2 z$ exponentiations and $z$ multiplications. Thus, the overall computation complexity of the client   is $O(z)$. For the server to solve $z$ puzzles, it calls $\mathtt{TLP.SolvPuz}(.)$ $z$ times, which leads to $O(Tz)$ computation complexity. Also, the verification cost  only involves $z$ invocations of the commitment scheme; if the hash-based commitment is used, then it would involve $z$ invocations of a hash function,  if Pedersen commitment is utilised, then it would involve $2 z$ exponentiations and $z$ multiplications. Thus, the  verification's complexity is $O(z)$.
%
%
%
%
% 
% 
% \noindent\textbf{\textit{Communication Complexity}}.  In step \ref{Generate-Puzzle}, the client publishes two vectors: $\vv{\bm{o}}$ and $\vv{\bm{h}}$, with  $2 z$ and $z$ elements respectively.  Each element of $\vv{\bm{o}}$ is a pair $(o_{\scriptscriptstyle j,1},o_{\scriptscriptstyle j,2})$, where $o_{\scriptscriptstyle j,1}$ is an output of symmetric key encryption, e.g.   $|o_{\scriptscriptstyle j,1}|=128$-bit, and $o_{\scriptscriptstyle j,2}$ is an element of $\mathbb{Z}_{\scriptscriptstyle N}$, e.g.  $|o_{\scriptscriptstyle j,2}|=2048$-bit. Also, each element $h_{\scriptscriptstyle j}$ of $\vv{\bm{h}}$ is either an output of a hash function, when a hash-based commitment is used, e.g.  $|h_{\scriptscriptstyle j}|=256$-bit, or an element of $\mathbb{F}_{\scriptscriptstyle q}$ when Pedersen commitment is used, e.g.  $|h_{\scriptscriptstyle j}|=1024$-bit. Thus, its  bandwidth is about $2432 z$ bits when the former,  or $3200 z$ bits when the latter commitment scheme is utilised. Also, its   complexity is $O(z)$. For the server to prove, in step \ref{prove-},   it sends $z$ pairs $(m_{\scriptscriptstyle j},d_{\scriptscriptstyle j})$ to the verifier, where $m_{\scriptscriptstyle j}$  is an arbitrary message, e.g.  $|m_{\scriptscriptstyle j}|=500$-bit, and  $d_{\scriptscriptstyle j}$ is either a long enough random value, e.g. $|d_{\scriptscriptstyle j}|=128$-bit, when the hash-based commitment is used, or an element of $\mathbb{F}_{\scriptscriptstyle q}$ when Pedersen scheme is used, e.g. $|d_{\scriptscriptstyle j}|=1024$-bit. So, its bandwidth is about either $628 z$ or $1524 z$ bits when the former or latter commitment scheme is used respectively. The solver's  communication complexity is $O(z)$. 
 

 


==> RC-PoR-P-Proof.tex <==
% !TEX root =main.tex


\begin{theorem}
The RC-PoR-P protocol is secure, w.r.t. Definition \ref{def::RC-S-P-Security}, if PoRID and SAP are secure and the encryption scheme is semantically secure. 
\end{theorem}


 In order to prove the above theorem, we show that RC-PoR-P meets all the security properties defined in Section \ref{sec::RC-S-P-Definition}.  We first prove that RC-PoR-P satisfies security against a malicious server.  

 \begin{lemma}
 If SAP is secure and  PoRID scheme supports correctness, soundness, and detectable abort, then RC-PoR-P is secure against malicious server, w.r.t. Definition \ref{deff::RC-S-P-SecurityAgainstMaliciousServer}. 
 \end{lemma}
 

 \begin{proof}[sketch]
 We first consider event $F(u^{\scriptscriptstyle *},\bm{q}_{\scriptscriptstyle j})= h_{\scriptscriptstyle j}\ \wedge coin_{\scriptscriptstyle\mathcal{C},j}\neq  \frac{coin_{\scriptscriptstyle\mathcal C}^{\scriptscriptstyle*}}{z}-o$ that captures the case where the server provides an accepting service proof but makes the client withdraw an incorrect amount of coins, i.e. $coin_{\scriptscriptstyle\mathcal{C},j}\neq  \frac{coin_{\scriptscriptstyle\mathcal C}^{\scriptscriptstyle*}}{z}-o$. In this case, since the proof is valid, an honest client accepts it and does not raise any dispute. 
  However, the server  would be able to make the client  withdraw incorrect amounts of coins, if it manages to either convince the arbiter that the client has misbehaved (through dispute resolution phase), or submit to the contract, at the coin transfer phase,  an accepting  statement $\ddot{x}'_{\scriptscriptstyle cp}$ other than what was agreed at the initiation phase, i.e. $\ddot{x}_{\scriptscriptstyle cp}$. Nevertheless, it cannot falsely accuse the client of misbehaviour. Because,  due to the security of SAP, it cannot  convince the arbiter to accept different decryption key or pads other than what was agreed with the client in the initiation phase; specifically, it cannot persuade the arbiter to accept  $\ddot{x}'_{\scriptscriptstyle qp}$, where $\ddot{x}'_{\scriptscriptstyle qp}\neq \ddot{x}_{\scriptscriptstyle qp}$, except with a negligible probability, $\mu(\lambda)$. This ensures that the honest client's message is accessed by  the arbiter with a high probability, as the arbiter can extract the client's message using valid pad information and decryption key. Moreover,  due to the security of SAP, the server cannot persuade the contract to accept any statement other than what was agreed initially between the client and server, except with a negligible probability $\mu(\lambda)$ when it finds the hash function's collision. Also, due to the correctness of VSID, the arbiter always accepts the honest client's accepting proof. 

We now move on to event $F(u^{\scriptscriptstyle *}, \bm{q}_{\scriptscriptstyle j})\neq h_{\scriptscriptstyle j} \ \wedge (d_{\scriptscriptstyle j}=1	\vee y_{\scriptscriptstyle \mathcal S}[j]=0 \ \vee (coin_{\scriptscriptstyle\mathcal{C},j}\neq \frac{coin_{\scriptscriptstyle\mathcal C}^{\scriptscriptstyle*}}{z} \ \vee  coin_{\scriptscriptstyle\mathcal{A}r,j}\neq l))$ which captures the case where the server provides an invalid service proof but either persuades the client to accept the proof, or  (when the client raises a dispute)  persuades the arbiter to accept the proof or makes the client or arbiter withdraw an incorrect amount of coins, i.e.    $coin_{\scriptscriptstyle\mathcal{C},j}\neq \frac{coin_{\scriptscriptstyle\mathcal C}^{\scriptscriptstyle*}}{z}$ or $coin_{\scriptscriptstyle\mathcal{A}r,j}\neq l$ respectively.   Nevertheless, due to the soundness of VSID, the probability that a corrupt server can convince an honest client to accept invalid proof (i.e. outputs $d_{\scriptscriptstyle j}=1$), is negligible, $\mu(\lambda)$. On the other hand, in the case where the client rejects the proof and raises a dispute, the server may try to convince the arbiter and make it output $y_{\scriptscriptstyle \mathcal S}[j]=0$, e.g. by sending a complaint right after the client does. But, for the adversary to win, it has to either provide a different accepting statement $\ddot{x}'_{\scriptscriptstyle qp}$, than what was initially agreed with the client (i.e. $\ddot{x}'_{\scriptscriptstyle qp}\neq \ddot{x}_{\scriptscriptstyle qp}$) and passes the verification, which   requires finding the hash function's collision, and its probability of success is negligible, $\mu(\lambda)$. Or it makes the arbiter  accept an invalid proof, but due to the detectable abort property of VSID, its probability of success is also negligible, $\mu(\lambda)$. In the case where the adversary does not succeed in convincing the client or arbiter, it may still try to  make them withdraw an incorrect amount of coins. To this end, at the coin transfer phase, it has to send a  different accepting statement  than what was initially agreed with the client. But, it would succeed only with a negligible probability, $\mu(\lambda)$, due to the security of SAP. 

Furthermore, in   both  events above, due to the security of SAP, the adversary cannot block an honest client's  messages, ``pay'' and $\ddot{x}_{\scriptscriptstyle cp}$, to the contract in the coin transfer phase.
  \hfill\(\Box\)\end{proof}



\begin{lemma}
 If SAP is secure and  VSID scheme supports correctness, inputs well-formedness, and detectable abort, then RC-S-P is secure against malicious client, w.r.t. Definition \ref{deff::RC-S-P-Security-Against Malicious-Client}. 
\end{lemma}


\begin{proof}[sketch]
  First, we consider event  $(M(u^{\scriptscriptstyle *},k)= \sigma  \wedge Q(\text{aux},k)= \bm{q}_{\scriptscriptstyle j}) \wedge
  (coin_{\scriptscriptstyle\mathcal{S},j}\neq  \frac{coin_{\scriptscriptstyle\mathcal S}^{\scriptscriptstyle*}}{z}+o)$ which captures the case where the client provides  accepting metadata and query  but makes the server withdraw an incorrect amount of coins, i.e. $coin_{\scriptscriptstyle\mathcal{S},j}\neq  \frac{coin_{\scriptscriptstyle\mathcal S}^{\scriptscriptstyle*}}{z}+o$. In short, for the event to  happen with a high probability, a malicious client has to break the security of SAP. In particular, since the metadata and query's proofs are valid, an honest server accepts them and does not raise any dispute.  But, the client may want to  make the server  withdraw incorrect amounts of coins, if it manages to either convince the arbiter, in phase \ref{RCSP::Dispute-Resolution}, that the server has misbehaved, or submit to the contract  an accepting  statement $\ddot{x}'_{\scriptscriptstyle cp}$ other than what was agreed at the initiation phase, i.e. $\ddot{x}_{\scriptscriptstyle cp}$, in phase \ref{RCSP::CoinTransfer}. However, it cannot falsely accuse the server of misbehaviour. As,  due to the security of SAP, it cannot  convince the arbiter to accept different decryption key and pads, by providing a different accepting statement $\ddot{x}'_{\scriptscriptstyle qp}$  (where $\ddot{x}'_{\scriptscriptstyle qp}\neq \ddot{x}_{\scriptscriptstyle qp}$), than what was initially agreed with the server, except with  probability $\mu(\lambda)$. This ensures that  the arbiter is given the honest server's messages (with a high probability). Moreover,  due to the security of SAP, the client cannot convince the contract to accept any accepting statement other than what was initially agreed  between the client and server, except with   probability $\mu(\lambda)$. Furthermore,   the correctness of VSID guarantees that  the arbiter always accepts the honest server's accepting proof. 
  
    We now turn our attention to $(M(u^{\scriptscriptstyle *},k)\neq \sigma \wedge a=1)\ \vee\ (Q(\text{aux},k)\neq \bm{q}_{\scriptscriptstyle j} \wedge b_{\scriptscriptstyle j}=1)$,   that captures the case where the server accepts an ill-formed metadata, or query. However, due to inputs well-formedness of VSID, the probability that either of the events happens is negligible, $\mu(\lambda)$. Next, we move of to      $Q(\text{aux},k)\neq \bm{q}_{\scriptscriptstyle j} \wedge
  (y_{\scriptscriptstyle\mathcal{C}}[j]=0 \ \vee  coin_{\scriptscriptstyle\mathcal{S},j}\neq \frac{coin_{\scriptscriptstyle\mathcal S}^{\scriptscriptstyle*}}{z}+o \ \vee  coin_{\scriptscriptstyle\mathcal{A}r,j}\neq l)$.  It considers the case where the client provides an invalid query, but  either convinces the arbiter to accept it, or  makes the server or arbiter  withdraw an incorrect amount of coins, i.e. $coin_{\scriptscriptstyle\mathcal{S},j}\neq \frac{coin_{\scriptscriptstyle\mathcal S}^{\scriptscriptstyle*}}{z}+o$ or  $coin_{\scriptscriptstyle\mathcal{A}r,j}\neq l$ respectively. Note, when the server rejects the query and raises a dispute, the client may try to convince the arbiter, and make it output $y_{\scriptscriptstyle \mathcal C}[j]=0$, e.g. by sending a complaint right after the server does so. However, for the adversary to win, either it has to provide a different accepting statement $\ddot{x}'_{\scriptscriptstyle qp}$, than what was initially agreed with the server (i.e. $\ddot{x}'_{\scriptscriptstyle qp}\neq \ddot{x}_{\scriptscriptstyle qp}$) and passes the verification. But,  due to the security of SAP, its probability of success is negligible, $\mu(\lambda)$. Or it has to make the arbiter  accept an invalid query, i.e. makes the arbiter output $y_{\scriptscriptstyle\mathcal{C}}[j]=0$. Nevertheless, due to the detectable abort property of VSID, its probability of success is  negligible, $\mu(\lambda)$. If the adversary does not succeed in convincing the server or arbiter, it may still try to  make them withdraw an incorrect amount of coins. To this end, at the coin transfer phase, it has to send a  different accepting statement  than what was initially agreed with the server. However, due to the security of SAP, its  success probability is negligible, $\mu(\lambda)$. Also, due to the security of SAP, the adversary cannot block an honest server's  messages, ``pay'' and $\ddot{x}_{\scriptscriptstyle cp}$, to the contract in the coin transfer phase.
 \hfill\(\Box\)\end{proof}
  
  
  Prior to proving  RC-S-P's privacy, we provide a lemma that will be used in the privacy's proof. Informally, the lemma states that encoded coins leaks no information about the actual amount of coins $(o,l)$, agreed between the client and server. 


\begin{lemma}\label{lemma::encoded-coins} Let $\beta\stackrel{\scriptscriptstyle\$}\leftarrow\{0,1\}$, price list be $\{(o_{\scriptscriptstyle 0},l_{\scriptscriptstyle 0}),(o_{\scriptscriptstyle 1},l_{\scriptscriptstyle 1})\}$, and encoded coin amounts be $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal{C}}= z\cdot(Max(o_{\scriptscriptstyle\beta},o_{\scriptscriptstyle|\beta-1|})+Max(l_{\scriptscriptstyle\beta},l_{\scriptscriptstyle|\beta-1|}))$ and $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal{S}}=z\cdot(Max(l_{\scriptscriptstyle\beta}, l_{\scriptscriptstyle |\beta-1|}))$. Then, given the price list, $z$, $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal{C}}$, and $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal{S}}$, an adversary $\mathcal{A}$ cannot tell the value of $\beta$ with probability significantly greater than $\frac{1}{2}$ (where the probability is taken over the choice of $\beta$ and the randomness of $\mathcal{A}$).
\end{lemma}



\begin{proof}
As it is evident, the list and $z$ contains no information about $\beta$. Also, since  $z$ is a public value, we could have   $coin'^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C}=\frac{coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C}}{z} = Max(o_{\scriptscriptstyle\beta},o_{\scriptscriptstyle|\beta-1|})+Max(l_{\scriptscriptstyle\beta}, l_{\scriptscriptstyle|\beta-1|})$. It is not hard to see $coin'^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C}$ is a function of maximum value of $(o_{\scriptscriptstyle 0},o_{\scriptscriptstyle 1})$, and maximum value of $(l_{\scriptscriptstyle 0},l_{\scriptscriptstyle 1})$. It is also  independent of $\beta$. Therefore, given the list, $z$ and $coin'^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C}$ the adversary learns nothing about $\beta$, unless it guesses the value,  with  success probability $\frac{1}{2}$. The same also holds for $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal S}$. 
 \hfill\(\Box\)\end{proof}


\begin{lemma} If SAP is secure and the encryption scheme is semantically secure, then RC-S-P preserves privacy, w.r.t. Definition \ref{deff::RC-S-P-Privacy}. 
\end{lemma}

\begin{proof}[sketch]
Due to the privacy property of SAP, that stems from the  hiding property of the commitment scheme, given the commitments $g_{\scriptscriptstyle qp}$ and $g_{\scriptscriptstyle cp}$, (that are stored in the blockchain as result of running SAP) the adversary learns no information about the committed values (e.g. $o, l, pad_{\scriptscriptstyle\pi}, pad_{\scriptscriptstyle q},$ and $\bar{k}$), except with negligible probability, $\mu_{\scriptscriptstyle 1}(\lambda)$.   Also, given encoded coins $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal{C}}=z\cdot (o_{\scriptscriptstyle max}+l_{\scriptscriptstyle max})$ and  $coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal{S}}=z\cdot l_{\scriptscriptstyle max}$, the adversary learns nothing about the actual price agreed between the server and client,  $(o,l)$, for each verification, due to Lemma \ref{lemma::encoded-coins}. Next we analyse the privacy of padded encrypted query vector $\bm{c}^{\scriptscriptstyle *}$. For  the sake of simplicity, we focus on   $\bm{q}^{\scriptscriptstyle *}_{\scriptscriptstyle j}\in c^{\scriptscriptstyle *}_{\scriptscriptstyle j}\in\bm{c}^{\scriptscriptstyle *}$, that is a padded encrypted query vector for $j$-th verification. Let $\bm{q}_{\scriptscriptstyle j,0}$ and $\bm{q}_{\scriptscriptstyle j,1}$  be query vectors, for $j$-th verification, related to the service inputs $u_{\scriptscriptstyle 0}$ and $u_{\scriptscriptstyle 1}$ that    are picked by the adversary according to  Definition  \ref{deff::RC-S-P-Privacy} which lets  the environment pick $\beta\stackrel{\scriptscriptstyle\$}\leftarrow \{0,1\}$. Also, let $\{\bm{q}_{\scriptscriptstyle j,0},...,\bm{q}_{\scriptscriptstyle j,m}\}$ be a  list of all queries of different sizes. In the experiment, if $\bm{q}_{\scriptscriptstyle j,\beta}$  is only   encrypted (but not padded), then given the ciphertext, due to semantical security of the encryption, an adversary cannot tell if the ciphertext corresponds to $\bm{q}_{\scriptscriptstyle j,0}$ or $\bm{q}_{\scriptscriptstyle j,1}$  (accordingly to $u_{\scriptscriptstyle 0}$ or $u_{\scriptscriptstyle 1}$) with probability greater than $\frac{1}{2}+\mu_{\scriptscriptstyle 1}(\lambda)$,  under the assumption  that $Max(|\bm{q}_{\scriptscriptstyle j,0}|,...,|\bm{q}_{\scriptscriptstyle j,m}|)=|\bm{q}_{\scriptscriptstyle j,\beta}|$. The  assumption is  relaxed with the use of a pad; as each encrypted query is padded  to the queries' maximum size, i.e. $Max(|\bm{q}_{\scriptscriptstyle j,0}|,...,|\bm{q}_{\scriptscriptstyle j,m}|)$, the adversary cannot tell with probability greater than $\frac{1}{2}+\mu_{\scriptscriptstyle 1}(\lambda)$ if the  padded encrypted proof corresponds to  $\bm{q}_{\scriptscriptstyle j,0}$ or $\bm{q}_{\scriptscriptstyle j,1}$, as the padded encrypted query \emph{always has the same size} and the pad values are picked from the same range as the encryption's ciphertext are defined. The same argument holds for $\bm{w}^{\scriptscriptstyle *}_{\scriptscriptstyle q_{_{\scaleto{j}{\size}}}}\in c^{\scriptscriptstyle *}_{\scriptscriptstyle j}\in\bm{c}^{\scriptscriptstyle *}$. 

Next we analyse the privacy of padded encrypted proof vector $\bm{\pi}^{\scriptscriptstyle *}$. The argument is similar to the one presented above; however, for  the sake of completeness we provide it.  Again, we focus on an element of the vector,  $\pi_{\scriptscriptstyle j}^{\scriptscriptstyle *}\in\bm{\pi}^{\scriptscriptstyle *}$, that is a padded encrypted proof for $j$-th verification. Let $\pi_{\scriptscriptstyle j,0}$ and $\pi_{\scriptscriptstyle j,1}$  be proofs, for $j$-th verification, related to the service inputs $u_{\scriptscriptstyle 0}$ and $u_{\scriptscriptstyle 1}$, where the inputs   are picked by the adversary, w.r.t. Definition  \ref{deff::RC-S-P-Privacy} in which  the environment picks $\beta\stackrel{\scriptscriptstyle\$}\leftarrow \{0,1\}$.  Let $\{\pi_{\scriptscriptstyle j,0},...,\pi_{\scriptscriptstyle j,m}\}$ be proof list including all proofs of different sizes. In the experiment, if $\pi_{\scriptscriptstyle j,\beta}$  is only   encrypted, then given the ciphertext, due to semantical security of the encryption, an adversary cannot tell if the ciphertext corresponds to $\pi_{\scriptscriptstyle j,0}$ or $\pi_{\scriptscriptstyle j,1}$  (accordingly to $u_{\scriptscriptstyle 0}$ or $u_{\scriptscriptstyle 1}$) with probability greater than $\frac{1}{2}+\mu_{\scriptscriptstyle 2}(\lambda)$,  if $Max(|\pi_{\scriptscriptstyle j,0}|,...,|\pi_{\scriptscriptstyle j,m}|)=|\pi_{\scriptscriptstyle j,\beta}|$. However, the  assumption is  relaxed with the use of a pad. In particular, since each encrypted proof is padded  to the proofs' maximum size, the adversary cannot tell with probability greater than $\frac{1}{2}+\mu_{\scriptscriptstyle 2}(\lambda)$ if the  padded encrypted proof corresponds to  $\pi_{\scriptscriptstyle j,0}$ or $\pi_{\scriptscriptstyle j,1}$. Also, since the value of $a$ is independent of $u_{\scriptscriptstyle 0}$  or $u_{\scriptscriptstyle 1}$, and only depends on whether the metadata is well-formed, it leaks nothing about the service input $u_{\scriptscriptstyle\beta}$ and $\beta$. Moreover, since each padded encrypted query and proof leak no information and always contains a fixed number of elements, an adversary cannot tell the status of a proof for each $j$-th verification (i.e. whether it is accepted or rejected) with the probability greater than $\frac{1}{2}+\mu_{\scriptscriptstyle 2}(\lambda)$, given  $\bm{c}^{\scriptscriptstyle *},coin^{\scriptscriptstyle *}_{\scriptscriptstyle \mathcal S},coin^{\scriptscriptstyle *}_{\scriptscriptstyle\mathcal C}, g_{\scriptscriptstyle cp},  g_{\scriptscriptstyle qp},$  $\bm{\pi}^{\scriptscriptstyle *}$, and $a$.
  \hfill\(\Box\)\end{proof}




==> RC-S-P-Definition_backup.tex <==
% !TEX root =main.tex

\section{Recurring Contingent Service Payment (RC-S-P) Definition}\label{sec::RC-S-P-Definition}

In this section, we introduce a formal definition of recurring contingent service payment (RC-S-P).    Before presenting the formal definition of RC-S-P, we outline what a \emph{verifiable service} (VS) is. At a high level, a VS scheme is a two-party protocol in which a client chooses a function, $F$, and provides (an encoding of) $F$, its input $u$, and a query $\bm{q}$ to a server.  The server is expected to evaluate $F$ on $u$ and $\bm{q}$ (and some public parameters) and respond with the output. Then, the client verifies that the output is indeed the output of the function computed on the provided input. In verifiable services, either the computation (on the input) or both the computation and storage of the input are delegated to the server. We present a full formal definition of a VS scheme in Appendix \ref{subsec:VS}. 


%
%Even though a VSID scheme offers two  appealing features, it is not sufficient to address all the issues we identified in Section \ref{sec::previous-work-limitations}. In particular, it does not take the privacy of service input and proofs' status into consideration and does not take into account a secure and fair payment (so it cannot deal with the issue related to wasting the server's resources). Thus, in the following, we present an upgraded VSID's definition that takes the above points into account.  We call the enhanced VSID, which  offers the features, \emph{recurring contingent service payment (RC-S-P)}. 
%





\begin{definition}[RC-S-P Scheme]\label{RC-S-P-def}
A recurring contingent service payment scheme RC-S-P  $=(\mathtt{RCSP}.\mathtt{keyGen}, $ $\mathtt{RCSP}.\mathtt{cInit}, $ $\mathtt{RCSP}.\mathtt{sInit},  $ $\mathtt{RCSP}.\mathtt{genQuery},\mathtt{RCSP}.\mathtt{prove},\mathtt{RCSP}.\mathtt{verify},\mathtt{RCSP}.\mathtt{resolve},\mathtt{RCSP}.\mathtt{pay})$ involves four parties; namely, client, server, arbiter and smart contract (which represents a bulletin board), and consists of eight algorithms defined as follows.\\[2pt]
%
\underline{$\mathtt{RCSP}.\mathtt{keyGen}(1^{\lambda}, F)\rightarrow \bm{k}$}:  A probabilistic algorithm run by client $\mathcal{C}$. It takes as input security parameter $1^\lambda$, and  function $F$ that will be run on the client's input by the server as a part of the service it provides. It outputs $\bm{k}:=(k,k')$ that contains a secret and public verification key pair $k:=(sk,pk)$ and a set of secret and public parameters, $k':=(sk',pk')$. It sends $pk$ and $pk'$ to the contract. \\[2pt]
%
%
\underline{$\mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, M,z, pl, enc)\rightarrow (u^{\st *},e,T, p_{\st\mathcal S},  \bm{y}, coin^{\st*}_{\st\mathcal C})$}: It is run by  $\mathcal{C}$. It takes as input $1^\lambda$,  the service input $u$,   $\bm{k}:=(k, k')$,   metadata generator function $M$, the total number of verifications $z$, and  price list $pl$ containing pairs of  actual coin amount for each accepting service proof and the amount for covering each potential dispute resolution's cost.  It also takes as input encoding/decoding functions $enc:=(E,D)$.  It encodes $u$, that yields  $u^{\st *}$. {It  sets $pp$ as (possibly) input dependent parameters, e.g., file size.}
 It computes metadata $\sigma=M(u^{\st *},k,{pp})$ and a  proof $w_{\st\sigma}$ asserting the metadata is well-structured. It sets the value of $p_{\st\mathcal S}$ to the total coins the server should deposit. It picks a private price pair $(o,l)\in pl$. It sets coin secret parameters $cp$ that include $(o,l)$ and parameters of $pl$. It constructs coin encoding token $T_{\st cp}$ containing   $cp$ and   $cp$'s witness, $g_{\st cp}$. It   constructs  encoding token $T_{\st qp}$ that contains secret  parameters $qp$ including {$pp$}, (a  representation of $\sigma$) and parameters (in $sk'$) that will be used to encode the service queries/proofs.   $T_{\st qp}$ contains     $qp$'s witness,  $g_{\st qp}$. 
  Given a valid value and its witness  anyone can check if they match. It sets a vector of parameters $\bm{y}$ that includes  binary vectors $[\bm{y}_{\st \mathcal  C}, \bm{y}_{\st \mathcal  S},\bm{y}'_{\st \mathcal  C}, \bm{y}'_{\st \mathcal  S}]$ each of which is set to $0$ and its length is $z$.  Note $\bm{y}$ may contain other public parameters (e.g., the contract's address).  It outputs  $u^{\st *}$,  $e:=(\sigma,w_{\st\sigma})$,  $T:=(T_{\st cp},T_{\st qp})$,  $p_{\st\mathcal S}$,    $\bm{y}$,  and the encoded coins amount  $coin^{\st*}_{\st\mathcal C}$ (that contains $o$ and $l$ coins in an encoded form).  $\mathcal{C}$ sends  $u^{\st *}$, $z$,  $e$, $T_{\st cp} \setminus  \{g_{\st cp}\}$ and $T_{\st qp} \setminus  \{g_{\st qp}\}$ to the server  $\mathcal{S}$ and  sends $g_{\st cp},  g_{\st qp},p_{\st\mathcal S}$, and $\bm{y}$,  and $coin^{\st*}_{\st\mathcal C}$  coins to the  contract. \\[2pt]
%
\underline{$\mathtt{RCSP}.\mathtt{sInit}(u^{\st *},e, pk,z, T, p_{\st\mathcal S},\bm{y},enc)\rightarrow (coin^{\st *}_{\st\mathcal S},a)$}: It is  run by  $\mathcal{S}$. It takes as input $u^{\st *}$, metadata-proof pair $e:=(\sigma,w_{\st\sigma})$,   $pk$ (read from the contract),  $z$, and $T:=(T_{\st cp},T_{\st qp})$, where $\{g_{\st cp},  g_{\st qp}\}$ are read from the smart contract. It reads $p_{\st\mathcal S}$, and $\bm{y}$ from the smart contract and takes as input the encoding/decoding functions $enc:=(E,D)$. It  checks the validity of $e$ and  $T$ elements. It checks elements of $\bm{y}$ and ensures each element of $\bm{y}_{\st \mathcal  C}, \bm{y}_{\st \mathcal  S},\bm{y}'_{\st \mathcal  C}, \bm{y}'_{\st \mathcal  S}\in \bm{y}$ have been set to $0$. If all checks pass, then it encodes the amount of its coins that yields $coin^{\st*}_{\st\mathcal S}$, and sets $a=1$. Otherwise, it sets $coin^{\st *}_{\st\mathcal S}=\bot$ and $a=0$. It outputs $coin^{\st *}_{\st\mathcal S}$ and $a$. The smart contract is given $coin^{\st *}_{\st\mathcal S}$ coins and $a$.  \\[2pt]
%
\underline{$\mathtt{RCSP}.\mathtt{genQuery}(1^\lambda, \text{aux},k,Q, T_{\st qp}, enc)\rightarrow c^{\st *}_{\st j}$}: A probabilistic algorithm run by  $\mathcal{C}$. It takes as input  $1^\lambda$,  auxiliary information $\text{aux}$,  the key pair $k$,   query generator  function $Q$, encoding token $T_{\st qp}$ and $enc:=(E,D)$.  It computes a pair $c_{\st j}$ containing a query vector $\bm{q}_{\st j}=Q( \text{aux},k,{pp})$,  and proof $\bm{w}_{\st q_{_{\scaleto{j}{\size}}}}$ proving the query is well-structured, where {$pp\in T_{\st qp}$}. It outputs the encoding of the pair, $c^{\st *}_{\st j}=E(c_{\st j},T_{\st qp})$, and sends the output to the contract. \\[2pt]
%
\underline{$\mathtt{RCSP}.\mathtt{prove}(u^{\st *},  \sigma,  c^{\st *}_{\st j},pk, T_{\st qp},enc)\rightarrow (b_{\st j},m_{\st \mathcal{S},j},\pi^{\st *}_{\st j})$}: It is run by  $\mathcal{S}$. It  takes as input $u^{\st *}$, metadata $\sigma$,   $c^{\st *}_{\st j}$,  $pk$,    $T_{\st qp}$, and $enc:=(E,D)$.   It checks the validity of decoded query pair $c_{\st j}=D(c^{\st *}_{\st j},T_{\st qp})$.  If it is rejected, then it sets $b_{\st j}=0$ and constructs a complaint $m_{\st \mathcal{S},j}$. Otherwise,  it   sets $b_{\st j}=1$ and $m_{\st \mathcal{S},j}=\bot$. It outputs $b_{\st j},m_{\st \mathcal{S},j}$,   and  encoded proof $\pi^{\st *}_{\st j}=E(\pi_{\st j},T_{\st qp})$, where  $\pi_{\st j}$ contains $h_{\st j}=F(u^{\st *},\bm{q}_{\st j},{pp})$ and a proof $\delta_{\st j}$  asserting the evaluation is performed correctly ($\pi_{\st j}$ may contain dummy values if $b_{\st j}=0$). The smart contract is given $\pi^{\st *}_{\st j}$.\\[2pt]
%
\underline{$\mathtt{RCSP}.\mathtt{verify}(\pi^{\st *}_{\st j}, c^{\st *}_{\st j},k,T_{\st qp},enc)\rightarrow (d_{\st j},m_{\st \mathcal{C},j})$}: A deterministic algorithm run by  $\mathcal{C}$. It takes as input  $\pi^{\st *}_{\st j}$,  query vector $\bm{q}_{\st j}\in c^{\st *}_{\st j}$,  $k$,   $T_{\st qp}$ and $enc:=(E,D)$. It checks the decoded proof $\pi_{\st j}=D(\pi^{\st *}_{\st j},T_{\st qp})$, if it is rejected,  it outputs $d_{\st j}=0$ and a complaint $m_{\st \mathcal{C},j}$. Otherwise, it outputs  $d_{\st j}=1$ and $m_{\st \mathcal{C},j}=\bot$.\\[2pt]
%
\underline{$\mathtt{RCSP}.\mathtt{resolve}(m_{\st \mathcal{C}},m_{\st \mathcal{S}},z, {\bm{\pi}}^{\st *}, {\bm{c}}^{\st *},pk, T_{\st qp},enc)\rightarrow \bm{y}$}: It is run by the arbiter $\mathcal{R}$. It takes as input $\mathcal{C}$'s complaints $m_{\st \mathcal{C}}$, $\mathcal{S}$'s complaints $m_{\st \mathcal{S}}$, $z$, all encoded proofs $ {\bm{\pi}}^{\st *}$, all encoded query pairs $ {\bm{c}}^{\st *}$,  $pk$, encoding token $T_{\st qp}$, and $enc:=(E,D)$. It verifies the token, decoded queries, and proofs.  It reads the  binary vectors $[\bm{y}_{\st \mathcal  C}, \bm{y}_{\st \mathcal  S},\bm{y}'_{\st \mathcal  C}, \bm{y}'_{\st \mathcal  S}]$ from the smart contract. It  updates $\bm{y}_{\st \mathcal E}$ by setting an element of it to one, i.e., $y_{\st \mathcal E,j}=1$, if party $\mathcal{E}\in\{\mathcal{C},\mathcal{S}\}$ has misbehaved in the $j$-th verification (i.e., provided invalid query or service proof). It also updates $\bm{y}'_{\st \mathcal E}$ (by setting an element of it to one) if party $\mathcal{E}$ has provided a complain that does not allow it to identify a misbehaved party, in  the $j$-th verification, i.e., when the arbiter is unnecessarily invoked. \\[2pt]
%
\underline{$\mathtt{RCSP}.\mathtt{pay}(\bm{y},T_{\st cp},a,p_{\st\mathcal S}, coin^{\st *}_{\st\mathcal C},coin^{\st *}_{\st\mathcal S})\rightarrow ({\bm{coin}}_{\st\mathcal C},{\bm{coin}}_{\st\mathcal S},{\bm{coin}}_{\st\mathcal{R}})$}: It is run by the smart contract. It takes as input the binary vectors $[\bm{y}_{\st \mathcal  C}, \bm{y}_{\st \mathcal  S},\bm{y}'_{\st \mathcal  C}, \bm{y}'_{\st \mathcal  S}]\in \bm{y}$ that indicate which party misbehaved, or sent invalid complaint  in each verification,   $T_{\st cp}:=\{cp,g_{\st cp}\}$,  $a$, the total coins the server should deposit $p_{\st\mathcal S}$, $coin^{\st *}_{\st\mathcal C}$, and $coin^{\st *}_{\st\mathcal S}$. If $a=1$ and  $coin^{\st *}_{\st\mathcal S}= p_{\st\mathcal S}$, then it verifies the validity of $T_{\st cp}$. If $T_{\st cp}$ is rejected, then it aborts. 
If it is accepted, then it constructs  vector ${\bm{coin}}_{\st\mathcal I}$, where $\mathcal{I}\in\{\mathcal{C},\mathcal{S},\mathcal{R}\}$; It sends ${{coin}}_{\st\mathcal{I},j}\in{\bm{coin}}_{\st\mathcal I}$ coins to party $\mathcal{I}$ for each $j$-th verification. Otherwise (i.e., $a=0$ or $coin^{\st *}_{\st\mathcal S}\neq p_{\st\mathcal S}$)  it  sends $coin^{\st *}_{\st\mathcal C}$ and  $coin^{\st *}_{\st\mathcal S}$ coins to $\mathcal C$ and $\mathcal S$ respectively. 	
%
\end{definition}

In the above definition, the algorithms $\mathtt{RCSP}.\mathtt{genQuery},\mathtt{RCSP}.\mathtt{prove},$ $\mathtt{RCSP}.\mathtt{verify}$ and $\mathtt{RCSP}.\mathtt{resolve}$ implicitly  take $a, coin^{\st*}_{\st\mathcal{S}}, p_{\st\mathcal{S}}$ as other inputs and  execute only if $a=1$ and $coin^{\st*}_{\st\mathcal{S}}=p_{\st\mathcal{S}}$; however, for the sake of simplicity we  avoided explicitly stating it  in the definition. 

An RC-S-P  scheme satisfies correctness and security. At a high level, correctness requires that by the end of the protocol's execution  (that involves  honest client and server) the client receives all $z$ valid service proofs while the server gets paid  for the proofs, without the involvement of the arbiter. More specifically, it requires that the server accepts an honest client's encoded data and query while the honest client accepts the server's valid service proof (and no one is identified as misbehaving party). Moreover, the honest client gets back all its deposited coins minus the service payment, the honest server gets back all its deposited coins  plus the service payment and the arbiter receives nothing. Correctness is formally stated below.



\begin{definition}[Correctness] \label{def::RC-S-P-Correctness} Am RC-S-P  scheme  is  correct   for  functions $F, Q,$ $ M, E, D$, and auxiliary information $\text{aux}_{\st 1},...,\text{aux}_{\st z}$,  if for any price list $pl$, and any service input $u$, it holds that the following probability is equal to $1$: %if $\mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, M,z,$ $pl,enc) \rightarrow (u^{\st *},e,T, p_{\st\mathcal S},  \bm{y},$ $coin^{\st*}_{\st\mathcal C})$,  $\mathtt{RCSP}.\mathtt{sInit} (u^{\st *},e, pk,z, T, p_{\st\mathcal S},\bm{y},enc)\rightarrow (coin^{\st *}_{\st\mathcal S},a)$,   $\forall j\in[z]: $\\ $\Big($$\mathtt{RCSP}.\mathtt{genQuery}(1^\lambda, \text{aux}_{\st j},k,Q, T_{\st qp},$ $ enc)\rightarrow c^{\st *}_{\st j}$, $\mathtt{RCSP}.\mathtt{prove}(u^{\st *},  \sigma,  c^{\st *}_{\st j},pk, T_{\st qp},enc)\rightarrow (b_{\st j},m_{\st\mathcal {S},j},\pi^{\st *}_{\st j})$, \\$\mathtt{RCSP}.\mathtt{verify}(\pi^{\st *}_{\st j}, c^{\st *}_{\st j},k,T_{\st qp},enc)\rightarrow (d_{\st j}, m_{\st\mathcal {C},j})$$\Big), \mathtt{RCSP}.\mathtt{resolve}(m_{\st \mathcal{C}},m_{\st \mathcal{S}},z, {\bm{\pi}}^{\st *}, {\bm{c}}^{\st *},pk, T_{\st qp},enc)\rightarrow \bm{y}$, \\$\mathtt{RCSP}.\mathtt{pay}(\bm{y},T_{\st cp},a,p_{\st\mathcal S}, coin^{\st *}_{\st\mathcal C},coin^{\st *}_{\st\mathcal S})\rightarrow (\bm{coin}_{\st\mathcal C},$ $\bm{coin}_{\st\mathcal S},$ $\bm{coin}_{\st\mathcal Ar})$, then $(a=1)\wedge (\bigwedge\limits^{\st z}_{\st j=1} b_{\st j}= \bigwedge\limits^{\st z}_{\st j=1} d_{\st j}=1)\wedge (\bm{y}_{\st \mathcal C}=\bm{y}_{\st \mathcal S}=\bm{y}'_{\st \mathcal C}=\bm{y}'_{\st \mathcal S}=0) \wedge (\sum\limits^{\st z}_{\st j=1}coin_{\st\mathcal C,j}=coin^{\st *}_{\st\mathcal C}-o\cdot z) \wedge  (\sum\limits^{\st z}_{\st j=1}coin_{\st\mathcal S,j}=coin^{\st *}_{\st\mathcal S}+o\cdot z)  \wedge (\sum\limits^{\st z}_{\st j=1}coin_{\st\mathcal Ar,j}=0)$, where $\bm{y}_{\st \mathcal C},\bm{y}_{\st \mathcal S},\bm{y}'_{\st \mathcal C},\bm{y}'_{\st \mathcal S}\in \bm{y}$.


\[
\Pr\left[{\scriptsize
\begin{array}{l}
\mathtt{RCSP}.\mathtt{keyGen}(1^\lambda, F)\rightarrow \bm{k}\\
%
\mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, M,z,$ $pl,enc) \rightarrow (u^{\st *},e,T, p_{\st\mathcal S},  \bm{y},$ $coin^{\st*}_{\st\mathcal C})\\
%
\mathtt{RCSP}.\mathtt{sInit} (u^{\st *},e, pk,z, T, p_{\st\mathcal S},\bm{y},enc)\rightarrow (coin^{\st *}_{\st\mathcal S},a)\\
%
\mathsf{For}\; j=1,\ldots,z\;\mathsf{do}: \\

\quad\mathtt{RCSP}.\mathtt{genQuery}(1^\lambda, \text{aux}_{\st j},k,Q, T_{\st qp}, enc)\rightarrow c^{\st *}_{\st j}\\
%
\quad\mathtt{RCSP}.\mathtt{prove}(u^{\st *},  \sigma,  c^{\st *}_{\st j},pk, T_{\st qp},enc)\rightarrow (b_{\st j},m_{\st\mathcal {S},j},\pi^{\st *}_{\st j})\\
%
\quad\mathtt{RCSP}.\mathtt{verify}(\pi^{\st *}_{\st j}, c^{\st *}_{\st j},k,T_{\st qp},enc)\rightarrow (d_{\st j}, m_{\st\mathcal {C},j})\\
%
\mathtt{RCSP}.\mathtt{resolve}(m_{\st \mathcal{C}},m_{\st \mathcal{S}},z, {\bm{\pi}}^{\st *}, {\bm{c}}^{\st *},pk, T_{\st qp},enc)\rightarrow \bm{y}\\
%
\mathtt{RCSP}.\mathtt{pay}(\bm{y},T_{\st cp},a,p_{\st\mathcal S}, coin^{\st *}_{\st\mathcal C},coin^{\st *}_{\st\mathcal S})\rightarrow (\bm{coin}_{\st\mathcal C},\bm{coin}_{\st\mathcal S},\bm{coin}_{\st\mathcal{R}})\\
%
\hline
%
(a=1)\wedge (\bigwedge\limits^{\st z}_{\st j=1} b_{\st j}= \bigwedge\limits^{\st z}_{\st j=1} d_{\st j}=1)\wedge (\bm{y}_{\st \mathcal C}=\bm{y}_{\st \mathcal S}=\bm{y}'_{\st \mathcal C}=\bm{y}'_{\st \mathcal S}=0) \wedge\\
%
(\sum\limits^{\st z}_{\st j=1}coin_{\st\mathcal C,j}=coin^{\st *}_{\st\mathcal C}-o\cdot z) \wedge  (\sum\limits^{\st z}_{\st j=1}coin_{\st\mathcal S,j}=coin^{\st *}_{\st\mathcal S}+o\cdot z)  \wedge (\sum\limits^{\st z}_{\st j=1}coin_{\st\mathcal{R},j}=0)\\
\end{array}
}\right]\]
\end{definition}
\noindent where $\bm{y}_{\st \mathcal C},\bm{y}_{\st \mathcal S},\bm{y}'_{\st \mathcal C},\bm{y}'_{\st \mathcal S}\in \bm{y}$.
%\textcolor{blue}{XXXX Thomas: something is not right in the definition of correctness... we write $\forall j$ but the execution of $\mathtt{RCSP}.\mathtt{genQuery}$ does not depend on $j$. Not sure how to fix it yet.XXXX}

An RC-S-P scheme is said to be secure if it satisfies  three main properties: (a)  security against  a malicious server, (b) security against a malicious client, and (c) privacy.  In the following, we formally define each of them.  Intuitively, security against a malicious server states that (at the end of the protocol execution) either (i) for each verification the client gets a valid proof and gets back its deposit minus the service payment, or (ii) the client gets its deposit back (for the $j$-th verification) and the arbiter receives $l$ coins, or (iii) if a malicious server unnecessarily invokes the arbiter, then it has to pay the arbiter. In particular, for each $j$-th verification, the security requires that only with a negligible probability the adversary wins, if it  provides either (a)  correct evaluation of the function on the service input but it either makes the client  withdraw an incorrect amount of coins (i.e., something other than its deposit minus service payment) or makes the arbiter withdraw an incorrect amount of coins if it unnecessarily invokes the arbiter, or (b) incorrect evaluation of the function on the service input,  but either persuades the client or the arbiter to accept it (i.e.,  $b_{\st j}=1$ or $y_{\st\mathcal S,j}=0$) or makes them  withdraw an incorrect amount of coins (i.e., $coin_{\st\mathcal{C},j}\neq \frac{coin_{\st\mathcal C}^{\st*}}{z}$ or  $coin_{\st\mathcal{R},j}\neq l$ coins).  Below, we formalize this intuition. 


\begin{definition}[Security Against Malicious Server]\label{deff::RC-S-P-SecurityAgainstMaliciousServer}  An RC-S-P scheme is secure against a malicious server for  functions $F,Q,M,E,D$, and an auxiliary information $aux$, if for  any price list $pl$, every $j$ (where $1\leq j\leq z$), and any PPT adversary $\mathcal{A}$,  it holds that the following probability is $\mathsf{negl}(\lambda)$:


\[ \Pr\left[{\scriptsize
  \begin{array}{l}
\mathtt{RCSP.keyGen}(1^{\lambda}, F)\rightarrow \bm{k}\\
%  
   \mathcal{A}(1^\lambda,pk, F)\rightarrow u\\
%   
   \mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, M,z,pl,enc)\rightarrow (u^{\st *},e,T, p_{\st\mathcal S},  \bm{y}, coin^{\st*}_{\st\mathcal C})\\
 %  
   \mathcal{A}(u^{\st *}, e, pk, z, T, p_{\st\mathcal S},\bm{y},enc)\rightarrow (coin^{\st *}_{\st\mathcal S},a)\\
  % 
 	\mathtt{RCSP}.\mathtt{genQuery}(1^\lambda, \text{aux},k,Q, T_{\st qp}, enc)\rightarrow c^{\st *}_{\st j}\\
  %
     \mathcal{A}(c^{\st *}_{\st j},\sigma, u^{\st *},enc,a)\rightarrow 
     (b_{\st j},m_{\st \mathcal{S},j},h^{\st *}_{\st j},\delta^{\st *}_{\st j})\\ 
  %   
 \mathtt{RCSP}.\mathtt{verify}(\pi^{\st *}_{\st j}, c^{\st *}_{\st j}, k,T_{\st qp},enc)\rightarrow (d_{\st j},m_{\st \mathcal{C},j})\\
%
   \mathtt{RCSP}.\mathtt{resolve}(m_{\st \mathcal{C}},m_{\st \mathcal{S}},z, {\bm{\pi}}^{\st *}, {\bm{c}}^{\st *},pk, T_{\st qp},enc)\rightarrow \bm{y}\\
  % 
   \mathtt{RCSP}.\mathtt{pay}(\bm{y},T_{\st cp},a,p_{\st\mathcal S}, coin^{\st *}_{\st\mathcal C},coin^{\st *}_{\st\mathcal S})\rightarrow ({\bm{coin}}_{\st\mathcal C},{\bm{coin}}_{\st\mathcal S},{\bm{coin}}_{\st\mathcal{R}})\\  
%
\hline  
%  
  \Big(F(u^{\st *}, \bm{q}_{\st j}, {pp})= h_{\st j} \wedge (coin_{\st\mathcal{C},j}\neq  \frac{coin_{\st\mathcal C}^{\st*}}{z}-o \vee  (coin_{\st\mathcal{R},j}\neq l\ \wedge\  y'_{\st \mathcal {S},j}=1))\Big)\ \vee\\ 
%
\Big(
F(u^{\st *},\bm{q}_{\st j}, {pp})\neq h_{\st j}  \wedge (d_{\st j}=1	\vee y_{\st \mathcal{S},j}=0  \vee coin_{\st\mathcal{C},j}\neq \frac{coin_{\st\mathcal C}^{\st*}}{z} \ \vee  coin_{\st\mathcal{R},j}\neq l) \Big)\\
%\text{s.t.}\\
%y_{\st j}= E^{\st -1}_{\st 2}(y^{\st *}_{\st j},t_{\st qp})\\
%E^{\st -1}_{\st 2},t_{\st qp}\in en\\
\end{array}
}    \right]\]

\noindent where  $\bm{q}_{\st j}\in D(c^{\st *}_{\st j},T_{\st qp})$, $\pi^{\st *}_{\st j}:=(h^{\st *}_{\st j}, \delta^{\st *}_{\st j}), h_{\st j}= D(h^{\st *}_{\st j},T_{\st qp})$, $
D\in enc$, $\sigma\in e$, $m_{\st \mathcal{C},j}\in m_{\st \mathcal{C}}, m_{\st \mathcal{S},j}\in m_{\st \mathcal{S}}, y'_{\st \mathcal{S},j}\in \bm{y}'_{\st \mathcal{S}}\in\bm{y}$,   $y_{\st \mathcal{S},j}\in \bm{y}_{\st \mathcal{S}}\in\bm{y}$, and $ {pp}\in T_{\st qp}$ %\TZ{The winning conditions formula does not read well.}



%Also, the probability is taken over uniform  choice of $k,k'\stackrel{\st\$}\leftarrow \{0,1\}^{\st\lambda}$, where $k,k'\in\bm{k}$, as well as the randomness of $\mathcal{A}$ and the randomness used in witnesses $g_{\st cp},g_{\st qp}\in t$.
\end{definition}





%
%\begin{definition}[RC-S-P Security Against Malicious Server]\label{deff::RC-S-P-SecurityAgainstMaliciousServer}  A RC-S-P  is secure against a malicious server for  functions $F,Q,M,D,E$, and an auxiliary information $aux$, if for  any price list $pl$, every $j$ (where $1\leq j\leq z$), and any PPT adversary $\mathcal{A}$, there exists a negligible function $\mu(\cdot)$, such that for any security parameter $\lambda$: 
%%\footnotesize{
%{\small
%$$ \Pr\left[
%  \begin{array}{l}
%  \Big(F(u^{\st *}, \bm{q}_{\st j}, {pp})= h_{\st j}\ \wedge\\ (coin_{\st\mathcal{C},j}\neq  \frac{coin_{\st\mathcal C}^{\st*}}{z}-o)\ \vee \\  (coin_{\st\mathcal{R},j}\neq l\ \wedge\  y'_{\st \mathcal {S},j}=1)\Big)\ \vee\\ 
%
%\Big(
%F(u^{\st *},\bm{q}_{\st j}, {pp})\neq h_{\st j} \ \wedge\\ (d_{\st j}=1	\vee y_{\st \mathcal{S},j}=0 \ \vee \\coin_{\st\mathcal{C},j}\neq \frac{coin_{\st\mathcal C}^{\st*}}{z} \ \vee  coin_{\st\mathcal{A}r,j}\neq l) \Big)\\
%%\text{s.t.}\\
%%y_{\st j}= E^{\st -1}_{\st 2}(y^{\st *}_{\st j},t_{\st qp})\\
%%E^{\st -1}_{\st 2},t_{\st qp}\in en\\
%\end{array} \middle |
%    \begin{array}{l}
%    \mathtt{RCSP.keyGen}(1^{\lambda}, F)\rightarrow \bm{k}\\
%    \mathcal{A}(1^\lambda,pk, F)\rightarrow u\\
%  
%    \mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, M,z,pl,enc)\rightarrow (u^{\st *},e,T, p_{\st\mathcal S},  \bm{y}, coin^{\st*}_{\st\mathcal C})\\
%    
%    \mathcal{A}(u^{\st *}, e, pk, z, T, p_{\st\mathcal S},\bm{y},enc)\rightarrow (coin^{\st *}_{\st\mathcal S},a)\\
%	\mathtt{RCSP}.\mathtt{genQuery}(1^\lambda, \text{aux},k,Q, T_{\st qp}, enc)\rightarrow c^{\st *}_{\st j}\\
%	
%     \mathcal{A}(c^{\st *}_{\st j},\sigma, u^{\st *},enc,a)\rightarrow 
%     (b_{\st j},m_{\st \mathcal{S},j},h^{\st *}_{\st j},\delta^{\st *}_{\st j})\\
%     
%     %(\pi^{\st *}_{\st j},b_{\st j})\\
%     
%\mathtt{RCSP}.\mathtt{verify}(\pi^{\st *}_{\st j}, c^{\st *}_{\st j}, k,T_{\st qp},enc)\rightarrow (d_{\st j},m_{\st \mathcal{C},j})\\
%   \mathtt{RCSP}.\mathtt{resolve}(m_{\st \mathcal{C}},m_{\st \mathcal{S}},z, {\bm{\pi}}^{\st *}, {\bm{c}}^{\st *},pk, T_{\st qp},enc)\rightarrow \bm{y}\\
%   
%   \mathtt{RCSP}.\mathtt{pay}(\bm{y},T_{\st cp},a,p_{\st\mathcal S}, coin^{\st *}_{\st\mathcal C},coin^{\st *}_{\st\mathcal S})\rightarrow ({\bm{coin}}_{\st\mathcal C},{\bm{coin}}_{\st\mathcal S},{\bm{coin}}_{\st\mathcal Ar})\\
%\end{array}    \right]\leq \mu(\lambda)$$
%}
%where  $\bm{q}_{\st j}\in D(c^{\st *}_{\st j},T_{\st qp})$, $\pi^{\st *}_{\st j}:=(h^{\st *}_{\st j}, \delta^{\st *}_{\st j}), h_{\st j}= D(h^{\st *}_{\st j},T_{\st qp})$, $
%D\in enc$, $\sigma\in e$, $m_{\st \mathcal{C},j}\in m_{\st \mathcal{C}}, m_{\st \mathcal{S},j}\in m_{\st \mathcal{S}}, y'_{\st \mathcal{S},j}\in \bm{y}'_{\st \mathcal{S}}\in\bm{y}$,   $y_{\st \mathcal{S},j}\in \bm{y}_{\st \mathcal{S}}\in\bm{y}$, and $ {pp}\in T_{\st qp}$. 
%
%
%
%%Also, the probability is taken over uniform  choice of $k,k'\stackrel{\st\$}\leftarrow \{0,1\}^{\st\lambda}$, where $k,k'\in\bm{k}$, as well as the randomness of $\mathcal{A}$ and the randomness used in witnesses $g_{\st cp},g_{\st qp}\in t$.
%\end{definition}
%





 
 
 
Informally, security against a malicious client requires that, for each  $j$-th verification, a malicious client with a negligible probability  wins if it provides either (a) valid metadata and query but either makes the server receive an incorrect amount of coins (something other than its deposit plus the service payment), or makes the arbiter withdraw incorrect amounts of coin if it unnecessarily invokes the arbiter  or (b) invalid metadata or query but convinces the server to accept either of them (i.e., the invalid metadata or query), or (c) invalid query but persuades the arbiter to accept it, or  makes them withdraw an incorrect amount of coins (i.e., $coin_{\st\mathcal{S},j}\neq \frac{coin_{\st\mathcal S}^{\st*}}{z}+o$ or  $coin_{\st\mathcal{R},j}\neq l$ coins). Below, we formally state the property. 
 

 
% 
% \begin{definition}[RC-S-P Security Against Malicious Client]\label{deff::RC-S-P-Security-Against Malicious-Client}  A RC-S-P  is secure against a malicious client  for functions $F,Q,M,D,E$, and an auxiliary information $aux$, if   for every $j$ (where $1\leq j\leq z$), and any probabilistic polynomial time adversary $\mathcal{A}$, there exists a negligible function $\mu(\cdot)$, such that for any security parameter $\lambda$: 
%
%
%{\small
%$$ \Pr\left[
%  \begin{array}{l}
% \Big((M(u^{\st *},k, {pp})= \sigma  \wedge Q(\text{aux},k, {pp})= \bm{q}_{\st j})\ \wedge\\
%  (coin_{\st\mathcal{S},j}\neq  \frac{coin_{\st\mathcal S}^{\st*}}{z}+o  \ \vee\\
% coin_{\st\mathcal{A}r,j}\neq l\ \wedge\  y'_{\st \mathcal {C},j}=1)\Big)\ \vee
%  \\
%  
%  
%  \Big(M(u^{\st *}, k,  {pp})\neq \sigma \wedge a=1\Big) \ \vee\\ 
%
%
%  \Big(Q(\text{aux},k,  {pp})\neq \bm{q}_{\st j}\ \wedge
%  (b_{\st j}=1 \ \vee \ y_{\st\mathcal{C},j}=0 \ \vee \\ coin_{\st\mathcal{S},j}\neq \frac{coin_{\st\mathcal S}^{\st*}}{z}+o \ \vee  coin_{\st\mathcal{A}r,j}\neq l) 
%  \Big)
% \\
% 
%\end{array} \middle |
%    \begin{array}{l}
%   \mathcal{A}(1^{\lambda}, F)\rightarrow (u^{\st *},z,\bm{k},e,T, pl, p_{\st\mathcal{S}}, coin^{\st*}_{\st\mathcal C},enc, \text{aux},\bm{y}, enc, pk)\\
%   
%   \mathtt{RCSP}.\mathtt{sInit}(u^{\st *}, e, pk, z, T, p_{\st\mathcal S},\bm{y},enc)\rightarrow (coin^{\st *}_{\st\mathcal S},a)\\
%   
%	\mathcal{A}(coin^{\st *}_{\st\mathcal S},a, 1^\lambda, \text{aux},k,Q, T_{\st qp}, enc)\rightarrow c^{\st *}_{\st j}\\
%
%     \mathtt{RCSP}.\mathtt{prove}(u^{\st *},  \sigma,  c^{\st *}_{\st j}, pk, T_{\st qp},enc)\rightarrow (b_{\st j},m_{\st \mathcal{S},j},\pi^{\st *}_{\st j})\\
%     
% \mathcal{A}(\pi^{\st *}_{\st j}, c^{\st *}_{\st j}, k, T_{\st qp},enc)\rightarrow (d_{\st j},m_{\st \mathcal{S},j})\\
%   
%   
%   \mathtt{RCSP}.\mathtt{resolve}(m_{\st \mathcal{C}},m_{\st \mathcal{S}},z, {\bm{\pi}}^{\st *}, {\bm{c}}^{\st *}, pk, T_{\st qp},enc)\rightarrow \bm{y}\\
%   \mathtt{RCSP}.\mathtt{pay}(\bm{y},T_{\st cp},a,p_{\st\mathcal S}, coin^{\st *}_{\st\mathcal C},coin^{\st *}_{\st\mathcal S})\rightarrow ({\bm{coin}}_{\st\mathcal C},{\bm{coin}}_{\st\mathcal S},{\bm{coin}}_{\st\mathcal Ar})\\
%\end{array}    \right]\leq \mu(\lambda)$$
%}
%where $\bm{q}_{\st j}\in D(c^{\st *}_{\st j},t_{\st qp})$, $
%D\in enc$, $\sigma\in e$, $y'_{\st \mathcal{C},j}\in \bm{y}'_{\st \mathcal{C}}\in\bm{y}$,   $y_{\st \mathcal{C},j}\in \bm{y}_{\st \mathcal{C}}\in\bm{y}$, and ${pp}\in T_{\st qp}$.  
%
%
%
%%Moreover,  the probability is taken over the randomness used in witnesses $g_{\st cp},g_{\st qp}\in t$ as well as  the randomness used in proofs $\bm{w}_{\st q_{_{\scaleto{j}{\size}}}}\in c_{\st j}$ and $w_{\st\sigma}\in e$ and  the randomness of $\mathcal{A}$.
%\end{definition}
 



 \begin{definition}[Security Against Malicious Client]\label{deff::RC-S-P-Security-Against Malicious-Client}  An RC-S-P scheme  is secure against a malicious client  for functions $F,Q,M,E,D$, and an auxiliary information $aux$, if   for every $j$ (where $1\leq j\leq z$), and any probabilistic polynomial time adversary $\mathcal{A}$, it holds that the following probability is $\mathsf{negl}(\lambda)$:
 % 


\[\Pr\left[{\scriptsize
  \begin{array}{l}
\mathcal{A}(1^{\lambda}, F)\rightarrow (u^{\st *},z,\bm{k},e,T, pl, p_{\st\mathcal{S}}, coin^{\st*}_{\st\mathcal C},enc, \text{aux},\bm{y}, enc, pk)\\
   %
  \mathtt{RCSP}.\mathtt{sInit}(u^{\st *}, e, pk, z, T, p_{\st\mathcal S},\bm{y},enc)\rightarrow (coin^{\st *}_{\st\mathcal S},a)\\
   %
	\mathcal{A}(coin^{\st *}_{\st\mathcal S},a, 1^\lambda, \text{aux},k,Q, T_{\st qp}, enc)\rightarrow c^{\st *}_{\st j}\\
%
     \mathtt{RCSP}.\mathtt{prove}(u^{\st *},  \sigma,  c^{\st *}_{\st j}, pk, T_{\st qp},enc)\rightarrow (b_{\st j},m_{\st \mathcal{S},j},\pi^{\st *}_{\st j})\\
    % 
  \mathcal{A}(\pi^{\st *}_{\st j}, c^{\st *}_{\st j}, k, T_{\st qp},enc)\rightarrow (d_{\st j},m_{\st \mathcal{S},j})\\
   %
   \mathtt{RCSP}.\mathtt{resolve}(m_{\st \mathcal{C}},m_{\st \mathcal{S}},z, {\bm{\pi}}^{\st *}, {\bm{c}}^{\st *}, pk, T_{\st qp},enc)\rightarrow \bm{y}\\
 %  
 \mathtt{RCSP}.\mathtt{pay}(\bm{y},T_{\st cp},a,p_{\st\mathcal S}, coin^{\st *}_{\st\mathcal C},coin^{\st *}_{\st\mathcal S})\rightarrow ({\bm{coin}}_{\st\mathcal C},{\bm{coin}}_{\st\mathcal S},{\bm{coin}}_{\st\mathcal{R}})\\
 %
 \hline
 %
 \Big((M(u^{\st *},k, {pp})= \sigma \ \wedge Q(\text{aux},k, {pp})= \bm{q}_{\st j})\ \wedge\\
  (coin_{\st\mathcal{S},j}\neq  \frac{coin_{\st\mathcal S}^{\st*}}{z}+o  \ \vee
 coin_{\st\mathcal{R},j}\neq l\ \wedge\  y'_{\st \mathcal {C},j}=1)\Big)\ \vee
  \\
  
  \Big(M(u^{\st *}, k,  {pp})\neq \sigma \wedge a=1\Big) \ \vee

  \Big(Q(\text{aux},k,  {pp})\neq \bm{q}_{\st j}\ \wedge
  (b_{\st j}=1 \ \vee\\ \ y_{\st\mathcal{C},j}=0 \ \vee  coin_{\st\mathcal{S},j}\neq \frac{coin_{\st\mathcal S}^{\st*}}{z}+o \ \vee  coin_{\st\mathcal{R},j}\neq l) 
  \Big)
 \\
 
\end{array}    }\right]\]

\noindent where $\bm{q}_{\st j}\in D(c^{\st *}_{\st j},t_{\st qp})$, $
D\in enc$, $\sigma\in e$, $y'_{\st \mathcal{C},j}\in \bm{y}'_{\st \mathcal{C}}\in\bm{y}$,   $y_{\st \mathcal{C},j}\in \bm{y}_{\st \mathcal{C}}\in\bm{y}$, and ${pp}\in T_{\st qp}$.  



%Moreover,  the probability is taken over the randomness used in witnesses $g_{\st cp},g_{\st qp}\in t$ as well as  the randomness used in proofs $\bm{w}_{\st q_{_{\scaleto{j}{\size}}}}\in c_{\st j}$ and $w_{\st\sigma}\in e$ and  the randomness of $\mathcal{A}$.
\end{definition}
 







 Note, in the above definition, an honest server either does not deposit (e.g., when $a=0$) or if it deposits (i.e., agrees to serve) ultimately receives its deposit \emph{plus the service payment} (with a high probability). Informally, RC-S-P is privacy-preserving if it guarantees the privacy of (1) the service input (e.g., outsourced file) and (2) the service proof's status during the private time bubble. In the following, we formally define privacy.
 

%  \begin{definition}[RC-S-P Privacy]\label{deff::RC-S-P-Privacy}  A RC-S-P   preserves privacy, for functions $F, Q, M, E, D$, and   auxiliary information $\text{aux}_{\st 1},...,\text{aux}_{\st z}$, if for any number of verifications $z$, any price list $pl$,  the following hold:
%  
%
%  
%  \begin{enumerate}
%\item For any PPT adversary $\mathcal{A}_{\st 1}$ there exists a negligible function $\mu(\cdot)$, such that for any security parameter $\lambda$:
%  
%{\small
%$$\Pr\left[
%  \begin{array}{l}
%  \mathcal{A}_{\st 1}(\bm{c}^{\st *},coin^{\st *}_{\st\mathcal S},coin^{\st *}_{\st\mathcal  C}, g_{\st cp}, \\ g_{\st qp}, \bm{\pi}^{\st *}, pl, a)\rightarrow\beta\\
%\end{array} \middle |
%    \begin{array}{l}
%            \mathtt{RCSP.keyGen}(1^{\lambda}, F)\rightarrow \bm{k}\\
%        \mathcal{A}_{\st 1}(1^\lambda, pk, F)\rightarrow (u_{\st 0},u_{\st 1})\\
%
%
%    \beta\stackrel{\st\$}\leftarrow\{0,1\}\\
%
%   \mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u_{\st\beta},\bm{k}, M,z,pl,enc)\rightarrow (u^{\st *}_{\st\beta},e,T, p_{\st\mathcal S},  \bm{y}, coin^{\st*}_{\st\mathcal C})\\
%\mathtt{RCSP}.\mathtt{sInit}(u_{\st\beta}^{\st *}, e, pk, z, T, p_{\st\mathcal S},\bm{y},enc)\rightarrow (coin^{\st *}_{\st\mathcal S},a)\\
%
%\forall j \in [z]:\\
%
%\Big(\mathtt{RCSP}.\mathtt{genQuery}(1^\lambda, \text{aux}_{\st j},k,Q, T_{\st qp}, enc)\rightarrow c^{\st *}_{\st j}\\
%     \mathtt{RCSP}.\mathtt{prove}(u^{\st *}_{\st\beta},   \sigma,  c^{\st *}_{\st j}, pk, T_{\st qp},enc)\rightarrow (b_{\st j},m_{\st \mathcal{S},j},\pi^{\st *}_{\st j})\\  
%   \mathtt{RCSP}.\mathtt{verify}(\pi^{\st *}_{\st j}, c^{\st *}_{\st j}, k,T_{\st qp},enc)\rightarrow (d_{\st j},m_{\st \mathcal{C},j})\Big)\\
%\end{array}\right]\leq \frac{1}{2}+\mu(\lambda).$$
%}
%


  \begin{definition}[Privacy]\label{deff::RC-S-P-Privacy}  An RC-S-P scheme  preserves privacy for functions $F, Q, M, E, D$, and   auxiliary information $\text{aux}_{\st 1},...,\text{aux}_{\st z}$, if for any price list $pl$,  the following hold:
  

  
  \begin{enumerate}
\item For any PPT adversary $\mathcal{A}_{\st 1}$, it holds that the following probability is no more than $\frac{1}{2}+\mathsf{negl}(\lambda)$.
  
\[\Pr\left[{\scriptsize
  \begin{array}{l}
   \mathtt{RCSP.keyGen}(1^{\lambda}, F)\rightarrow \bm{k}\\
%
         \mathcal{A}_{\st 1}(1^\lambda, pk, F)\rightarrow (u_{\st 0},u_{\st 1})\\
 %
     \beta\stackrel{\st\$}\leftarrow\{0,1\}\\
 %
    \mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u_{\st\beta},\bm{k}, M,z,pl,enc)\rightarrow (u^{\st *}_{\st\beta},e,T, p_{\st\mathcal S},  \bm{y}, coin^{\st*}_{\st\mathcal C})\\
 %
  \mathtt{RCSP}.\mathtt{sInit}(u_{\st\beta}^{\st *}, e, pk, z, T, p_{\st\mathcal S},\bm{y},enc)\rightarrow (coin^{\st *}_{\st\mathcal S},a)\\
%
\mathsf{For}\; j=1,\ldots,z\;\mathsf{do}: \\
%
  \quad\mathtt{RCSP}.\mathtt{genQuery}(1^\lambda, \text{aux}_{\st j},k,Q, T_{\st qp}, enc)\rightarrow c^{\st *}_{\st j}\\
%
   \quad  \mathtt{RCSP}.\mathtt{prove}(u^{\st *}_{\st\beta},   \sigma,  c^{\st *}_{\st j}, pk, T_{\st qp},enc)\rightarrow (b_{\st j},m_{\st \mathcal{S},j},\pi^{\st *}_{\st j})\\  
 %
  \quad\mathtt{RCSP}.\mathtt{verify}(\pi^{\st *}_{\st j}, c^{\st *}_{\st j}, k,T_{\st qp},enc)\rightarrow (d_{\st j},m_{\st \mathcal{C},j})\\ 
 %
 \hline
 % 
  \mathcal{A}_{\st 1}(\bm{c}^{\st *},coin^{\st *}_{\st\mathcal S},coin^{\st *}_{\st\mathcal  C}, g_{\st cp}, g_{\st qp}, \bm{\pi}^{\st *}, pl, a)\rightarrow\beta\\
\end{array}}\right]\]
\noindent where   $\bm{c}^{\st *}=[{c}^{\st *}_{\st 1},...,{c}^{\st *}_{\st z}]$ and $\bm{\pi}^{\st *}=[\pi^{\st *}_{\st 1},...,\pi^{\st *}_{\st z}]$.


\item For any PPT adversaries $\mathcal{A}_{\st 2}$ and $\mathcal{A}_{\st 3}$, it holds that the following probability is no more than $Pr_\mathrm{max}+\mathsf{negl}(\lambda)$:

%

\[\Pr\left[{\scriptsize
  \begin{array}{l}
  \mathtt{RCSP.keyGen}(1^{\lambda}, F)\rightarrow \bm{k}\\
%
  \mathcal{A}_{\st 2}(1^\lambda, pk, F)\rightarrow u\\
%
    \mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, M,z,pl,enc)\rightarrow (u^{\st *},e,T, p_{\st\mathcal S},  \bm{y}, coin^{\st*}_{\st\mathcal C})\\
 %
 \mathtt{RCSP}.\mathtt{sInit}(u^{\st *}, e, pk, z, T, p_{\st\mathcal S},\bm{y},enc)\rightarrow (coin^{\st *}_{\st\mathcal S},a)\\
%
\mathsf{For}\; j=1,\ldots,z\;\mathsf{do}: \\

  \quad\mathcal{A}_{\st 2}(1^\lambda, \text{aux}_{\st j},k,{Q}, T_{\st qp}, enc)\rightarrow c^{\st *}_{\st j}\\
%
     \quad \mathtt{RCSP}.\mathtt{prove}(u^{\st *},   \sigma,  c^{\st *}_{\st j}, pk, T_{\st qp},enc)\rightarrow (b_{\st j},m_{\st \mathcal{S},j},\pi^{\st *}_{\st j})\\  
 %
   \quad \mathtt{RCSP}.\mathtt{verify}(\pi^{\st *}_{\st j}, c^{\st *}_{\st j}, k,T_{\st qp},enc)\rightarrow (d_{\st j},m_{\st \mathcal{C},j})\\
  %
  \hline
  %
  \mathcal{A}_{\st 3}(\bm{c}^{\st *},coin^{\st *}_{\st\mathcal S},coin^{\st *}_{\st\mathcal  C}, g_{\st cp}, g_{\st qp}, \bm{\pi}^{\st *}, pl, a)\rightarrow(d_{\st j},j)\\
\end{array} }\right]\]





\noindent where  $Pr_\mathrm{max}$ is defined  as follows. Let  $Exp_{\st\mathsf{priv}}^{\st\mathcal{A}_2}(1^{\st \lambda})$ be the above experiment. Let  $\bm{q}_{\st j}\in D(c^{\st *}_{\st j},T_{\st qp})$, $ {pp}\in T_{\st qp}$. We define the events $Con_{\st 0,j}^{\st (1)}:Q(\text{aux}_{\st j}, k, pp)\neq \bm{q}_{\st j}$, $ Con_{\st 0,j}^{\st (2)}:b_{\st j}=0, Con_{\st 1,j}^{\st (1)}:Q(\text{aux}_{\st j}, k, pp)= \bm{q}_{\st j}$, and $ Con_{\st 1,j}^{\st (2)}:b_{\st j}=1$. For $i\in\{0,1\}$ and $j\in[z]$, we define  
%
\[Pr_{\st i,j}:=\Pr\left[{\scriptsize
\begin{array}{l}
\hspace{3mm}Exp_{\st\mathsf{priv}}^{\st\mathcal{A}_2}(1^{\st \lambda})\\
%%%%%%%%%
%  \mathtt{RCSP.keyGen}(1^{\lambda}, F)\rightarrow \bm{k}\\
%%
%  \mathcal{A}_{\st 2}(1^\lambda, pk, F)\rightarrow u\\
%%
%    \mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, M,z,pl,enc)\rightarrow (u^{\st *},e,T, p_{\st\mathcal S},  \bm{y}, coin^{\st*}_{\st\mathcal C})\\
% %
% \mathtt{RCSP}.\mathtt{sInit}(u^{\st *}, e, pk, z, T, p_{\st\mathcal S},\bm{y},enc)\rightarrow (coin^{\st *}_{\st\mathcal S},a)\\
%%
%\ \  \forall j \in [z]:\\
%
%  \Big(\mathcal{A}_{\st 2}(1^\lambda, \text{aux}_{\st j},k,{Q}, T_{\st qp}, enc)\rightarrow c^{\st *}_{\st j}\\
%%
%      \mathtt{RCSP}.\mathtt{prove}(u^{\st *},   \sigma,  c^{\st *}_{\st j}, pk, T_{\st qp},enc)\rightarrow (b_{\st j},m_{\st \mathcal{S},j},\pi^{\st *}_{\st j})\\  
% %
%    \mathtt{RCSP}.\mathtt{verify}(\pi^{\st *}_{\st j}, c^{\st *}_{\st j}, k,T_{\st qp},enc)\rightarrow (d_{\st j},m_{\st \mathcal{C},j})\Big)\\
%  %
%  %%%%%
  \hline
  %
Con_{\st i,j}^{\st (1)} \ \wedge \ Con_{\st i,j}^{\st (2)}\end{array}}\right].\]
%
%$$Pr_{\st i,j}=Pr[Con_{\st i,j}^{\st (1)} \ \wedge \ Con_{\st i,j}^{\st (2)}], \mbox{  and } i\in\{0,1\}.$$ 
%
Then, we have  $Pr_\mathrm{max}:=\mathrm{max}\{Pr_{\st 0,1},Pr_{\st 1,1},..., Pr_{\st 0,z},Pr_{\st 1,z}\}$.
 




%\item For any PPT adversaries $\mathcal{A}_{\st 2}$ and $\mathcal{A}_{\st 3}$ there exists a negligible function $\mu(\cdot)$ such that for any security parameter $\lambda$:
%
%
%{\small
%$$\Pr\left[
%  \begin{array}{l}
%  \mathcal{A}_{\st 3}(\bm{c}^{\st *},coin^{\st *}_{\st\mathcal S},coin^{\st *}_{\st\mathcal  C}, g_{\st cp}, \\ g_{\st qp}, \bm{\pi}^{\st *}, pl, a)\rightarrow(d_{\st j},j)\\
%\end{array} \middle |
%    \begin{array}{l}
%            \mathtt{RCSP.keyGen}(1^{\lambda}, F)\rightarrow \bm{k}\\
%        \mathcal{A}_{\st 2}(1^\lambda, pk, F)\rightarrow u\\
%
%
%   \mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, M,z,pl,enc)\rightarrow (u^{\st *},e,T, p_{\st\mathcal S},  \bm{y}, coin^{\st*}_{\st\mathcal C})\\
%\mathtt{RCSP}.\mathtt{sInit}(u^{\st *}, e, pk, z, T, p_{\st\mathcal S},\bm{y},enc)\rightarrow (coin^{\st *}_{\st\mathcal S},a)\\
%
%\forall j \in [z]:\\
%
%\Big(\mathcal{A}_{\st 2}(1^\lambda, \text{aux}_{\st j},k,{Q}, T_{\st qp}, enc)\rightarrow c^{\st *}_{\st j}\\
%     \mathtt{RCSP}.\mathtt{prove}(u^{\st *},   \sigma,  c^{\st *}_{\st j}, pk, T_{\st qp},enc)\rightarrow (b_{\st j},m_{\st \mathcal{S},j},\pi^{\st *}_{\st j})\\  
%   \mathtt{RCSP}.\mathtt{verify}(\pi^{\st *}_{\st j}, c^{\st *}_{\st j}, k,T_{\st qp},enc)\rightarrow (d_{\st j},m_{\st \mathcal{C},j})\Big)\\
%\end{array}\right]\leq Pr'+\mu(\lambda)$$
%}
%
%
%
%
%where   $\bm{c}^{\st *}=[{c}^{\st *}_{\st 1},...,{c}^{\st *}_{\st z}], \bm{\pi}^{\st *}=[\pi^{\st *}_{\st 1},...,\pi^{\st *}_{\st z}]$, and $Pr'$ is defined  as follows. Let  $\bm{q}_{\st j}\in D(c^{\st *}_{\st j},T_{\st qp})$  and $ {pp}\in T_{\st qp}$. Let $Con_{\st 0,j}^{\st (1)}:Q(\text{aux}_{\st j}, k, pp)\neq \bm{q}_{\st j}$ and  $ Con_{\st 0,j}^{\st (2)}:b_{\st j}=0, Con_{\st 1,j}^{\st (1)}:Q(\text{aux}_{\st j}, k, pp)= \bm{q}_{\st j}$,  $ Con_{\st 1,j}^{\st (2)}:b_{\st j}=1$. For $i\in\{0,1\}$ and $j\in[z]$, we define  
%
%$$Pr_{\st i,j}:=\Pr\left[
%Con_{\st i,j}^{\st (1)} \ \wedge \ Con_{\st i,j}^{\st (2)} \middle |
%    \begin{array}{l}
%            \mathtt{RCSP.keyGen}(1^{\lambda}, F)\rightarrow \bm{k}\\
%        \mathcal{A}_{\st 2}(1^\lambda, pk, F)\rightarrow u\\
%
%
%   \mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, M,z,pl,enc)\rightarrow (u^{\st *},e,T, p_{\st\mathcal S},  \bm{y}, coin^{\st*}_{\st\mathcal C})\\
%\mathtt{RCSP}.\mathtt{sInit}(u^{\st *}, e, pk, z, T, p_{\st\mathcal S},\bm{y},enc)\rightarrow (coin^{\st *}_{\st\mathcal S},a)\\
%
%\forall j \in [z]:\\
%
%\Big(\mathcal{A}_{\st 2}(1^\lambda, \text{aux}_{\st j},k,{Q}, T_{\st qp}, enc)\rightarrow c^{\st *}_{\st j}\\
%     \mathtt{RCSP}.\mathtt{prove}(u^{\st *},   \sigma,  c^{\st *}_{\st j}, pk, T_{\st qp},enc)\rightarrow (b_{\st j},m_{\st \mathcal{S},j},\pi^{\st *}_{\st j})\\  
%   \mathtt{RCSP}.\mathtt{verify}(\pi^{\st *}_{\st j}, c^{\st *}_{\st j}, k,T_{\st qp},enc)\rightarrow (d_{\st j},m_{\st \mathcal{C},j})\Big)\\
%\end{array}\right].$$
%
%
%
%Then, we have  $Pr':=Max\{Pr_{\st 0,1},Pr_{\st 1,1},..., Pr_{\st 0,z},Pr_{\st 1,z}\}$.
% 


%
%{\small
%$$ 
%  \begin{array}{l}
%
%\end{array} 
%    \begin{array}{l}
%            \mathtt{RCSP.keyGen}(1^{\lambda}, F)\rightarrow \bm{k}\\
%        \mathcal{A}_{\st 2}(1^\lambda, pk, F)\rightarrow u\\
%
%
%
%
%   \mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, M,z,pl,enc)\rightarrow (u^{\st *},e,T, p_{\st\mathcal S},  \bm{y}, coin^{\st*}_{\st\mathcal C})\\
%\mathtt{RCSP}.\mathtt{sInit}(u^{\st *}, e, pk, z, T, p_{\st\mathcal S},\bm{y},enc)\rightarrow (coin^{\st *}_{\st\mathcal S},a)\\
%
%\forall j \in [z]:\\
%
%\Big(\mathcal{A}_{\st 2}(1^\lambda, \text{aux}_{\st j},k,{Q}, T_{\st qp}, enc)\rightarrow c^{\st *}_{\st j}\\
%     \mathtt{RCSP}.\mathtt{prove}(u^{\st *},   \sigma,  c^{\st *}_{\st j}, pk, T_{\st qp},enc)\rightarrow (b_{\st j},m_{\st \mathcal{S},j},\pi^{\st *}_{\st j})\\  
%   \mathtt{RCSP}.\mathtt{verify}(\pi^{\st *}_{\st j}, c^{\st *}_{\st j}, k,T_{\st qp},enc)\rightarrow (d_{\st j},m_{\st \mathcal{C},j})\Big)\\
%\end{array}$$
%}




%{\small
%$$ Pr_{\st i}=\Pr\left[
%  \begin{array}{l}
%Con_{\st i}^{(\st 1)}\wedge  Con_{\st i}^{(\st 2)}
%  
%  \\
%\end{array} \middle |
%    \begin{array}{l}
%            \mathtt{RCSP.keyGen}(1^{\lambda}, F)\rightarrow \bm{k}\\
%        \mathcal{A}_{\st 2}(1^\lambda, pk, F)\rightarrow u\\
%
%
%
%
%   \mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, M,z,pl,enc)\rightarrow (u^{\st *},e,T, p_{\st\mathcal S},  \bm{y}, coin^{\st*}_{\st\mathcal C})\\
%\mathtt{RCSP}.\mathtt{sInit}(u^{\st *}, e, pk, z, T, p_{\st\mathcal S},\bm{y},enc)\rightarrow (coin^{\st *}_{\st\mathcal S},a)\\
%
%\forall j \in [z]:\\
%
%\Big(\mathcal{A}_{\st 2}(1^\lambda, \text{aux}_{\st j},k,{Q}, T_{\st qp}, enc)\rightarrow c^{\st *}_{\st j}\\
%     \mathtt{RCSP}.\mathtt{prove}(u^{\st *},   \sigma,  c^{\st *}_{\st j}, pk, T_{\st qp},enc)\rightarrow (b_{\st j},m_{\st \mathcal{S},j},\pi^{\st *}_{\st j})\\  
%   \mathtt{RCSP}.\mathtt{verify}(\pi^{\st *}_{\st j}, c^{\st *}_{\st j}, k,T_{\st qp},enc)\rightarrow (d_{\st j},m_{\st \mathcal{C},j})\Big)\\
%\end{array}\right]$$
%}




%{\small
%$$ Pr_{\st i}=\Pr\left[
%  \begin{array}{l}
%Con_{\st i}^{(\st 1)}\wedge  Con_{\st i}^{(\st 2)}
%  
%  \\
%\end{array} \middle |
%    \begin{array}{l}
%            \mathtt{RCSP.keyGen}(1^{\lambda}, F)\rightarrow \bm{k}\\
%        \mathcal{A}_{\st 2}(1^\lambda, pk, F)\rightarrow u\\
%
%
%
%
%   \mathtt{RCSP}.\mathtt{cInit}(1^\lambda, u,\bm{k}, M,z,pl,enc)\rightarrow (u^{\st *},e,T, p_{\st\mathcal S},  \bm{y}, coin^{\st*}_{\st\mathcal C})\\
%\mathtt{RCSP}.\mathtt{sInit}(u^{\st *}, e, pk, z, T, p_{\st\mathcal S},\bm{y},enc)\rightarrow (coin^{\st *}_{\st\mathcal S},a)\\
%
%%\forall j \in [z]:\\
%
%\mathcal{A}_{\st 2}(1^\lambda, \text{aux},k,{Q}, T_{\st qp}, enc)\rightarrow c^{\st *}_{\st j}\\
%     \mathtt{RCSP}.\mathtt{prove}(u^{\st *},   \sigma,  c^{\st *}_{\st j}, pk, T_{\st qp},enc)\rightarrow (b_{\st j},m_{\st \mathcal{S},j},\pi^{\st *}_{\st j})\\  
%   \mathtt{RCSP}.\mathtt{verify}(\pi^{\st *}_{\st j}, c^{\st *}_{\st j}, k,T_{\st qp},enc)\rightarrow (d_{\st j},m_{\st \mathcal{C},j})\\
%\end{array}\right]$$
%}


%$\text{ such that }   \bm{q}_{\st j}\in D(c^{\st *}_{\st j},t_{\st qp})$. Let $Con_{\st 0,j}^{\st (1)}:Q(aux_{\st j}, k, pp)\neq \bm{q}_{\st j},  Con_{\st 0,j}^{\st (2)}:b_{\st j}=0, Con_{\st 1,j}^{\st (1)}:Q(aux_{\st j}, k, pp)= \bm{q}_{\st j}$,  $ Con_{\st 1,j}^{\st (2)}:b_{\st j}=1$,   $Pr_{\st i,j}=Pr[Con_{\st i,j}^{\st (1)} \ \wedge \ Con_{\st i,j}^{\st (2)}]$, and $i\in\{1,2\}$. Then, $Pr'$ is defined as follows: $Pr'=Max([Pr_{\st i,j}])$.  

\end{enumerate}
\end{definition}
 
Note that in the above definition, for each $j$-th verification, adversary $\mathcal{A}_{\st 2}$ with probability $Pr_{\st 0,j}$ produces an invalid query  and with probability $Pr_{\st 1,j}$ produces a valid query. It is required that  the privacy holds regardless of the queries and proofs  status, i.e., whether they are valid or invalid, as long as they are correctly encoded and provided. In the above definitions, the private time bubble is a time period from the point when $\mathtt{RCSP.keyGen}(.)$ is executed up to the time  when $\mathtt{RCSP}.\mathtt{resolve}(.)$  is run. In other words, the privacy holds up to the point where $\mathtt{RCSP}.\mathtt{resolve}(.)$  is run. That is why the latter algorithm is excluded from the  experiments in Definition \ref{deff::RC-S-P-Privacy}. 
 
 
 \begin{definition}[RC-S-P Security]\label{def::RC-S-P-Security} An RC-S-P scheme is secure if it satisfies security against malicious server, security against malicious client, and preserves privacy, w.r.t. Definitions \ref{deff::RC-S-P-SecurityAgainstMaliciousServer}-\ref{deff::RC-S-P-Privacy}. 
 \end{definition}
 

 In Appendix \ref{app::RC-S-P}, we present a \emph{generic} RC-S-P construction that realises the above definition and prove its security. 
 


==> RCPoRP-without-Arbiter-Proof.tex <==
% !TEX root =main.tex

 \begin{lemma}
 If SAP and blockchain are secure and  PoRID scheme supports correctness, soundness, and detectable abort, then ${\text{RC-}\overline{\text{PoR}}\text{-P}}$ is secure against malicious server, w.r.t. Definition \ref{deff::RC-S-P-SecurityAgainstMaliciousServer-2}. 
 \end{lemma}
 

 \begin{proof}
 First, we  consider event  
 %
  $$\Big(F(u^{\st *}, \bm{q}_{\st j},{pp})= h_{\st j}\ \wedge (coin_{\st\mathcal{C},j}\neq  \frac{coin_{\st\mathcal C}^{\st*}}{z}-o)\Big)$$
   that captures the case where the server provides an accepting  proof, i.e. PoR, but makes an honest client withdraw  incorrect amounts of coin, i.e., $coin_{\st\mathcal{C},j}\neq  \frac{coin_{\st\mathcal C}^{\st*}}{z}-o$. Note, in ${\text{RC-}\overline{\text{PoR}}\text{-P}}$ protocol, the total coins the client should receive after $z$ verifications is   $coin^{\st *}_{\st\mathcal C}-o\cdot(z-y_{\st\mathcal S})+l\cdot(y_{\st\mathcal S}-y_{\st\mathcal C})$. Since we focus on  $j$-th verification, the amounts of  coin that should be credited to the client for the $j$-th verification is
 %
% 
% $F(u^{\st *},\bm{q}_{\st j})= h_{\st j}\ \wedge coin_{\st\mathcal{C},j}\neq  \frac{coin_{\st\mathcal C}^{\st*}}{z}-o$ that captures the case where the server provides an accepting service proof but makes an honest client withdraw an incorrect amounts of coin, i.e. $coin_{\st\mathcal{C},j}\neq  \frac{coin_{\st\mathcal C}^{\st*}}{z}-o$. Recall, in the protocol, the total coins the client should receive after $z$ verifications is $coin^{\st *}_{\st\mathcal C}-o(z-y_{\st\mathcal S})-l\cdot y_{\st\mathcal C}$. Since we focus on  $j$-th verification, the amount of  coins that should be credited to the client for that verification is
  %
  \begin{equation}\label{equ::what-client-recives-in-j-2}
   coin_{\st\mathcal{C},j}=\frac{coin^{\st *}_{\st\mathcal C}}{z}-o\cdot(1-y_{\st\mathcal {S},j})+l\cdot(y_{\st\mathcal {S},j}-y_{\st\mathcal {C},j})
     \end{equation}

    
As the  proof is valid, an honest client accepts it and does not raise any dispute. But, the server  would be able to make the client  withdraw incorrect amounts of coin, if it manages to either convince the contract that the client has misbehaved, by making the contract output  $y_{\st\mathcal {C},j}=1$ through the dispute resolution phase, or submit to the contract, in the coin transfer phase,  an accepting  statement $\ddot{x}'_{\st cp}$ other than what was agreed in the initiation phase, i.e., $\ddot{x}'_{\st cp}\neq\ddot{x}_{\st cp}$, so it can change the payments' parameters, e.g., $l$ or $o$. Nevertheless, it cannot falsely accuse the client of misbehaviour. As,  due to the security of SAP, it cannot  convince the contract to accept different query's parameters other than what was agreed with the client in the initiation phase. In particular, it cannot persuade the contract to accept  $\ddot{x}'_{\st qp}$ such that $\ddot{x}'_{\st qp}\neq \ddot{x}_{\st qp}$, except with a negligible probability, $\mu(\lambda)$.  Furthermore, if the adversary provides a valid statement then, then due to the correctness of the PoR and query-checking
process, values  $y_{\st\mathcal {C}}$ and $y_{\st\mathcal {S}}$ are not incremented by $1$  in the $j$-th verification, i.e., $y_{\st\mathcal{C},j}=y_{\st\mathcal{S},j}=0$. Also,  due to the security of SAP, the server cannot change the payment parameters by persuading the contract to accept any statement $\ddot{x}'_{\st cp}$ other than what was agreed initially between the client and server, except with a negligible probability $\mu(\lambda)$.  Therefore, according to Equation \ref{equ::what-client-recives-in-j-2}, the client is credited $\frac{coin_{\st\mathcal C}^{\st*}}{z}-o$ coins for the $j$-th verification, with a high probability.  We now move on to event 
     %
  $$  \Big(F(u^{\st *},\bm{q}_{\st j}, {pp})\neq h_{\st j} \ \wedge (d_{\st j}=1	\vee y_{\st \mathcal{S},j}=0 \ \vee \  {coin_{\st\mathcal{C},j}\neq \frac{coin_{\st\mathcal C}^{\st*}}{z}+l} ) \Big)$$
    
    
    
     
     It captures the case where the server provides an invalid  proof but either persuades the client to accept the proof, or  persuades the contract to set $y_{\st \mathcal{S},j}=0$  or makes the client  withdraw incorrect amounts of coin, i.e.    $coin_{\st\mathcal{C},j}\neq \frac{coin_{\st\mathcal C}^{\st*}}{z}+l$.   Nevertheless, due to the soundness of PoR, the probability that a corrupt server can convince an honest client to accept invalid proof, i.e. outputs $d_{\st j}=1$, is negligible, $\mu(\lambda)$. So, the client detects it with a high probability and raises a dispute.  Also, the server may try to make the contract keep $y_{\st \mathcal {S},j}=0$. For $y_{\st \mathcal {S},j}=0$ to happen, it has to make the contract  recognise the client as the misbehaving party, i.e., makes the contract output $y_{\st \mathcal {C},j}=1$. In this case, the client's complaint would not be processed by the contract; therefore,  $y_{\st \mathcal {S},j}$ remains $0$.   Nevertheless, as we discussed above, the probability that the adversary makes the contract  recognise the client as misbehaving is negligible, $\mu(\lambda)$. Therefore, with a high probability  $y_{\st \mathcal {S},j}=1$ and $y_{\st \mathcal {C},j}=0$, after the contract  is invoked by the client or  server. The adversary may  try to  make the client withdraw  incorrect amounts of coin, e.g., in the case where it does not succeed in convincing the client or contract. To do so,  in the coin transfer phase, it has to send a  different accepting statement  than what was initially agreed with the client. But, it would succeed only with a negligible   probability, $\mu(\lambda)$, due to the security of SAP.   So, according to Equation \ref{equ::what-client-recives-in-j-2}, the client is credited $\frac{coin_{\st\mathcal C}^{\st*}}{z}+l$ coins for the $j$-th verification, with a high probability. 
 % \hfill\(\Box\)
  \end{proof}

%We first consider event $F(u^{\st *},\bm{q}_{\st j})= h_{\st j}\ \wedge coin_{\st\mathcal{C},j}\neq  \frac{coin_{\st\mathcal C}^{\st*}}{z}-o$ that captures the case where the server provides an accepting service proof but makes an honest client withdraw an incorrect amounts of coin, i.e. $coin_{\st\mathcal{C},j}\neq  \frac{coin_{\st\mathcal C}^{\st*}}{z}-o$. Since the proof is valid, an honest client accepts it and does not raise any dispute. 
%  However, the server  would be able to make the client  withdraw incorrect amounts of coins, if it manages to either convince the arbiter that the client has misbehaved (by making the arbiter increment $y_{\st\mathcal {C}}$  by $1$ through dispute resolution phase), or submit to the contract, at the coin transfer phase,  an accepting  statement $\ddot{x}'_{\st cp}$ other than what was agreed at the initiation phase, i.e. $\ddot{x}_{\st cp}$. Nevertheless, it cannot falsely accuse the client of misbehaviour. Because,  due to the security of SAP, it cannot  convince the arbiter to accept different decryption key or pads other than what was agreed with the client in the initiation phase; specifically, it cannot persuade the arbiter to accept  $\ddot{x}'_{\st qp}$, where $\ddot{x}'_{\st qp}\neq \ddot{x}_{\st qp}$, except with a negligible probability, $\mu(\lambda)$. This ensures that the honest client's message is accessed by  the arbiter with a high probability, as the arbiter can extract the client's message using valid pad information and decryption key.  On the other hand, if the adversary provides a valid statement, i.e. $\ddot{x}_{\st qp}$, then due to the correctness of VSID, algorithm $\mathtt{VSID.identify}()$ outputs $I_{\st j}=\bot$. Therefore, due to the security of SAP and correctness of VSID,   $y_{\st\mathcal {C}}$ and $y_{\st\mathcal {S}}$ are not incremented by $1$  in $j$-th verification, i.e. $y_{\st\mathcal{C}}[j]=y_{\st\mathcal{S}}[j]=0$.  Moreover,  due to the security of SAP, the server cannot persuade the contract to accept any statement other than what was agreed initially between the client and server, except with a negligible probability $\mu(\lambda)$ when it finds the hash function's collision. Recall, in the protocol, the total coins the client receives after $z$ verifications is $coin^{\st *}_{\st\mathcal C}-o(z-y_{\st\mathcal S})-l\cdot y_{\st\mathcal C}$. Since we focus on each $j$-th verification, the amount of  coins credited to the client for that verification is
%  
%  \begin{equation}\label{equ::what-client-recives-in-j}
%   \frac{coin^{\st *}_{\st\mathcal C}}{z}-o(1-y_{\st\mathcal S}[j])-l\cdot y_{\st\mathcal C}[j]
%     \end{equation}
%     
%     In the above event, as we discussed,  with a high probability $y_{\st\mathcal{C}}[j]=y_{\st\mathcal{S}}[j]=0$ , so the client is credited $\frac{coin_{\st\mathcal C}^{\st*}}{z}-o$ coins for that verification. 
%     
   

Next, we prove that ${\text{RC-}\overline{\text{PoR}}\text{-P}}$ satisfies security against a malicious client. The proof is also slightly simpler than that  of RC-PoR-P against a malicious client (i.e., proof of Claim \ref{claim::RC-PoR-P-SecurityAgainstMaliciousClient}) as it does not involve any third party arbiter. 


\begin{lemma}
 If SAP and blockchain are secure and  PoRID scheme supports correctness, inputs well-formedness, and detectable abort, then ${\text{RC-}\overline{\text{PoR}}\text{-P}}$ is secure against malicious client, w.r.t. Definition \ref{deff::RC-S-P-Security-Against Malicious-Client-2}. 
\end{lemma}


\begin{proof}
  First, we consider event 
  %
   $$\Big((M(u^{\st *},k,{pp})= \sigma \  \wedge \ Q(\text{aux},k, {pp})= \bm{q}_{\st j})\ \wedge \
(coin_{\st\mathcal{S},j}\neq  \frac{coin_{\st\mathcal S}^{\st*}}{z}+o)\Big)$$
  
  
  It captures the case where the client provides  accepting metadata and query  but makes the server withdraw an incorrect amounts of coin, i.e. $coin_{\st\mathcal{S},j}\neq  \frac{coin_{\st\mathcal S}^{\st*}}{z}+o$. According to  ${\text{RC-}\overline{\text{PoR}}\text{-P}}$ protocol, the total coins the server should receive after $z$ verifications is $coin^{\st *}_{\st\mathcal S}+o\cdot(z-y_{\st\mathcal S})+l\cdot(y_{\st\mathcal C}-y_{\st\mathcal S})$. As we focus on  $j$-th verification, the amount of  coins that should be credited to the server for the $j$-th verification is
  %
  \begin{equation}\label{equ::what-server-recives-in-j-2}
   coin_{\st\mathcal{S},j}=\frac{coin^{\st *}_{\st\mathcal S}}{z}+o\cdot(1-y_{\st\mathcal {S},j})+l\cdot(y_{\st\mathcal {C},j}-y_{\st\mathcal {S},j})
     \end{equation}
  
  
  
  Since the metadata and query are valid, an honest server accepts them and does not raise any dispute, so we have $y_{\st\mathcal{C},j}=0$.  The client however could  make the server  withdraw incorrect amounts of coin, if it manages to either convince the contract, in the dispute resolution phase,  that the server has misbehaved, i.e., makes the contract output $y_{\st\mathcal{S},j}=1$, or submit to the contract  an accepting  statement $\ddot{x}'_{\st cp}$ other than what was agreed at the initiation phase, i.e. $\ddot{x}_{\st cp}$, in the coin transfer phase. But, it cannot falsely accuse the server of misbehaviour, because due to the security of SAP, it cannot convince the contract to accept different decryption key and pads' detail, by providing a different accepting statement $\ddot{x}'_{\st qp}$  (where $\ddot{x}'_{\st qp}\neq \ddot{x}_{\st qp}$), than what was initially agreed with the server, except with a negligible  probability, $\mu(\lambda)$.  So, with a high probability $y_{\st\mathcal{S},j}=0$. On the other hand, if the adversary provides a valid statement, i.e. $\ddot{x}_{\st qp}$, then due to the correctness of the PoR and query-checking process,  we would have $I_{\st j}=\bot$. Thus, due to the security of SAP and the correctness of the PoR and query-checking process,  we would have $y_{\st\mathcal{C},j}=y_{\st\mathcal{S},j}=0$ with a high probability.    Also,  due to the security of SAP, the client cannot change the payment parameters by convincing the contract to accept any accepting statement $\ddot{x}'_{\st cp}$ other than what was initially agreed between the client and server (i.e. $\ddot{x}'_{\st cp}\neq \ddot{x}_{\st cp}$), except with a negligible probability, $\mu(\lambda)$. That means, according to  Equation \ref{equ::what-server-recives-in-j-2}, the server is credited $\frac{coin_{\st\mathcal S}^{\st*}}{z}+o$ coins for that verification, with a  high probability.  We now move on  to 
  %
  $$\Big(M(u^{\st *},k,{pp})\neq \sigma\ \wedge \ a=1\Big)$$
     
     
    It captures the case where the server accepts ill-formed metadata. However, due to the security of the Merkle tree scheme, the probability of the event happening is negligible,  $\mu(\lambda)$. So, with a high probability $a=0$; in this case,  the server does not raise any dispute, instead it avoids serving the client.    Next, we turn our attention   to 
     %
     $$\Big(Q(\text{aux},k,{pp})\neq \bm{q}_{\st j})\ \wedge \ (b_{\st j}=1\ \vee \ y_{\st\mathcal{C},j}=0 \ \vee \ coin_{\st\mathcal{S},j}\neq \frac{coin_{\st\mathcal S}^{\st*}}{z}+o+l)\Big)$$
     
       It considers the case where the client provides an invalid query, but  either convinces the server or contract to accept it, or  makes the server   withdraw  incorrect amounts of coin, i.e. $coin_{\st\mathcal{S},j}\neq \frac{coin_{\st\mathcal S}^{\st*}}{z}+o+l$.  Due to the correctness of the query-checking process, the probability that the server outputs $b_{\st j}=1$ is $0$.  When the honest server rejects the query and raises a dispute, the contract checks the server's query and sets $y_{\st\mathcal{C},j}=1$. After that, due to the security of blockchain the client cannot make the contract to set $y_{\st\mathcal{C},j}=0$ except with probability $\mu(\lambda)$. Also, as discussed above, the client cannot make the contract recognise the  honest server as a misbehaving party with a probability significantly greater than $\mu(\lambda)$. That means with a high probability $y_{\st\mathcal{S},j}=0$.  The adversary may still try to  make the server withdraw   incorrect amounts of coin (e.g., if the adversary does not succeed in convincing the server). To this end, at the coin transfer phase, it has to convince the contract to accept a  different  statement  than what was initially agreed with the server. However, due to the security of SAP, its  success probability is negligible, $\mu(\lambda)$.     Hence, according to Equation \ref{equ::what-server-recives-in-j-2}, the server is credited  $\frac{coin_{\st\mathcal S}^{\st*}}{z}+o+l$ coins for the $j$-th verification.   
 %\hfill\(\Box\)
 \end{proof}
  
  
In the following, we provide a lemma for  ${\text{RC-}\overline{\text{PoR}}\text{-P}}$'s privacy. For the lemma's proof, we refer readers to the proof of Claim \ref{claim::RC-PoR-P-privacy}. 
%
\begin{lemma} If SAP is secure and the encryption scheme is semantically secure, then ${\text{RC-}\overline{\text{PoR}}\text{-P}}$ preserves privacy, w.r.t. Definition \ref{deff::RC-S-P-Privacy}. 
\end{lemma}

%
%\begin{proof}[sketch] Briefly, due to SAP's privacy property, given  commitments $g_{\st qp}$ and $g_{\st cp}$ (stored in the blockchain as a result of running SAP) the adversary learns no information about the committed values (e.g. $o, l, pad_{\st\pi}$ and $\bar{k}$), except with negligible probability $\mu(\lambda)$. Moreover, given  price list $pl$, and the parties' encoded coins $coin^{\st *}_{\st\mathcal{C}}$ and  $coin^{\st *}_{\st\mathcal{S}}$, the adversary learns nothing about the actual price agreed between the server and client, i.e. $(o,l)$, for each verification, due to Lemma \ref{lemma::encoded-coins}.  Also, since each proof $\bm{\pi}^{\st *}_{\st j}$ is encrypted and then padded, given $\bm{\pi}^{\st *}_{\st j}$ the adversary cannot tell  whether $\bm{\pi}^{\st *}_{\st j}$ is associated with $u_{\st 0}$ or with $u_{\st 1}$ (i.e. where $u_{\st 0}$ and $u_{\st 1}$ are the adversary's choice of files), with probability significantly greater than $\frac{1}{2}+\mu(\lambda)$. As each ciphertext $\hat{k}^{\st *}_{\st j}$ is an output a semantically secure symmetric key encryption scheme, it leaks noting to the adversary.  The value of $a$ is also independent of $u_{\st 0}$  or $u_{\st 1}$, and only depends on whether the metadata is well-formed, so it leaks nothing about the service input $u_{\st\beta}$ and $\beta\in\{0,1\}$. Hence, the adversary cannot tell with a probability significantly greater than $\frac{1}{2}+\mu(\lambda)$ which file of its choice has been used as the server input. 
%
%Furthermore, since each query and padded encrypted proof leak no information and always contain a fixed number of elements, an adversary cannot tell the status of  proof for each $j$-th verification (i.e. whether it is accepted or rejected) with the probability greater than $\frac{1}{2}+\mu(\lambda)$, given  $\hat{k}^{\st *}_{\st j},coin^{\st *}_{\st \mathcal S},coin^{\st *}_{\st\mathcal C}, g_{\st cp},  g_{\st qp},$  $\bm{\pi}^{\st *},pl$, and $a$.
%  \hfill\(\Box\)\end{proof}
%



==> commitment.tex <==
% !TEX root =main.tex




\subsection{Commitment Scheme}\label{subsec:commit}


 A commitment scheme involves two parties,  \emph{sender} and  \emph{receiver}, and includes  two phases: \emph{commit} and  \emph{open}. In the commit phase, the sender  commits to a message: $x$ as $\mathtt{Com}(x,r)=\mathtt{Com}_{\st x}$, that involves a secret value: $r\stackrel{\st\$}\leftarrow \{0,1\}^{\st\lambda}$. In the end of the commit phase,  the commitment $\mathtt{Com}_{\st x}$ is sent to the receiver. In the open phase, the sender sends the opening $\ddot{x}:=(x,r)$ to the receiver who verifies its correctness: $\mathtt{Ver}(\mathtt{Com}_{\st x},\ddot{x})\stackrel{\st ?}=1$ and accepts if the output is $1$.  A commitment scheme must satisfy two properties: (a) \textit{hiding}: it is infeasible for an adversary (i.e., the receiver) to learn any information about the committed  message $x$, until the commitment $\mathtt{Com}_{\st x}$ is opened, and (b) \textit{binding}: it is infeasible for an adversary (i.e., the sender) to open a commitment $\mathtt{Com}_{\st x}$ to different values $\ddot{x}':=(x',r')$ than that was  used in the commit phase, i.e., infeasible to find  $\ddot{x}'$, \textit{s.t.} $\mathtt{Ver}(\mathtt{Com}_{\st x},\ddot{x})=\mathtt{Ver}(\mathtt{Com}_{\st x},\ddot{x}')=1$, where $\ddot{x}\neq \ddot{x}'$.  There exist efficient non-interactive  commitment schemes both in (a) the standard model, e.g., Pedersen scheme \cite{Pedersen91}, and (b)  the random oracle model using the well-known hash-based scheme such that committing  is : $\mathtt{H}(x||r)=\mathtt{Com}_{\st x}$ and $\mathtt{Ver}(\mathtt{Com}_{\st x},\ddot{x})$ requires checking: $\mathtt{H}(x||r)\stackrel{\st ?}=\mathtt{Com}_{\st x}$, where $\mathtt{H}:\{0,1\}^{\st *}\rightarrow \{0,1\}^{\st\lambda}$ is a collision resistant hash function; i.e., the probability to find $x$ and $x'$ such that $\mathtt{H}(x)=\mathtt{H}(x')$ is negligible in the security parameter $\lambda$.

==> experiment-details.tex <==
% !TEX root =main.tex
  
  
  
  \section{Experiment details}\label{sec:Experiment-details}
  
  The RC-PoR-P's off-chain and on-chain parts have been implemented in  C++ and Solidity programming languages respectively. To conduct the off-chain experiment, we used  a server with dual Intel Xeon Gold 5118,   2.30 GHz CPU and 256 GB RAM. To carry out the on-chain experiment, we used a MacBook Pro laptop with quad-core Intel Core i5, 2 GHz CPU  and 16 GB RAM that interacts with the Ethereum private blockchain. We ran the experiment $10$ times. In the experiment, we used the SHA-2 hash function and set its output length and the security parameter  to $128$ bits.  We  set the size of every block to $128$ bits, as in \cite{DBLP:conf/asiacrypt/ShachamW08}.   We used a random file whose  size is in the range $[64\ \text{MB},4\ \text{GB}]$. This results in the number of file blocks in the range $[2^{\st 22},2^{\st 28}]$. 

Since in the  experiment we used  relatively large file sizes, to lower on-chain transaction costs, we allow  the parties to use the technique  explained in Appendix \ref{subsec:RCSP_discussion}, which lets the server and client exchange  the (PoR) proofs off-chain in an irrefutable fashion\footnote{\scriptsize For each $j$-th verification, $\mathcal{S}$ sends each related path to $\mathcal{C}$, via an authenticated channel. If $\mathcal{C}$ rejects a path, then it inserts into its complaint  $\mathcal{S}$'s message that includes one of the invalid paths for $j$-th  verification. Our analysis excludes signature generation and verification processes as they can be efficiently incorporated by using standard authenticated channels (e.g., PKI-based XML signatures).}. The prototype implementation utilises the Cryptopp \cite{cryptopp} and  GMP \cite{gmp} libraries. 

==> long-PoR-def.tex <==
% !TEX root =main.tex

In general, a PoR scheme considers the case where an honest client wants to store its file(s) on a  potentially malicious server, i.e active adversary. It is a challenge-response interactive protocol, where the server proves to the client that its file is intact and retrievable. Below, we restate PoR's formal definition (and security property) originally provided in \cite{DBLP:journals/iacr/JuelsK07,DBLP:conf/asiacrypt/ShachamW08}. A PoR scheme comprises five algorithms: 

\begin{itemize}
\item[$\bullet$] $\mathtt{PoR.keyGen}(1^{\lambda})\rightarrow k:=(sk,pk)$.  A probabilistic algorithm, run by a client. It takes as input the security parameter  $1^{\lambda}$ and outputs  private and public verification keys $k:=(sk,pk)$.

\

\item[$\bullet$] $\mathtt{PoR.setup}(1^{\lambda}, u,k)\rightarrow (u^{\st *}, \sigma, {pp})$. A probabilistic algorithm, run by the client. It takes as input the security parameter $1^{\lambda}$,  a file $u$, and key $k$. It encodes $u$, denoted by $u^{\st *}$ and generates   metadata, $\sigma$.  The client outputs encoded file $u^{\st *}$, metadata $\sigma$, and  { (possibly file dependent) public parameters $pp$}. It sends $u^{\st *},\sigma$, and { $pp$} to the server.

\

\item[$\bullet$] $\mathtt{PoR.genQuery}(1^{\lambda},k,{ pp})\rightarrow \bm{q}$. A probabilistic algorithm, run by the client. It takes as input the security parameter  $1^{\lambda}$,  key $k$, and {  public parameters $pp$}. It outputs a  query vector $\bm{q}$, possibly picked uniformly at random. The query is given to the server. 

\

\item[$\bullet$] $\mathtt{PoR.prove}(u^{\st *}, \sigma,\bm{q},pk,{ pp})\rightarrow \pi$. It is run by the server.  It takes as input the encoded file $u^{\st *}$, metadata $\sigma$, query $\bm{q}$,  public key $pk$, and {  public parameters $pp$}. It  outputs a proof, $\pi$, given to the client. 

\

\item[$\bullet$] $\mathtt{PoR.verify}(\pi,\bm{q},k,{ pp})\rightarrow d\in\{0,1\}$. It is run by the client. It takes as input the proof $\pi$,  query $\bm{q}$,  key pair $k$, and {  public parameters $pp$}. It outputs either $0$ if it rejects,  or $1$ if it accepts the proof. 

\end{itemize}


Informally, a PoR scheme has two main properties: \emph{correctness} and \emph{soundness}. Correctness requires that the verification algorithm accepts  proofs generated by an honest verifier. Formally, it requires that for any key $k$, any file $u\in\{0,1\}^{\st *}$, and any  pair $(u^{\st *},\sigma)$ output by $\mathtt{PoR.setup}(1^{\st\lambda}, u,k)$, and any query $\bm{q}$, the verifier  accepts when it interacts with an honest prover.

 Soundness requires that if a prover convinces the verifier (with high probability) then the file is stored by the prover. This is formalized via the notion of an extractor algorithm, that is able to extract the file in interaction with the adversary using a polynomial number of  rounds. Before we define  soundness, we restate the  experiment, defined in \cite{DBLP:conf/asiacrypt/ShachamW08}, that takes place between an environment $\mathcal{E}$ and  adversary $\mathcal{A}$. In this experiment, $\mathcal{A}$ plays the role of a corrupt party and $\mathcal{E}$ simulates an honest party's role. 


\begin{enumerate}
\item $\mathcal{E}$ executes $\mathtt{PoR.keyGen}(1^{\lambda})$ algorithm and provides public key, $pk$, to $\mathcal{A}$.   
\item $\mathcal{A}$ can pick  arbitrary file $u$, and  uses it to make queries to  $\mathcal{E}$ which runs  $\mathtt{PoR.setup}(1^{\lambda}, u,k)\rightarrow (u^{\st *}, \sigma, { pp})$   and returns the output to $\mathcal{A}$. Also, upon receiving the output of $\mathtt{PoR.setup}(1^{\lambda}, u,k)$, $\mathcal{A}$ can ask $\mathcal{E}$  to run   $\mathtt{PoR.genQuery}(1^{\lambda}$ $, k,{ pp})\rightarrow \bm{q}$ and give the output to it. $\mathcal{A}$ can locally run $\mathtt{PoR.prove}(u^{\st *}, \sigma, \bm{q},pk,{ pp})\rightarrow \pi$ to get its outputs as well. 
\item $\mathcal{A}$ can request from $\mathcal{E}$ the execution of $\mathtt{PoR.verify}(\pi,\bm{q},k,{ pp})$ for any $u$ used to query $\mathtt{PoR.setup}(.)$. Accordingly, $\mathcal{E}$ informs  $\mathcal{A}$ about the verification output. The adversary can send a polynomial number of queries to $\mathcal{E}$. Finally, $\mathcal{A}$ outputs metadata $\sigma$ returned from a setup query and the description of a prover, $\mathcal{A}'$, for any file it has already chosen above. 
\end{enumerate}

It is said that a cheating prover, $\mathcal{A}'$, is \emph{$\epsilon$-admissible} if it convincingly answers $\epsilon$ fraction of verification challenges. Informally, a PoR scheme supports extractability, if there is an extractor algorithm $\mathtt{Ext}(k,\sigma, \mathtt{P}')$, that takes as input the key $k$, metadata $\sigma$, and the description $\mathtt{P}'$ of the  machine implementing the prover's role $\mathcal{A}'$ and outputs the file, $u$. The extractor has the ability to reset the adversary to the beginning of the challenge phase and repeat this step polynomially many times for the purpose of extraction, i.e., the extractor can rewind $\mathtt{P}'$.


%XXXXThomas: \emph{What is actually the entity that can be rewinded (i.e., the adversary)? Is it $\mathtt{P}'$ or $\mathcal{A}'$?}XXXX. Aydin: done


\begin{definition}[$\epsilon$-soundness]\label{extractable} A PoR scheme is $\epsilon$-sound if   there exists an extraction algorithm $\mathtt{Ext}(.)$ such that, for every adversary $\mathcal{A}$ which plays the experiment above and outputs an $\epsilon$-admissible cheating prover $\mathcal{A}'$ for a file $u$,  the extraction algorithm  recovers $u$ from $\mathcal{A}'$, given honest party's private key, public parameters, metadata and the description of $\mathcal{A}'$,  i.e., $\mathtt{Ext}(k,{ pp},\sigma, \mathtt{P}')\rightarrow u$, except with a negligible probability. 
\end{definition}






%\begin{definition}[$\epsilon$-sound]\label{extractable} A PoR scheme is $\epsilon$-sound if  for every adversary, $\mathcal{A}$, which plays the experiment above, and outputs an $\epsilon$-admissible cheating prover $\mathcal{A}'$, for a file $u$,  there exists an extraction algorithm $\mathtt{Ext}()$, that recovers $u$ from $\mathcal{A}'$, given honest parties public-private keys, metadata and the description of $\mathcal{A}'$,  i.e. $\mathtt{Ext}(k,\sigma, \mathtt{P}')\rightarrow u$, except with a negligible probability. 
%\end{definition}


In contrast to the PoR definition in \cite{DBLP:journals/iacr/JuelsK07,DBLP:conf/asiacrypt/ShachamW08} where $\mathtt{PoR.genQuery}(.)$ is implicit, in the above we have explicitly defined  $\mathtt{PoR.genQuery}(.)$, as it    plays an important role in this paper. Also, there are PoR protocols, e.g., in \cite{MillerPermacoin}, that do not involve $\mathtt{PoR.keyGen}(.)$. Instead, a set of public parameters/keys (e.g., file size or a root of Merkle tree) are output by $\mathtt{PoR.setup}(.)$. To make the PoR definition generic to capture both cases, we have explicitly included the public parameters $pp$ in the algorithms definitions too.  







==> old-RC-PoR-P-Evaluation.tex <==
% !TEX root =main.tex


\vspace{-2mm}

\section{Evaluation of RC-PoR-P}\label{sec:evaluation}
\vspace{-1mm}


\input{RC-PoR-P-run-time}
\input{table-PoR-cost}


In this section, we provide an analysis of the RC-PoR-P protocol. %, presented in Section \ref{sec::RC-PoR-P-protocol}.  
%
%Tables \ref{table::RCPoRP-Asymptotic-Cost} and \ref{table::RC-PoR-P-runTime} summarises the protocol's asymptotic and concrete costs respectively. 
%
    Table \ref{table::RC-PoR-P-runTime} summarises its concrete cost (we provide a table for its asymptotic cost in Appendix \ref{sec::RC-PoR-P-Assymptotic-Cost}). 
%
Also, we compare RC-PoR-P  with  (a) the zero-knowledge contingent (publicly verifiable) PoR payment  in \cite{CampanelliGGN17} and  the fair PoR payment scheme in \cite{s-PoR} as they are more efficient than the state-of-the-art and closest to our work. Table \ref{table::Cost-comp} summarises the comparison.  To conduct the concrete cost study, we have implemented  RC-PoR-P. We  set the size of every block to $128$ bits, as in \cite{DBLP:conf/asiacrypt/ShachamW08}.   We used a random file whose  size is in the range $[64\ \text{MB},4\ \text{GB}]$. This results in the number of file blocks in the range $[2^{\st 22},2^{\st 28}]$. The protocol's off-chain and on-chain source codes are publicly available in \cite{RC-S-P-off-chain} and \cite{RC-S-P-on-chain} respectively. We refer readers to Appendix \ref{sec:Experiment-details}, for further details about the experiment setup. 





\vspace{-2mm}

\subsection{Computation Cost}\label{subsec:comp_cost}
\vspace{-1mm}

In our analysis,  the cost of erasure-coding a file is not taken into consideration,  as it is identical in all PoR schemes. In RC-PoR-P, $\mathcal{C}$'s cost in phase \ref{RCPoRP::Client-side-Initiation} is $O(m)$. In this  phase, its off-chain \emph{run-time} increases by about $2\times$ (i.e.,  from $23.1$ to  $45.5,...,$ from $732.1$ to $1596.6$ seconds) when $m$ increases (i.e., from $2^{\st 22}$ to $2^{\st 23},...,$ from $2^{\st 27}$ to $2^{\st 28}$ blocks). This phase also  costs it $123\cdot 10^{\st -5}$ ether.  $\mathcal{C}$'s complexity in phase \ref{Billing-cycles-genQuery} is  $O(z\cdot \phi)$. Its off-chain run-time in this phase is negligibly small. This phase also costs it $6\cdot 10^{\st -5} \cdot z$ ether. Also, its complexity in  phase \ref{RC-PoR-P::Client-side-Proof-Verification} is  $O(z\cdot\phi\cdot \log_{\st 2}(m))$. Its off-chain run-time in this phase is very low and  grows  almost $1.1\times$   (i.e., from $0.09 \cdot z$ to $0.11 \cdot z, ...,$ from $0.21\cdot z$ to $0.24\cdot z$ seconds) when $m$ increases. 
 
 
 


Now, we analyse $\mathcal{S}$'s computation cost. In phase \ref{RCPoRP::Server-side-Initiation}, $\mathcal{S}$'s complexity is $O(m)$. Its off-chain run-time in this phase grows $2\times$  (i.e., from $8.9$ to $16.5, ...,$ from $248.8$ to $548.8$ seconds)  when $m$ increases. This phase costs it  $9\cdot 10^{\st -5}$ ether. $\mathcal{S}$'s complexity in phase \ref{RC-PoR-P::Server-side-Proof-Generation} is $O(z\cdot\phi\cdot \log_{\st 2}(m))$.  In this phase, its off-chain run-time grows  about  $2.1\times$ (i.e., from $22.4\cdot z$ to  $30.4 \cdot z,...,$ from $793.1\cdot z$ to $1820.7\cdot z$ seconds) when $m$ increases.\footnote{\scriptsize To determine $\mathcal{S}$'s cost for generating a proof, we considered the case where $\mathcal{S}$ does not store the Merkle tree nodes (to save storage space), instead it generates the tree's paths every time a challenge is given to it. If we let $\mathcal{S}$  store the tree, then it would have a lower computation overhead.} 
 

%\TZ{The adverbs ``gently'' and ``slowly'' are subjective. This worries me a bit. For instance $2^28$ is $64$ times greater than $2^22$, however $1820.7$ is $81$ times bigger than $22.4$. I would not consider growth by a constant $>1$ as ``slow''.}




$\mathcal{R}$’s cost in phase \ref{RCPoRP::Dispute-Resolution} is at most $O(z\cdot \log_{\st2}(m))$.  Due to the use of the proof of misbehaviour in the protocol, $\mathcal{R}$’s cost is about $\frac{1}{\phi}=\frac{1}{460}$ of its computation cost in the absence of such a technique where it has to check all $\phi$ proofs for each verification.\footnote{\scriptsize As shown in \cite{DBLP:conf/ccs/AtenieseBCHKPS07}, to ensure 99\% of file blocks is retrievable, it would be sufficient to set the number of challenged blocks to $460$.} Its off-chain run-time is very low and   increases about $1.3\times$ (i.e., from $2\cdot 10^{\st -5}\cdot z'$ to  $4\cdot 10^{\st -5}\cdot z', ...,$ from $9\cdot 10^{\st -5}\cdot z'$ to $10^{\st -4}\cdot z'$ seconds) when $m$ increases.  Phase  \ref{RCPoRP::Dispute-Resolution} also imposes $10^{\st -4}$ ether to $\mathcal{R}$.  
%
In phase \ref{RCPoRP::CoinTransfer}, SC  invokes the hash function only twice, so its computation complexity is constant. This phase imposes $6\cdot 10^{\st -5}$ ether to the party that calls  $\mathtt{RCPoRP}.\mathtt{pay}$. 

\vspace{-2mm}
%
\subsection{Communication Cost}\label{subsec:comm_cost} 
 \vspace{-1mm}
 
We first analyse $\mathcal{C}$'s communication cost. In phase \ref{RCPoRP::Client-side-Initiation}, $\mathcal{C}$ sends  ${||u^{\st *}||}+384$ bits. So,  in this phase, its complexity is $O(||u^{\st *}||)$. In phase \ref{RCPoRP::Dispute-Resolution}, it sends  $(\ddot{x}_{\st qp}, m_{\st\mathcal{C}})$, where $\ddot{x}_{\st qp}$ contains (a) padding information  whose size is a few bits and (b) the symmetric-key encryption's key whose size is  $128$ bits. Also,   $m_{\st\mathcal{C}}$  contains at most $z$ invalid paths of the Merkle tree. Thus, in this phase, its communication cost is  $z\cdot \log_{\st 2}(||u^{\st *}||)+128$ bits or $O(z\cdot \log_{\st 2}(||u^{\st *}||))$.  
%
$\mathcal{S}$'s complexity for $z$ verifications is $O(z\cdot ||\bm{\pi}^{\st *}_{\st j}||)$, as in phase  \ref{RC-PoR-P::Server-side-Proof-Generation}, for each verification, it sends out a proof vector $\bm{\pi}^{\st *}_{\st j}$. 
%
$\mathcal{R}$'s communication cost is constant, as it only sends a transaction containing four values in phase \ref{RCPoRP::Dispute-Resolution}. 

\vspace{-2mm}

%%%%%%%%%%%%%
\subsection{Comparison}
\vspace{-1mm}


 The PoR scheme in \cite{s-PoR} assumes that $\mathcal{C}$ is trusted. The initiation phase involves
 $O(z)$ modular exponentiations and $O(m+z\phi)$ multiplications to generate puzzles and MACs respectively.  $\mathcal{S}$  performs $O(Tz)$ exponentiations and $z$ multiplications to solve the puzzles, where $T$ is a time parameter. For $z$ verifications, $\mathcal{S}$ performs $O(z\phi)$ multiplications to generate $z$  proofs. A verifier performs $O(z\phi)$ multiplications to verify all proofs. 
 
 
 
 

 %
 As we showed in Section \ref{sec:attack-mitigation}, the scheme in \cite{CampanelliGGN17} is not secure against a malicious $\mathcal{C}$.  In this scheme, $\mathcal{C}$ generates a signature for each file block which involves $O(m)$ exponentiations. For $\mathcal{S}$ to generate $z$ proofs, it performs $O(z\phi)$ exponentiations and invokes zk proof system $O(z\phi)$ times.  The verifier has the same computation complexity as the prover. Campanelli \textit{et al.} \cite{CampanelliGGN17} provide an implementation of zkCSP for publicly  and privately verifiable PoRs. \textbf{The total size of the outsourced file used in their experiment is at most  $\bm{256}$ bits, which is very small}. In contrast, in our experiment, we used a much large file size, i.e., $4$-GB.  

 
 
 
 
 The proof size in the schemes in \cite{s-PoR} and \cite{CampanelliGGN17} is  $O(1)$.  They do not address the privacy issue highlighted in Section \ref{sec::Lack-of-Privacy}. Nevertheless, RC-PoR-P is secure against a malicious $\mathcal{C}$ and rectifies the privacy issue. Similar to the other two schemes, its initiation complexity is  $O(m)$; unlike them, it does not require any modular exponentiations.  Instead, it involves symmetric key operations which impose much lower overheads. Moreover, unlike the other two schemes that have $O(z\phi)$ complexity in the prove and verify phases, RC-PoR-P's complexity, in theory, is slightly higher, i.e., it is $O(z\phi \log_{\st 2}(m))$. RC-PoR-P's prove and verify algorithms, similar to the ones  \cite{s-PoR}, involve only symmetric key operations; whereas, the ones in \cite{CampanelliGGN17} need asymmetric key operations. Also, in RC-PoR-P, the proof size complexity is larger than the other two schemes. %However, each message length in RC-PoR-P is much shorter than the one in \cite{CampanelliGGN17}, i.e., $128$-bit vs $2048$-bit. 

Thus,  RC-PoR-P is computationally more efficient than  \cite{CampanelliGGN17} and  \cite{s-PoR} while offering stronger security guarantees, i.e., security against a malicious client and privacy.

%%%%%%%%%
%







 









==> table-PoR-cost-old.tex <==
% !TEX root =main.tex


 \begin{table*}[!htbp]

\caption{ \small Contingent PoRs' Cost  Comparison. } \label{table::Cost-comp} 
\begin{footnotesize}
\begin{center}
\renewcommand{\arraystretch}{.80}
%\scalebox{1}{
%\begin{subtable}{.56\linewidth}%xxxx
\begin{minipage}{1\linewidth}
%\caption{\small Computation and I/O Costs}
\setlength{\tabcolsep}{1pt}%compress the table horizontally
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 

   \hline
\cellcolor[gray]{.9}&\cellcolor[gray]{.9}&
 \multicolumn{4}{c|}{\cellcolor[gray]{.9}\scriptsize \underline{ \  \  \  \  \   \  \    \  \  \  \ \  \  \  \  \  \  \ \  \  \      Computation Cost     \  \  \  \  \   \  \    \  \  \  \ \  \  \  \  \  \  \ \  \  \   }}& \multicolumn{4}{c|}{\cellcolor[gray]{.9}\scriptsize \underline{\  \  \  \  \  \  \ \ \  \  \  \  \  \   \  \  \  \  \  \  \  \  Communication Cost   \  \  \  \  \   \  \    \  \  \  \ \  \  \  \  \  \  \ \  \  \   }}\\
% \cline{3-6}
  \cellcolor[gray]{.9}\multirow{-2}{*}{\scriptsize Protocols} &\cellcolor[gray]{.9}\multirow{-2}{*} {\scriptsize Operation}&\cellcolor[gray]{.9}\scriptsize$\mathtt{Initiate}$&\cellcolor[gray]{.9}\scriptsize$\mathtt{Solve\ Puzzle}$&\cellcolor[gray]{.9}\scriptsize$\mathtt{Prove}$&\cellcolor[gray]{.9}\scriptsize$\mathtt{Verify}$&\cellcolor[gray]{.9} {\scriptsize Client}&\cellcolor[gray]{.9} {\scriptsize Server}&\cellcolor[gray]{.9} {\scriptsize Verifier}&\cellcolor[gray]{.9}{\scriptsize Proof Size}
  \\
\hline
    %SO-PoR 1st row
%\cellcolor[gray]{.9}& \multirow{2}{*}{\rotatebox[origin=c]{0}{\cellcolor[gray]{.9}\scriptsize }} \scriptsize Exp.&\scriptsize$z+1$&\scriptsize$T z$&\scriptsize$-$ &\scriptsize$-$&\scriptsize $128(n+$&&&\\
%     \cline{2-6}  
%     %SO-PoR 2nd row
% \multirow{-2}{*}{\rotatebox[origin=c]{0}{\cellcolor[gray]{.9}\scriptsize  SO-PoR }}&\cellcolor[gray]{.9}\scriptsize Add. or Mul.&\scriptsize$2(n+cz)$ &\scriptsize$z$&\scriptsize$4 c z$&\scriptsize$2z(1+c)$&\scriptsize  $cz+19z)$&\multirow{-2}{*}{\scriptsize $884z$}&\multirow{-2}{*}{\scriptsize$-$}&\multirow{-2}{*}{\scriptsize $O(1)$}\\
     \cline{2-6}   
      
     \hline 
       %[3] 1st row 
       
          \hline 
          
 \cellcolor[gray]{.9}  &\multirow{2}{*}{\rotatebox[origin=c]{0}{\scriptsize }}\cellcolor[gray]{.9}\scriptsize Exp.&\scriptsize$z+1$&\scriptsize$ T z$&\scriptsize$-$&$-$&&\scriptsize$-$&\scriptsize $-$&\\
     \cline{2-6}
    
     
    
     %[3] 2nd row 
\cellcolor[gray]{.9}   \multirow{-2}{*}{\rotatebox[origin=c]{0}{\scriptsize   \cite{s-PoR}}}  &\cellcolor[gray]{.9}\scriptsize Add. or Mul.&\scriptsize$2(m+\phi z)$&\scriptsize$z$&\scriptsize$4 \phi z$&\scriptsize$2z(1+\phi)$&\multirow{-2}{*} {\scriptsize $-$}&\scriptsize $-$&\scriptsize $-$&\multirow{-2}{*} {\scriptsize $-$}\\   

   \cline{2-6}

%      \cellcolor[gray]{.9}  &\multirow{2}{*}{\rotatebox[origin=c]{0}{\scriptsize }}\cellcolor[gray]{.9}\scriptsize Hash &\scriptsize$9 n$&\scriptsize$ -$&\scriptsize$-$&$-$&&\scriptsize$256z+$&\scriptsize $4672n+$&\\
%      
%         \cline{2-6}
%     
%      \cellcolor[gray]{.9}  &\multirow{2}{*}{\rotatebox[origin=c]{0}{\scriptsize }}\cellcolor[gray]{.9}\scriptsize Zero knowlege&\scriptsize$9 n$&\scriptsize$ -$&\scriptsize$-$&$-$&&\scriptsize$256z+$&\scriptsize $4672n+$&\\
      
      \hline
      
       \hline
      %[53] 1st row
  \cellcolor[gray]{.9}    &\multirow{2}{*}{\rotatebox[origin=c]{0}{\  \scriptsize }}\cellcolor[gray]{.9}\scriptsize Exp.&\scriptsize$-$&$-$&\scriptsize$-$&\scriptsize$-$&&&&\\
     \cline{2-6}
     %[53] 2nd row
 \cellcolor[gray]{.9}&\cellcolor[gray]{.9}\scriptsize Add. or Mul.&\scriptsize$-$&\scriptsize$-$&\scriptsize$-$&\scriptsize$-$&&&&\\ 
    \cline{2-6}
    %[53] 3rd row 
      \cellcolor[gray]{.9}  &\multirow{2}{*}{\rotatebox[origin=c]{0}{\scriptsize }}\cellcolor[gray]{.9}\scriptsize Hash &\scriptsize$-$&\scriptsize$ -$&\scriptsize$-$&$-$&&\scriptsize$-$&\scriptsize $-$&\\
      
         \cline{2-6}
     
      \cellcolor[gray]{.9} \multirow{-4}{*}{\rotatebox[origin=c]{0}{\scriptsize  \cite{CampanelliGGN17}}}   &\multirow{2}{*}{\rotatebox[origin=c]{0}{\scriptsize }}\cellcolor[gray]{.9}\scriptsize Zero knowlege&\scriptsize$-$&\scriptsize$ -$&\scriptsize$-$&$-$&&\scriptsize$-$&\scriptsize $-$&\\
 \hline
  
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 \hline
\cellcolor[gray]{.9}& \multirow{2}{*}{\rotatebox[origin=c]{0}{\cellcolor[gray]{.9}\scriptsize }} \scriptsize Hash&\scriptsize$6+2m(\sum\limits^{\scriptscriptstyle\log_{\scriptscriptstyle 2}(m)}_{\scriptscriptstyle i=1}\frac{1}{2^{\scriptscriptstyle i}})$&\scriptsize$-$&\scriptsize$\phi z\log_{\scriptscriptstyle 2}(m)$ &\scriptsize$((\phi z+z') \log_{\scriptscriptstyle 2}(m))+2$&&\scriptsize$-$&&\\
     \cline{2-6}  
 \multirow{-3}{*}{\rotatebox[origin=c]{0}{\cellcolor[gray]{.9}\scriptsize  \text{RC-PoR-P} }}&\cellcolor[gray]{.9}\scriptsize Sym. key enc.&\scriptsize$-$ &\scriptsize$-$&\scriptsize$\phi z(\log_{\scriptscriptstyle 2}(m)+1)+z$&\scriptsize$(\phi z+z') (\log_{\scriptscriptstyle 2}(m)+1)+z'$&\multirow{-2}{*} {\scriptsize $-$}&\scriptsize $-$&\multirow{-2}{*} {\scriptsize$-$}&\multirow{-2}{*} {\scriptsize$-$} \\
     \cline{2-6}    
     \hline 
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 
 
\end{tabular}  %xxxxxx
\end{minipage}
\end{center}
\end{footnotesize}
\end{table*}
%\vspace{-2mm}

%--------------------------------------------------------


% \begin{table*}[!htbp]
%\begin{footnotesize}
%\begin{center}
%\caption{ \small Outsourced PoR Cost  Comparison} \label{table::O-PoR-Cost} 
%\renewcommand{\arraystretch}{.80}
%%\scalebox{1}{
%%\begin{subtable}{.56\linewidth}%xxxx
%\begin{minipage}{1\linewidth}
%\caption{\small Computation and I/O Costs}
%\setlength{\tabcolsep}{.55pt}%compress the table horizontally
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
%
%   \hline
%\cellcolor[gray]{.9}&\cellcolor[gray]{.9}&
% \multicolumn{4}{c|}{\cellcolor[gray]{.9}\scriptsize \underline{\  \  \  \  \  \  \ \ \  \  \  \  \  \      Algorithms' Computation Cost     \  \  \  \ \  \  \  \  \  \  \ \  \  \   }}&\cellcolor[gray]{.9}&\cellcolor[gray]{.9}&\cellcolor[gray]{.9}&\cellcolor[gray]{.9}&\cellcolor[gray]{.9}\\
%% \cline{3-6}
%  \cellcolor[gray]{.9}\multirow{-2}{*}{\scriptsize Protocols} &\cellcolor[gray]{.9}\multirow{-2}{*} {\scriptsize Operation}&\cellcolor[gray]{.9}\scriptsize$\mathtt{Store}$&\cellcolor[gray]{.9}\scriptsize$\mathtt{SolvPuz}$&\cellcolor[gray]{.9}\scriptsize$\mathtt{Prove}$&\cellcolor[gray]{.9}\scriptsize$\mathtt{Verify}$&\cellcolor[gray]{.9}\multirow{-2}{*} {\scriptsize I/O Cost}&\cellcolor[gray]{.9}\multirow{-2}{*} {\scriptsize Client}&\cellcolor[gray]{.9}\multirow{-2}{*} {\scriptsize Server}&\cellcolor[gray]{.9}\multirow{-2}{*} {\scriptsize Verifier}&\cellcolor[gray]{.9}\multirow{-2}{*} {\scriptsize Proof Size}
%  \\
%\hline
%    %SO-PoR 1st row
%\cellcolor[gray]{.9}& \multirow{2}{*}{\rotatebox[origin=c]{0}{\cellcolor[gray]{.9}\scriptsize }} \scriptsize Exp.&\scriptsize$z+1$&\scriptsize$T z$&\scriptsize$-$ &$-$&&\scriptsize $128(n+$&&&\\
%     \cline{2-6}  
%     %SO-PoR 2nd row
% \multirow{-2}{*}{\rotatebox[origin=c]{0}{\cellcolor[gray]{.9}\scriptsize  SO-PoR }}&\cellcolor[gray]{.9}\scriptsize Add. or Mul.&\scriptsize$2(n+cz)$ &\scriptsize$z$&\scriptsize$4 c z$&\scriptsize$2z(1+c)$&\multirow{-2}{*} {\scriptsize $O(1)$}&\scriptsize  $cz+19z)$&\multirow{-2}{*}{\scriptsize $884z$}&\multirow{-2}{*}{\scriptsize -}&\multirow{-2}{*}{\scriptsize $O(1)$}\\
%     \cline{2-6}   
%      
%     \hline 
%       %[3] 1st row 
%       
%          \hline 
%          
% \cellcolor[gray]{.9}  &\multirow{2}{*}{\rotatebox[origin=c]{0}{\scriptsize }}\cellcolor[gray]{.9}\scriptsize Exp.&\scriptsize$9 n$&\scriptsize$ -$&\scriptsize$-$&$-$&&&\scriptsize$256z+$&\scriptsize $4672n+$&\\
%     \cline{2-6}
%     %[3] 2nd row 
%\cellcolor[gray]{.9}   \multirow{-2}{*}{\rotatebox[origin=c]{0}{\scriptsize   \cite{armknecht2014outsourced}}}  &\cellcolor[gray]{.9}\scriptsize Add. or Mul.&\scriptsize$10 n$&$-$&\scriptsize$4 z(c+c')$&\scriptsize$z(9c+3)$&\multirow{-2}{*} {\scriptsize $O(1)$}&\multirow{-2}{*} {\scriptsize $128n$}&\scriptsize $||\vv{\bm{F}}||$&\scriptsize $256z$&\multirow{-2}{*} {\scriptsize $O(1)$}\\   
%      
%      \hline
%      
%       \hline
%      %[53] 1st row
%  \cellcolor[gray]{.9}    &\multirow{2}{*}{\rotatebox[origin=c]{0}{\  \scriptsize }}\cellcolor[gray]{.9}\scriptsize Exp.&\scriptsize$-$&$-$&\scriptsize$z (3+c)$&\scriptsize$6 z$&&&&&\\
%     \cline{2-6}
%     %[53] 2nd row
% \cellcolor[gray]{.9}&\cellcolor[gray]{.9}\scriptsize Add. or Mul.&\scriptsize$4 n$&$-$&\scriptsize$2 z(3 c+4)$&\scriptsize$2 c z$&&&&&\\ 
%    \cline{2-6}
%    %[53] 3rd row 
%\cellcolor[gray]{.9}\multirow{-3}{*}{\rotatebox[origin=c]{0}{\scriptsize   \cite{xu2016lightweight}}}&\cellcolor[gray]{.9}\scriptsize Pairing&\scriptsize$-$&\scriptsize$-$&\scriptsize$7 z$&$-$&\multirow{-3}{*} {\scriptsize $O(1)$}&\multirow{-3}{*} {\scriptsize $2048n$}&\multirow{-3}{*} {\scriptsize $6144z$}&\multirow{-3}{*} {-}&\multirow{-3}{*} {\scriptsize $O(1)$}\\ 
% \hline
%  
%  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% \hline
%\cellcolor[gray]{.9}& \multirow{2}{*}{\rotatebox[origin=c]{0}{\cellcolor[gray]{.9}\scriptsize }} \scriptsize Exp.&\scriptsize$-$&\scriptsize$3T z$&\scriptsize$-$ &\scriptsize$3z$&&&\scriptsize$128cz \log n+$&&\\
%     \cline{2-6}  
% \multirow{-2}{*}{\rotatebox[origin=c]{0}{\cellcolor[gray]{.9}\scriptsize  \cite{Storage-Time} }}&\cellcolor[gray]{.9}\scriptsize Add. or Mul.&\scriptsize$-$ &\scriptsize$Tz$&\scriptsize$-$&\scriptsize$-$&\multirow{-2}{*} {\scriptsize $O(\log n)$}&\multirow{-2}{*} {\scriptsize $128$}&\scriptsize $4096z$&\multirow{-2}{*} {-}&\multirow{-2}{*} {\scriptsize$O(\log n)$} \\
%     \cline{2-6}    
%     \hline 
% 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% 
% 
%\end{tabular}  %xxxxxx
%\end{minipage}
%\end{center}
%\end{footnotesize}
%\end{table*}
%

%--------------------------------------------------------


